Efficient Uncertainty Tracking for Complex Queries with Attribute-level Bounds (extended version)

Certain answers are a principled method for coping with the uncertainty that arises in many practical data management tasks. Unfortunately, this method is expensive and may exclude useful (if uncertain) answers. Prior work introduced Uncertainty Annotated Databases (UA-DBs), which combine an under- and over-approximation of certain answers. UA-DBs combine the reliability of certain answers based on incomplete K-relations with the performance of classical deterministic database systems. However, UA-DBs only support a limited class of queries and do not support attribute-level uncertainty which can lead to inaccurate under-approximations of certain answers. In this paper, we introduce attribute-annotated uncertain databases (AU-DBs) which extend the UA-DB model with attribute-level annotations that record bounds on the values of an attribute across all possible worlds. This enables more precise approximations of incomplete databases. Furthermore, we extend UA-DBs to encode an compact over-approximation of possible answers which is necessary to support non-monotone queries including aggregation and set difference. We prove that query processing over AU-DBs preserves the bounds of certain and possible answers and investigate algorithms for compacting intermediate results to retain efficiency. Through an compact encoding of possible answers, our approach also provides a solid foundation for handling missing data. Using optimizations that trade accuracy for performance, our approach scales to complex queries and large datasets, and produces accurate results. Furthermore, it significantly outperforms alternative methods for uncertain data management.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> creating-uaadbs.tex <==
%!TEX root=./uaadb.tex
\subsection{Creating \abbrUAADBs}
\label{sec:creating-abbruaadbs}

One advantage that \abbrUAADBs inherit from \abbrUADBs is that other models for incomplete and probabilistic databases can be translated into this model such that the generated \abbrUAADB bounds the input uncertain database, \revb{albeit with reduced precision and no probabilities}. Alternatively, lenses~\cite{Yang:2015:LOA:2824032.2824055,BB19} can be used to directly generate \abbrUAADBs that encode the uncertainty introduced by data cleaning and curation heuristics.
We present translation schemes for \termTIs, \abbrXDBs, and \abbrVtable in \cite{techreport} and prove that they preserve bounds.
These schemes are trivial extensions of the schemes devised for \abbrUADBs presented in~\cite{FH19} and are omitted here.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> exp_figures_1.tex <==
% -*- root: uaadb.tex -*-
\begin{figure}[t]
  \centering
  \begin{minipage}{1.0\linewidth}
\begin{subfigure}[b]{.48\textwidth}
	\centering
  \includegraphics[width=1\linewidth, trim=0cm 0cm 3cm 0cm, clip]{uncert_Q0.pdf}
  \vspace*{-8mm}
  \bfcaption{vary uncertainty (1GB)}
  \label{fig:q1}
\end{subfigure}
\begin{subfigure}[b]{.48\textwidth}
	\centering
  \includegraphics[width=1\linewidth, trim=0cm 0cm 3cm 0cm, clip]{uncert_Q1.pdf}
  \vspace*{-8mm}
  \bfcaption{vary DB size (2\% uncertainty)}
  \label{fig:q2}
\end{subfigure}
\end{minipage}
  \caption{PDbench Queries}
  \label{fig:exp-pdbench}
\end{figure}

% \begin{figure*}[!ht]
%   \begin{minipage}{1.0\linewidth}
% \centering
% \begin{subfigure}[b]{.31\textwidth}
% 	\centering
%   \includegraphics[width=0.9\textwidth, trim=0cm 0cm 3cm 0cm, clip]{uncert_Q0.pdf}
%   \vspace*{-8mm}
%   \bfcaption{PDBench - Q1}
%   \label{fig:q1}
% \end{subfigure}
% \begin{subfigure}[b]{.31\textwidth}
% 	\centering
%   \includegraphics[width=0.9\textwidth, trim=0cm 0cm 3cm 0cm, clip]{uncert_Q1.pdf}
%   \vspace*{-8mm}
%   \bfcaption{PDBench - Q2}
%   \label{fig:q2}
% \end{subfigure}
% \begin{subfigure}[b]{.31\textwidth}
% 	\centering
%   \includegraphics[width=0.9\textwidth, trim=0cm 0cm 3cm 0cm, clip]{uncert_Q2.pdf}
%   \vspace*{-8mm}
%   \bfcaption{PDBench - Q3}
%   \label{fig:q3}
% \end{subfigure}
% \vspace*{-4mm}
% \bfcaption{Performance of PDBench queries -  varying the amount of uncertainty for scale factor 1}
% \label{fig:runtime_uncert}
% \end{minipage}

% \begin{minipage}{1.0\linewidth}
% \centering
% \begin{subfigure}[b]{.31\textwidth}
% 	\centering
%   \includegraphics[width=0.9\textwidth, trim=0cm 0cm 3cm 0cm, clip]{scale_Q0.pdf}
%   \vspace*{-8mm}
%   \bfcaption{PDBench - Q1}
%   \label{fig:q1d}
% \end{subfigure}
% \begin{subfigure}[b]{.31\textwidth}
% 	\centering
%   \includegraphics[width=0.9\textwidth, trim=0cm 0cm 3cm 0cm, clip]{scale_Q1.pdf}
%   \vspace*{-8mm}
%   \bfcaption{PDBench - Q2}
%   \label{fig:q2d}
% \end{subfigure}
% \begin{subfigure}[b]{.31\textwidth}
% 	\centering
%   \includegraphics[width=0.9\textwidth, trim=0cm 0cm 3cm 0cm, clip]{scale_Q2.pdf}
%   \vspace*{-8mm}
%   \bfcaption{PDBench - Q3}
%   \label{fig:q3d}
% \end{subfigure}
% \vspace*{-3mm}
% \bfcaption{PDBench queries -  varying database size for 2\% uncertainty}
% \label{fig:runtime_data}
% \end{minipage}
%\vspace{2mm}

% \begin{minipage}{1.0\linewidth}
% \centering


% \bfcaption{Microbenchmarks}
% \label{fig:microbench}
% \end{minipage}
% \vspace{2mm}
\end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> implementation.tex <==
%!TEX root=./uaadb.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation}
\label{sec:implementation}
We implement \abbrAUDBs as a middleware over conventional database systems.
For that, we define an encoding of $\uaaK{\semN}$-relations, denoted $\Enc$ (inverse $\Dec$), which maps a $\uaaK{\semN}$-database to a bag semantics database.
% $\Enc(\rangeRel)=R$ and $\Dec(R)=\rangeRel$ to denote the encoding and decoding of range relations
Using the encoding we apply query rewriting to propagate annotations and implement $\uaaK{\semN}$-relational query semantics over the encoding.  % while processing the query. We specifically implement \abbrAUDB for bag semantics, as this is the model used by most DBMSes.
Our frontend rewriting engine receives a query  $\query$ over an $\uaaK{\semN}$-annotated database $\rangeDB$ and rewrites this into a query $\qmerge$ that, when evaluated over $\Enc(\rangeDB)$, returns the encoding of $\query(\rangeDB)$. That is,
\begin{align*}
  \query(\rangeDB) = \Dec(\qmerge(\Enc(\rangeDB)))
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Relational encoding of \abbrAUDBs}
%
We use $\schemaOf(\rel)$ to denote the schema of input relation $\rel$.
The schema of $\Enc(\rangeRel)$ for an $\uaaN$-relation $\rangeRel$
with schema $\schemaOf(\rangeRel) = \tuple{a_1, \ldots, a_n}$ is
%
\[
  \schemasymb(\Enc(\rangeRel)) = \tuple{\bar{A},\ubMarker{\bar{A}},\lbMarker{\bar{A}}, \rlb, \ratt, \rub } \text{   where,}\\
\]\\[-8mm]
\[
  \bar{A}=\{\bgMarker{A_1}, \ldots, \bgMarker{A_n}\},\;
  \ubMarker{\bar{A}}=\{\ubMarker{A_1}, \ldots, \ubMarker{A_n}\},\;
  \lbMarker{\bar{A}}=\{\lbMarker{A_1}, \ldots, \lbMarker{A_n}\}
\]

For each tuple $\rangeTup$ with $\rangeRel(\rangeTup) \neq \uaaZero{\semN}$, there will be one tuple $\tup$ in $\Enc(\rangeRel)$. Attributes $\rlb$, $\ratt$, and $\rub$ are used to store $\rangeRel(\rangeTup)$:
\begin{align*}
  \tup.\rlb & = \lbMarker{\rangeRel(\rangeTup)}
& \tup.\ratt & = \bgMarker{\rangeRel(\rangeTup)}
& \tup.\rub & = \ubMarker{\rangeRel(\rangeTup)}
\end{align*}

For each attribute $A_i$, the three attributes $\lbMarker{A_i}$, $\bgMarker{A_i}$, and $\ubMarker{A_i}$ are used to store the range-annotated value $\rangeTup.A_i$:
\begin{align*}
  \lbMarker{A_i} & = \lbMarker{\rangeTup.A_i}
                 & \bgMarker{A_i} & = \bgMarker{\rangeTup.A_i}
                 & \ubMarker{A_i} & = \ubMarker{\rangeTup.A_i}
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Rewriting}
%
Queries are rewritten in two phases.
First, a function $\rewrUAA{\cdot}$ applies a naive rewriting that produces an encoding of the query result, but that may include duplicate records.
Second, an aggregation sums up the annotations of all such ``value-equivalent'' tuples in the naive result.
We use $\qmerge$ to denote the final rewrite of input query $\query$.
By allowing multiple value-equivalent tuples to be present in intermediate results, this two-phase approach avoids unnecessary intermediate aggregations for operators such as projection and union that may output value-equivalent tuples.
We present the detailed rewrite rules and prove their correctness in an accompanying technical report~\cite{techreport}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Theorem}% [Rewrite Correctness]
%   \label{theo:rewrite-correctness}
%   Let $\rangeDB$ be a $\uaaN$-relation, $\query$ be a query, then
%   \begin{align*}
%     \Dec(\Enc(\rangeDB)) &= \rangeDB \tag{$\Enc$ \textbf{is invertible}}\\
%   \qmerge(\Enc(\rangeDB)) &= \Enc(\query(\rangeDB)) \tag{$\rewrUAA{\cdot}$ \textbf{is correct}}
%   \end{align*}
% \end{Theorem}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}
% We prove the theorem by induction over the structure of queries demonstrating that the semantics of a rewritten operators aligns with our $\uaaN$-semantics. See~\cite{techreport} for the detailed proof.
% \end{proof}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Optimizations for Joins}
% \subsection{Optimizations for Joins}
One potential performance bottleneck of query evaluation over \abbrUAADBs is that equi-joins may degenerate into cross products if the bounds of join attribute values are loose. For example, if the join attribute bounds of every tuple from the LHS overlaps with the join attribute bounds of every tuple from the RHS.
We now develop an optimization for joins that splits each input relation $\rangeRel$ of the join into two parts: $\splitbg(\rangeRel)$ and $\splitpos(\rangeRel)$ as follows. If the equijoin is on attributes $\tuple{a_1, \ldots, a_n}$:
\begin{eqnarray*}
  \lbatt{\splitbg(\rangeRel)(\rangeTup)} &\defas&
    \begin{cases}
      \lbatt{\rangeRel(\rangeTup)} & \textbf{if } \forall i : \lbatt{\rangeTup.a_i} = \bgatt{\rangeTup.a_i} = \ubatt{\rangeTup.a_i} \\
      0 & \textbf{otherwise}
    \end{cases}
\\
  \bgatt{\splitbg(\rangeRel)(\rangeTup)} &\defas& \ubatt{\splitbg(\rangeRel)(\rangeTup)} \;\defas\; \bgatt{\rangeRel(\rangeTup)}
\\
\lbatt{\splitpos(\rangeRel)(\rangeTup)}  &\defas&  \bgatt{\splitpos(\rangeRel)(\rangeTup)}  \;\defas\; 0
\\
  \ubatt{\splitpos(\rangeRel)(\rangeTup)} &\defas& \ubatt{\rangeRel(\rangeTup)}
\end{eqnarray*}
This operation ensures (i) that any relation $\rel$ bound by $\rangeRel$ is also bound by both $\splitpos(\rangeRel)$ and $\splitbg(\rangeRel) \cup \splitpos(\rangeRel)$, (ii) that the join attributes of $\splitbg(\rangeRel)$ are all certain, and (iii) that $\bgatt{\splitbg(\rangeRel)} = \bgatt{\rangeRel}$.
Properties (i) and (iii) allow us to compute a bounding \abbrUAARel for the join $\rangeRel_1 \bowtie \rangeRel_2$ as\\[-3mm]
%
\[
      (\splitbg(\rangeRel_1) \bowtie \splitbg(\rangeRel_2) )
 \cup (\splitpos(\rangeRel_1) \bowtie \splitpos(\rangeRel_2))
\]
% \[
%       \left(\splitbg(\rangeRel_1) \bowtie \splitbg(\rangeRel_2) \right)
%  \cup \left(\splitpos(\rangeRel_1) \bowtie \splitpos(\rangeRel_2)\right)
% \]
Thanks to property (ii), the first join is a classical relational join and can be evaluated efficiently.
\revm{The latter join remains expensive, but tuples in this join can be compressed:
Based on a join compression size $n$ and join attribute $A$, we construct $n$ buckets $[\lbatt{b_i}, \ubatt{b_i}]$ over the domain of $A$ such that (i) for every tuple in $\rangeTup \in \splitpos(\rangeRel_i)$, there exists an $i$ such that $\lbatt{b_i} \leq \lbatt{\rangeTup.A} \leq \ubatt{\rangeTup.A} \leq \ubatt{b_i}$, and (ii) the number of tuples contained in this way by each bucket is roughly uniform.
The compressed $\splitpos(\rangeRel_i)$ relation has exactly $n$ tuples (one for each bucket) with attribute bounds that cover all tuples assigned to the bucket, lower and selected-guess multiplicities of 0, and an upper-bound multiplicity of the number of tuples assigned to the bucket.
For example, \Cref{fig:joinOptimization} shows the overlapping ranges of the join attributes of seven tuples ($a-g$).
To create a compressed representation of size 3 (i.e., $n = 3$), these tuples are partitioned into 3 roughly-equally-sized bins, and the resulting attribute bounds are selected as the maximum upper and lower bounds of the component tuples.
}
The compression size allows a trade-off between faster query evaluation and tighter % \emph{upper}
bounds.
We prove that the resulting join operation is correct in~\cite{techreport}.


\begin{figure}
\includegraphics[width=0.9\columnwidth]{figs/join_optimization.pdf}
\caption{\revm{An example of join compression with a compression size of 3: Tuples $a-g$ are compressed into bins $B_1 - B_3$.}}
\label{fig:joinOptimization}
\trimfigurespacing
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> introduction-Jan24-uarelations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{UA-relations}
\label{sec:ua-relations}


\mypar{Bag Semantics}
An important advantage of our approach is that it also supports bag semantics. This in particular is relevant if we apply UA-relations for an approach such as Mimir that introduces uncertainty as part of queries over deterministic data, because the input relation would be stored in a relational database which uses bag semantics.% , thus, may contain duplicates.
\BG{The previous sentence needs to be written better}. 

\begin{Example}\label{example:bag-UA-relation-UAA-relation}
  Reconsider possible worlds representation of the probabilistic database $\pdb$ from Figure~\ref{table:pdb} and uncertainty taint representation derived from $\pdb$ in Figure~\ref{table:example-UT}. Figure~\ref{table:example-UA} shows the UA-relation representation of the same uncertainty taint approach while adapting bag semantics where tuples are annotated by natural numbers recording the multiplicity of the tuple. In UA-relation, we use a pair of numbers to record the multiplicity of a tuple and multiplicity of certain respectively. i.e. (1,1) denotes the tuple repeats 0 times uncertain and 1 time certain. 
%  We further extend the UA-relation to UAA-relation that is shown in Figure~\ref{table:example-UAA}. An attribute value is marked certain if the value is the same in all possible worlds were the tuple exists. 
  We have developed a technique that uses conventional query processing to produce the UA-result for a query if applied to the UA-relational representation of a PDB without requiring conventional \abbrPQP to be applied. % as shown in Example~\ref{example:pqp}
\end{Example}



%As shown in Example~\ref{example:UT}, instead of using a full probabilistic database, we only consider the instance from the probabilistic database with the highest probability and mark tuples and attribute values as either certain or uncertain. Intuitively, a tuple is tainted as certain if the tuple exists in all instances of the probabilistic database and tainted as uncertain if the tuple only exists in some of the instances.


%An attribute in a tuple is tainted as certain if the value is the same in all instances of the probabilistic database where the tuple exists and tainted uncertain otherwise. 
Obviously, the UA-database corresponding to a possible world of a PDB does not retain all the information encoded by the PDB, e.g., the UA-database does not record probabilities and does not encode information about tuples that do not occur in the possible world the UA-database corresponds to.  However, the advantage of UA-relations is that query evaluation is significantly more efficient than query evaluation over probabilistic databases. We propose and implement a query rewriting approach that evaluates queries over UA-relations by propagating uncertainty taints. This approach has performance that is close to deterministic query processing. Herein lies the main advantage of UA-relations, as a non-destructive approximation of uncertainty that allows for fast query evaluation. Figure~\ref{fig:overview} shows an overview of our approach. We assume that probabilistic databases stores in some model are given. Alternatively, we can apply our approach in the context of a system like Mimir~\cite{Yang:2015:LOA:2824032.2824055} which introduces uncertainty on the fly. 
%\BG{explain correctness criteria.}

\begin{figure}[t]
  \centering
  \begin{subtable}{\linewidth}
  \centering
  \caption{$\pdb$ in uncertainty taint representation}
  \begin{tabular}{ |c|c|c|l }
        \cline{1-3}
    \textbf{name}  & \textbf{color}  & \textbf{category}  & \\
    \cline{1-3}
    apple & red & fruit & \tcMarker\\
        
    pear & yellow & fruit& \tcMarker\\
        
    carrot & red & vegetable& \tcMarker\\
        
    tomato & red & fruit& \tuMarker\\
        \cline{1-3}
  \end{tabular}
  \label{table:example-UT}
  \end{subtable}
  
  \begin{subtable}{\linewidth}
  \centering
  \caption{UA-relation bag representation}
  \begin{tabular}{ |c|c|c|l }
        \cline{1-3}
    \textbf{name}  & \textbf{color}  & \textbf{category}  & \\
    \cline{1-3}
    apple & red & fruit & (1,1)\\
        
    pear & yellow & fruit& (1,1)\\
        
    carrot & red & vegetable& (1,1)\\
        
    tomato & red & fruit& (1,0)\\
        \cline{1-3}
  \end{tabular}
  \label{table:example-UA}
  \end{subtable}
  
% \begin{subtable}{\linewidth}
% \centering
% \caption{UAA-relation bag representation}
% \begin{tabular}{ |c|c|c|l }
%       \cline{1-3}
%   \textbf{name}  & \textbf{color}  & \textbf{category}  & \\
%   \cline{1-3}
%   \cMarker{apple} & \cMarker{red} & \cMarker{fruit} & (1,1)\\
%       
%   \cMarker{pear} & \cMarker{yellow} & \cMarker{fruit} & (1,1)\\
%       
%   \cMarker{carrot} & \cMarker{red} & \cMarker{vegetable} & (1,1)\\
%       
%   \cMarker{tomato} & \cMarker{red} & \uMarker{fruit} & (1,1)\\
%       \cline{1-3}
% \end{tabular}
% \label{table:example-UAA}
% \end{subtable}
  
\caption{Uncertainty marker representation: use the possible world with the highest probability and mark attributes and tuples as either $T$=certain or $\redL{F}$=uncertain. For bag semantics representation, we annotate tuples with a pair of values representing the total multiplicity of the tuple and certain duplicates of this tuple, respectively.}
\label{table:UT-rep}
\end{figure}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \centering
  
% \begin{subtable}{\linewidth}
  \centering
% \caption{Query over bag UA-relation}
  \begin{tabular}{ |c|l }
        \cline{1-1}
    \textbf{category}  & \\
    \cline{1-1}
    fruit & (3,2)\\
                
    vegetable & (1,1)\\
    \cline{1-1}
  \end{tabular}
% \label{table:example-UA-res}
% \end{subtable}
  
% \begin{subtable}{\linewidth}
% \centering
% \caption{Query over bag UAA-relation}
% \begin{tabular}{ |c|l }
%       \cline{1-1}
%   \textbf{category}  & \\
%   \cline{1-1}
%   \cMarker{fruit} & (2,2)\\
%       
%   \cMarker{vegetable} & (1,1)\\
%       
%   \uMarker{fruit} & (1,1)\\
%       \cline{1-1}
% \end{tabular}
% \label{table:example-UAA-res}
% \end{subtable}
  \caption{Query evaluation over uncertainty-annotated relations}
  \label{fig:qp-over-ua-relations}
\end{figure}
%%%%%%%%%%%%%%%%%%%%

==> introduction-Jan24-uncertaintyannotations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Uncertainty Annotations}
\label{sec:uncertainty-labeling}
\BG{This subsection needs to be organized better. We need to explain separately set and bag semantics as well as UAA and we need examples for query evaluation.}
\BG{Maybe introduce uncertainty labelings first or not???}

In this paper, we study light-weight representations of uncertainty which enrich the data of one possible world from a probabilistic database with uncertainty information. Specifically, we study relations where tuples (and possibly attribute values) are annotated with uncertainty labels (certain or uncertain). Given a probabilistic database $\pdb$, we can derive an uncertainty-annotated database (\abbrUADB) by annotating the tuples in one possible world $\db \in \pdb$ (typically the possible world with the highest probability) with uncertainty labels. Given a \abbrUADB $\uadb$ for a possible world $\db$ of a \abbrPDB $\pdb$ we say the database is \textit{c-sound} if every tuple marked as certain is certain in $\pdb$. Similarly a $\uadb$ is called \textit{c-complete} if all certain tuples of $\pdb$ are marked as certain. Note that for most probabilistic data models it is trivial to derive a c-sound and c-complete UA-database.

The query semantics we define for \abbrUADBs is backward compatible to deterministic processing. That is, ignoring annotations, the result of a query over a \abbrUADB is the same as evaluating the same query over the possible world from which we have derived the \abbrUADB.
Furthermore,  the result of a query is c-sound as long as the input is c-sound, i.e., we never label a tuple as certain in a query result if the tuple is not a certain answer to the query according to the input \abbrPDB. However, query answers are only guaranteed to be c-complete for certain classes of queries. We argue that declaring an uncertain result as certain is more objectionable than declaring a certain result as uncertain. Thus, c-soundness is more important than c-completeness. \BG{remove that if we do not demonstrate it}
Note that given the complexity of exact \abbrCAQP we cannot hope for an efficient query evaluation algorithm that preserves both c-sound and c-complete. 
In summary, our approach combines the advantages of best guess query processing with approximation of certain answer semantics: 1) query evaluation is efficient and can be expressed in SQL, 2) all certain answers to the query will be returned, 3) the labelling of an answer determines whether the answer is certain or not. 

\begin{Example}\label{example:UT}
%\BG{say something about c-soundness/perservation}
  Reconsider the \abbrPDB from Figure~\ref{table:pdb}, Figure~\ref{table:example-UT} shows a set semantics uncertainty labeling derived from the running example possible world $\db_1$ (the possible world with the highest probability). Note that the labeling is c-sound (and c-complete) and we can always derive c-sound uncertainty taint from an instance of \abbrPDB  \BG{Give this relation a name for query evaluation}
To generate this representation, we annotate each tuple in the possible world as either certain ($\tcMarker$) or uncertain ($\tuMarker$). A row is marked certain if the row exists in all possible worlds of the probabilistic database and as uncertain otherwise. In this example, only the last tuple (red tomato) is uncertain and, thus, is annotated with $\tuMarker$. Now consider the evaluation of a query $\query_{cat} = \projection_{category}(\db)$ from Example~\ref{example:pqp} over this encoding. The results are shown in Figure~\ref{fig:qp-over-ua-relations}. Both result tuples are certain, since there exists a certain tuple with these category values.
\end{Example}


% The purpose of this exercise is to enable fast query evaluation over uncertain data which pairs the advantages of deterministic query processing (efficiency and ease of use) with certain answer semantics (

In this paper, we introduce UA-relations (Uncertainty Annotated-relations), relations where tuples are annotated with uncertainty taints. We employ UA-relations as a low-overhead representation of probabilistic data that allows queries to be evaluated efficiently. Given a probabilistic database $\pdb$, we can derive an UA-database by annotating the tuples in one possible world $\db \in \pdb$ (typically the possible world with the highest probability) with uncertainty taints that capture information about the presence of the tuple in $\pdb$. 
%To deal effectively with probabilistic data models that use attribute-level uncertainty (e.g., pc-tables), we extend UA-databases by also annotating attribute values with uncertainty taints - we call the resulting model \textit{UAA-relations} (Uncertainty Annotated Attribute databases).
We study query evaluation over such relations and demonstrate that two important correctness properties hold:
1) ignoring annotations, the result of a query over a UA-relation is the same as evaluating the same query over the possible world from which we have created the UA-relation and 2) we never label a tuple as certain in a query result if the tuple is not a certain answer to the query according to the input \abbrPDB. \BG{The result is that we get the best of both worlds: deterministic query evaluation, but still keeping important uncertainty information}




When evaluating queries over a possible world annotated with uncertainty labels, we expect the query results to be annotated in a way that is consistent with the result of the conventional query processing without labeling and the labeling can provide extra uncertainty information to the user.

==> labelschemes.tex <==
\input{introduction-Jan24-uncertaintyannotations.tex}


Recall that our goal is to annotate tuples from one possible world with uncertainty information and then design a query semantics over such annotated data which propagates uncertainty in a way that is compatible with possible world query semantics. For this we define a class of semirings whose elements are pairs of values from $\kDom$, i.e., elements from $\dpK{\semK}{2}$. Such a pair $(d,c)$ will be used to record the annotation $d$ that the tuple carries in the possible world as well as the part $c$ of the annotation  that is certain.  Given an annotation $k = (d,c)$ we define:

\begin{align}
  \cOf{k} &= c & \dOf{k} &= d
\end{align}
%$\cOf{k} = c$ and $\uOf{k} = u$.

% \begin{Definition}[Uncertainty Label Semirings]
% For any a m-semiring  $\semK$, we define a semiring $\uK = (\uKDom, \addOf{\uK}, \multOf{\uK}, \zeroOf{\uK}, \oneOf{\uK})$ where $\uKDom = \kDom^2$ and the operations are defined pointwise based on the corresponding operations for $\pwK$.
% \end{Definition}

We now define uncertainty labelings of a possible world $\db$ as $\dpK{\semK}{2}$-databases where the $\dOf{k}$ component of a tuple $\tup$'s annotation is equal to $\db(\tup)$.  % that replace the annotations in a possible world with annotations from $\uK$.

\section{Uncertainty Labelings}
\label{sec:uncert-labell}
\BG{We need examples in this section, probably more clear explanations, definition for bag AUL needs to be checked for correctness. Also the macros $\backslash TUL$ and $\backslash AUL$ are ugly, let's come up with a better notation}
We now introduce labeling schemes that enrich a possible world from a probabilistic database with uncertainty information by annotating tuples (and potentially also attribute values) as either certain or uncertain. We then proceed to define intuitive correctness criteria for such labelings. We define labeling over probabilistic databases for both set and bag semantics. For instance, we should not label tuples as certain that are not certain in the probabilistic database from which the labeling stems from. To be able to label attribute values we start by introduce domains of values that are either labeled as certain ($\tcMarker$) or uncertain ($\tuMarker$). Furthermore, we define matching of tuples with such values, a relaxed version of equality which ignore uncertain attribute values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Labeled Domain and Tuple Matching]
  Consider a universal domain $\aDom$ of values. Given a set of uncertainty labels $\uLabels = \{\tcMarker, \tuMarker\}$, we define $\uDom = \{ d^{l} \mid l \in \uLabels \wedge d \in \aDom\}$, the labeled version of $\aDom$. Given a labeled value $d^{l}$ we define an operator $\labelOf$ the extracts the label from the value: $\labelOf(d^{l}) = l$.   Given a tuple $\tup = (\aVal_1, \ldots, \aVal_n)$ and $\tup_{\uLabels} = (e_1, \ldots, e_n)$ such that $\aVal_i \in \aDom$ and $e_i \in \uDom$ we say $t$ matches $\tup_{\uLabels}$, written as $\tup \tmatches \tup_{\uLabels}$ if for all $i \in \{1, \ldots,n\}$ either $\labelOf(e_i) = \tuMarker$ or $\aVal_i = e_i$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For instance, a tuple $(1,3)$ would match a tuple $(\uMarker{2}, \cMarker{3})$, but not a tuple $(\cMarker{2}, \uMarker{3})$. Given a relation $\rel$ we define $\ltupDom(\rel)$ the set of labeled tuples with the same schema as $\rel$ ($\ltupDom(\db)$ is defined analog).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{General Correctness Criteria for UAA-relations}
Depending on the attribute level uncertainty representation. Tuple equivalence between a labeled tuple $\tup_l$ and a tuple $\tup$ can be individually defined:
\[
	\tup_l \tmatches \tup \Leftrightarrow \begin{cases}
	\tup.A=\tup_l.A \vee \AUL(\tup_l.A)=u, & \text{if} \; u/c\\
    \tup.A=\tup_l.A \vee \tup.A \intersection \AUL(\tup_l.A), & \text{if} \; range
	\end{cases}
 \]

A global matching GM maps a labeled tuple $\tup_l$ from $\db_l$ with a tuple $\tup$ from $\db$ to a semiring element $k$.
\[GM(\tup_l,\db_l,\tup,\db,\pdb)=k \; s.t. \; \tup_l \in \db_l \wedge \tup \in \db \wedge \db \in \pdb\ \wedge \tup_l \tmatches \tup\]
For a specific labeled database $\db_l$ and a set of possible worlds $\pdb$, all tuples in the $\db_l$ need to matched.
\[ \forall_{\db \in \pdb}: \forall_{\tup_l \in \db_l}: \TUL(\tup_l)=\sum_{\tup \in \db}GM(\tup_l,\db_l,\tup,\db,\pdb) \]
Then we define c-soundness and c-completeness of $\db_l$ on $\pdb$:
c-sound iff:
\[\exists_{GM} \; s.t. \; \forall_{\db \in \pdb}: \forall_{\tup \in \db}: \db(\tup) \succeq_{\semK} \sum_{\tup_l \in \db_l}GM(\tup_l,\db_l,\tup,\db,\pdb)\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Set Semantics Labelings}
\label{sec:set-semant-labell}

We define tuple and attribute-level uncertainty labelings. Tuple labelings are simplify functions that map every tuple from a $\tupDom(\db)$ to a value from $\uLabels$ or the special value $\notHere$ to indicate that the tuple does not belong to $\db$. While we could alternatively just map tuples from $\db$ instead of using $\tupDom(\db)$ and the additional label $\notHere$, using total functions enables us to define sets and bags in an analog fashion.
For attribute-level uncertainty labelings, we define labeled versions of databases and relations where each attribute value is marked as either certain or uncertain.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Attribute-labeled Database]
%   Consider a database $\db$ over a domain $\aDom$. We say a database $\ldb$ over $\uDom$ with the same schema s $\db$ is an attribute-labeling of $\db$ iff the condition shown below holds. We define labelings of relations in the same fashion.
%   \begin{align*}
%     \forall \tup \in \db: \exists \tup' \in \ldb: \tup \tmatches \tup' \wedge (\forall \tup'' \in \ldb: \tup \tmatches \tup'' \rightarrow \tup' = \tup'')\\
%     \forall \tup \in \ldb: \exists \tup' \in \db: \tup' \tmatches \tup \wedge (\forall \tup'' \in \db: \tup'' \tmatches \tup' \rightarrow \tup' = \tup'')
%   \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Uncertainty Labeling]
  Let $\pdb$ be a probabilistic database and $\db$ one of its possible worlds. A tuple uncertainty labeling $\TUL$ for the pair $(\pdb,\db)$ is a function from $\tupDom(\db)$ to $\{ \tcMarker, \tuMarker, \notHere \}$ such that for all $\tup \in \tupDom(\db)$ we have $\TUL(\tup) = \notHere \Leftrightarrow \tup \not\in \db$. An attribute uncertainty labeling  $\AUL$ for the pair $(\pdb,\db)$ is a function $\ltupDom(\db) \mapsto \{\tcMarker, \tuMarker, \notHere \}$ such that:
  \begin{itemize}
  \item $\forall \tup \in \tupDom(\db): t \in \db \Leftrightarrow \exists \tup' \in \ltupDom(\db): \tup \tmatches \tup' \wedge \AUL(\tup') \neq \notHere$
   \item $\not\exists \tup \in \tupDom(\db), \tup_1, \tup_2 \in \ltupDom(\db): \tup \tmatches \tup_1 \wedge \tup \tmatches \tup_2 \wedge \AUL(\tup_1) \neq \notHere \wedge \AUL(\tup_2) \neq \notHere$
  \end{itemize}
  % \begin{align}
  %   \forall \tup \in \db: \exists \tup' \in \ltupDom(\db): \tup \tmatches \tup' \wedge \AUL(\tup') \neq \notHere \wedge (\forall \tup'' \in \ltupDom(\db): \AUL(\tup'') = \notHere \vee (\tup \tmatches \tup'' \rightarrow \tup' = \tup''))\\
  %   \forall \tup \in \ldb: \exists \tup' \in \db: \tup' \tmatches \tup \wedge (\forall \tup'' \in \db: \tup'' \tmatches \tup' \rightarrow \tup' = \tup'')
  % \end{align}
  % a tuple labeling $\TUL$ for $(\pdb, \db)$ and a function $\AUL$ from each attribute value (pair of tuple and attribute) to $\{ \tcMarker, \utMarker \}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Intuitively, the definition of attribute labelings ensures that only one labeled version of each tuple in $\db$ is mapped to a label different from $\notHere$. Furthermore, only labeled versions of tuples which do not exist have to be mapped to $\notHere$. Note that an attribute labeling maps each tuple $\tup \in \db$ to exactly one labeled tuple, the only labeled version of $\tup$ which is not mapped to $\notHere$. In the following use $\tup_{\AUL}$ to denote the labeled tuple assigned to
$\tup$ by an attribute uncertainty labeling $\AUL$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
  Reconsider

  \BG{Reexplain (part of) an intro example given the formalism}
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness Criteria for Set Labelings}
\label{sec:corr-crit-sets}

Of course, a labeling should assign the $\tcMarker$ and $\tuMarker$ annotations in a way that is coherent with the input probabilistic database $\pdb$. Ideally, a tuple uncertainty labeling (TUL) should assign the $\tcMarker$ label only to tuples that are certain (exist in all possible worlds of $\pdb$) and assigns the $\tuMarker$ label to all other tuples. However, as we will see there is a trade-off between the computational complexity of generating such a labeling and maintaining it under queries and fulfilling this correctness criterion. Thus, we also introduce less strict correctness criteria so as not to sacrifice efficiency. For an attribute uncertainty labeling, we have to define what we mean by a tuple $\tup$ with  uncertain attribute values to occur in a possible world since the tuple may have different values in different possible worlds.
\BG{needs examples}
% For that we define tuple matchings. For an AUL $\AUL$ for $(\pdb,\db)$, a labeled tuple $\tup_l$ matches a tuple $\tup$ from a possible $\db \in \pdb$, written as $\tup_l \tmatches \tup$, if $\tup$ agrees with $\tup_l$ on all certain attribute values (where $\AUL(\tup_l, A)= \tcMarker$).
\BG{Discuss why c-soundness is more critical then c-completeness (either here or already in intro}
\BG{@move this to related work? Explain relationship to m-tables labelings to make clear the relationship and distinction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[C-soundness and C-completeness]
  Let $\pdb$ be a probabilistic database and $\db$ one of its possible worlds. A TUL $\TUL$ is
  \begin{itemize}
  \item \textbf{c-sound} if $\forall \tup \in \db: \TUL(\tup) = \tcMarker \Rightarrow \tup \in \cSet(\pdb)$
  \item \textbf{c-complete} if $\forall \tup \in \db: \tup \in \cSet(\pdb) \Rightarrow \TUL(\tup) = \tcMarker$
  \end{itemize}
  Analog, an AUL $\AUL$ is

  \begin{itemize}
  \item \textbf{c-sound} if
    $\forall \tup \in \db: \TUL(\tup) = \tcMarker \Rightarrow \forall \db' \in
    \pdb: \exists \tup' \in \db': \tup \tmatches \tup'$

    \item   \textbf{c-complete} if $\forall \db' \in \pdb: \exists \tup' \in \db': \tup \tmatches \tup' \Rightarrow \TUL(\tup) = \tcMarker$

\end{itemize}

\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BG{define tuple matching between two labeled tuples too, so far does not look like we need that.}

Additionally, since we want to be able to evaluate queries over a labeling we have to require that (1) ignoring labels, queries behave exactly like deterministic queries over $\db$ and (2) that queries preserve the correctness of a labeling. For instance, if the labeled input of a query $\query$ is both c-sound and c-complete, then the output query $\query$ evaluated over this input should be c-sound and c-complete wrt. the full probabilistic query result ($\query(\pdb)$). We call this property preservation of c-soundness/c-completeness under queries.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Preservation of Correctness under Queries]
Let $\TUL$ be a c-sound/c-complete TUL for $(\pdb,\db)$ and $\query$ a query from a class of queries $\qClass$. A semantics for evaluating queries over labeling is said to preserve c-soundness/c-completeness if for $\query(\TUL)$ is a c-sound/c-complete labeling for $(\query(\pdb), \query(\db))$. The definition of AUL is analog.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that if a query semantics for a labeling scheme preserves both c-soundness and c-completeness, then it follows that it behaves like deterministic query evaluation for deterministic inputs (a PDB with one possible world). However, since the UA- and UAA-relations we introduce are only c-sound for some classes of queries, we are interested in this additional correctness criteria which we will refer to as \textit{backward compatibility} (with deterministic query semantics).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bag Semantics Labelings}
\label{sec:bag-semant-label}



Furthermore, since we also target bag semantics, we extend the notions of a tuple uncertainty labeling and attribute uncertainty labeling as well as correctness criteria for bag instances.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Bag Labeling]
  Given a probabilistic database $\pdb$ with bag semantics and one of its possible worlds $\db$, a TUL $\TUL$ for $(\pdb, \db)$ is a function that assigns to each tuple $\tup \in \db$ a pair of natural numbers $(u,c) \in \semN \times \semN$ with $|(u,c)| = u + c = \db(\tup)$. Given a tuple $\tup = (a_1, \ldots, a_n)$, a labeled version of tuple $\tup$ is a tuple $\tup_l = ({a_1}^{l_1}, \ldots, {a_n}^{l_n})$ where each $l_i \in \{\tcMarker, \tuMarker\}$.
  An AUL for $(\pdb,\db)$ is a function whose input is the set of all labeled tuples for tuples from $\db$ and whose domain is $\semN \times \semN$. Note that AUL may split $\tup$ into set of $\tup_l$s as $S$ such that $\db(t) = \sum_{\tup_l \in S}|TUL(\tup_l)|$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BG{Do we have a better way of defining bag AULs?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness Criteria for Bag Labelings}
\label{sec:corr-crit-sets}


The pair of natural numbers $(u,c)$ assigned by a bag TUL to a tuple denotes the tuple's certain and uncertain multiplicity. That is, $u + c$ is the multiplicity of $\tup$ in $\db$ and ideally $c = \cMult(\pdb,\tup)$. For a bag AUL, multiple annotated we record certain and uncertain multiplicities for each possible combination of attribute labels for a tuple. Based on these versions of TULs and AULs for bag semantics PDBs, we now define c-soundness and c-correctness (preservation of correctness is the same for set and bag semantics).
To define these properties for bag AULs, we define a global tuples matching function $GM$ maps a triple of the form $(\tup_l,\db,\tup)$ to a natural number $n$ where $\db \in \pdb$ and $\tup \in \db$ and $\tup_l \tmatches \tup$ and $\tup_l \in \db_l$. Here $\db_l$ denotes the group of all labeled tuples. The function means a labeled tuple $\tup_l$ is matched to $n$ multiplicities of tuples $\tup \in D$. For a global tuple matching $GM$, define restrictions:
$$\forall \db \in \pdb: \forall \tup \in \db: \db(t) \geq \sum_{\tup_l \in \db_l}GM(\tup_l,\db,\tup) $$
$$\forall \db \in \pdb: \forall \tup_l \in D_l: |TUL(\tup_l)| \geq \sum_{\tup \in \db}GM(\tup_l,\db,\tup) $$
The first restriction enforces that each duplicate of tuple $\tup$ can match to at most one labeled tuple $\tup_l$. The second restriction enforces that a labeled tuple can not match to number of tuples more than its own multiplicity. Then we extend $\cMult$ to take matching into account:
\begin{align}
	\cMatches(GM,\pdb,\tup_l)=\min_{\db \in \pdb}(\sum_{\tup \in \db}GM(\tup_l,\db,\tup))
\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}
  Let $\pdb$ be a bag probabilistic database and $\db$ one of its possible worlds. Let $\TUL(\tup) = (u,c)$. We use $c_\tup$ denote $c$ for a given tuple $\tup$. A TUL $\TUL$ is
  \begin{itemize}
  \item \textbf{c-sound} if $\forall \tup \in \db: c_\tup \leq \cMult(\pdb, \tup)$
  \item \textbf{c-complete} if $\forall \tup \in \db: c_\tup \geq \cMult(\pdb, \tup)$
  \end{itemize}
  Analog, an AUL $(\TUL,\AUL)$ is

  \begin{itemize}
  \item \textbf{c-sound} if \\
    $\exists GM: \forall \tup \in \db: c_t \leq \cMatches(GM,\pdb,\tup) $
  \item   \textbf{c-complete} if \\
  	$\exists GM: \forall \tup \in \db: c_t \geq \cMatches(GM,\pdb,\tup) $
    \end{itemize}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{Example} \label{example:labeltup}
Consider a c-sound UA-relation tuple (apple,red,fruit) with annotation $(1,2)$. The annotation indicates there are three duplicate tuples in the single possible world we labeling on, and all possible worlds have at least one instance of this tuple. Consider a c-sound UAA-relation tuple (\cMarker{apple},\uMarker{red},\cMarker{fruit}) with annotation $(1,2)$. The annotation indicates there are three duplicate tuples of (apple,red,fruit) in the single possible world we are labeling on, and all possible worlds have at least one instance of the tuple, each of which can uniquely match to (apple,*,fruit), where * can be any value.
%  \BG{Show for a single tuple some labeled tuples with different multiplicities and discuss what this means.}
\end{Example}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> querysem.tex <==
\section{Query Semantics}
\label{sec:rules}
\SF{Updated}
\BG{This needs more context in the beginning to make clear the connection and difference with K-relational query semantics}

In this section, We introduce propagation and rewriting rules on top of the uncertainty model in both tuple and attribute levels. We start with applying our annotation semiring $K_{uncert}$ to standard K-relation querying semantics on applicable relational algebra operators. Then we extend the querying semantics to UAA-relations where, different from the traditional K-relations model, attribute level annotations and row level annotations are both involved. At last we state some non-monotone relational algebra operators that can not be properly defined by K-relational models and discuss how to properly query over them while preserving c-soundness. Let $rowD(Q,t,I)$ denote the row determinism for tuple $t$ in the result of query $Q$ over database instance $I$. Let $attrD(Q,t,A,I)$ denote the determinism for attribute $A$ of tuple $t$ in the result of query $Q$ over instance $I$.
%Let $exprD(t,E)$ denote the determinism for expression $E$ of tuple $t$. If a row is marked as certain then it belongs to the set of certain answers which also called c-sound. If it is marked uncertain then it may belong to the set of certain answers or may be uncertain which means c-completeness is not guaranteed.%


\subsection{UAA-relation query semantics}
UAA-relations maintain similar querying semantics on projection, cross product and union operations. For positive queries, attribute level uncertainty is maintained in the output because the uncertainty is embedded in the universe itself. So the attribute determinism is trivially $attrD(Q,t,A,I)=det(t.A)$. For selection and join operation with clauses, attribute level annotations may propagate to row level annotations. In this case, we may need to map attribute level determinism to row level annotation structure because such query operators determine row based on attribute values. Define transfer to be a function that transfers a boolean expression $\theta$ into row level annotations:
\[
trans(\theta(t))=\begin{cases}
    (0,1), & \text{if } [[\theta((t))]]=T^T\\
    (1,0), & \text{if } [[\theta((t))]]=T^F\\
    (0,0), & \text{else}
\end{cases}
\]

Then specify modified selection and join querying semantics as:
\begin{enumerate}

\item selection
\[rowD(\selection_\theta(Q),t,I)=rowD(Q,t,I) \otimes trans(\theta(t))\]

\item join
\begin{align*}
	rowD(Q_1 & \join_\theta Q_2,t,I) \\
	=&rowD(Q_1,t,I) \otimes rowD(Q_2,t,I) \otimes trans(\theta(t))
\end{align*}

\end{enumerate}

Join and selection involves row level uncertainty affected by attribute level uncertainty using  function $trans()$ which transfers an annotated expression evaluation result into row level taint structure. Projection may involving grouping of same tuples leading to an addition operation similar to union. Example \ref{example:attr-full} shows a fully annotated database instance and the step-by-step propagated result by the propagation rules.


\begin{Example}
	Figure~\ref{table:4.full} shows a full detailed example by executing query \\
	$\projection_{color}(\selection_{color='red'}(food \join_{category=pref} preference))$ over a UAA-relation instance \textsf(food) and \textsf(preference). First join operator outputs first and third tuple with row annotations $(1,3) \otimes (0,2)=(2,6)$ and $(2,1) \otimes (0,2)=(4,2)$ respectively. Second tuple row level annotation is calculated as $(0,2)\otimes(1,1)\otimes(1,0)=(4,0)$ since $ [[vegetable^T=vegetable^F]]=T^F $. Second operator as selection only changes row annotation of third tuple into $(4,2)\otimes(1,0)=(6,0)$ since $ [[red^F=[['red']]]]=[[red^F=red^T]]=T^F $. Third operator as projection sums up identical tuples giving second result tuple row annotation to be $(4,0)\oplus(6,0)=(10,0)$.
\label{example:attr-full}
\end{Example}

\begin{figure}[ht]
	\centering
	\begin{subtable}{\linewidth}
	\centering
	\caption{Tainted input table: \textsf{food}}
	\begin{tabular}{ |c|c|c|l}
				\cline{1-3}
		\textbf{name}  & \textbf{color}  & \textbf{category}   & \\
		\cline{1-3}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} & (1,3)\\
%				\cline{1-3}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} & (0,2)\\
%				\cline{1-3}
		\cMarker{apple} & \uMarker{red} & \cMarker{fruit} & (2,1)\\
				\cline{1-3}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Tainted input table: \textsf{preference}}
	\begin{tabular}{ |c|c|l}
				\cline{1-2}
		\textbf{group}  & \textbf{pref}   & \\
		\cline{1-2}
		\cMarker{child} & \cMarker{fruit} & (0,2)\\
%				\cline{1-2}
		\cMarker{adult} & \uMarker{vegetable} & (1,1)\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Join result}
	\begin{tabular}{ |c|c|c|c|c|l}
				\cline{1-5}
		\textbf{name}  & \textbf{color}  & \textbf{category} & \textbf{group}  & \textbf{pref}  & \\
		\cline{1-5}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (2,6)\\
%				\cline{1-5}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} & \cMarker{adult} & \uMarker{vegetable} & (4,0)\\
%				\cline{1-5}
		\cMarker{tomato} & \uMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (4,2)\\
				\cline{1-5}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Selection result}
	\begin{tabular}{ |c|c|c|c|c|l}
				\cline{1-5}
		\textbf{name}  & \textbf{color}  & \textbf{category} & \textbf{group} & \textbf{pref}  & \\
		\cline{1-5}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (2,6)\\
%				\cline{1-5}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} & \cMarker{adult} & \uMarker{vegetable} & (4,0)\\
%				\cline{1-5}
		\cMarker{tomato} & \uMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (6,0)\\
				\cline{1-5}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{final result after projection}
	\begin{tabular}{ |c|l}
				\cline{1-1}
		\textbf{color}  &\\
		\cline{1-1}
		\cMarker{red} & (2,6)\\
%				\cline{1-1}
		\uMarker{red} & (10,0)\\
				\cline{1-1}
	\end{tabular}
	\end{subtable}

\caption{A query execution with annotation propagation example on UAA-relation. (a)-(b) are input tables. (c)-(e) are intermediate and final output results.(current rule is not c-sound in case of multiple group by attributes)}
\label{table:4.full}
\end{figure}

\subsection{Non-monotone Queries}
There are several relational algebra operators involving negative operations which are not directly defined by our semiring model. Since we only propagating one possible world from the probabilistic database, in general cases input tuples may be filtered out un-deterministically by operations like selection over attributes containing uncertain data. Which means some tuples exist in partial worlds of conventional probabilistic query processing may missing in result of our model. For the current implementation, we are tainting all affected fields to uncertain to preserve c-sound property. We need to redefine grouping mechanism in aggregation operator for our model to work under the promise as well.\\
For the query evaluation for aggregation, we need to change grouping mechanism so that tuples are not grouped by their value in $\mathcal(U)^+$, but are grouped by the non-annotated value $val(v)$. i.e. for an input instance $R$ to the aggregation operator, we evaluate the value output for aggregation by first strip off all attribute level annotations. Then we reassign annotations to the output. Define function $strip_{all}(R)= \forall_{t \in R} : strip(t)$, Aggregation operator evaluation scheme is: $[[_g\gamma_F(R)]]=_g\gamma_F(strip_{all}(R))$. \\
Define function that map an annotation $(u,c)$ to its unit form as:
\[unit(u,c)=\begin{cases}
	(0,1), & \text{if } c>0 \\
	(1,0), & \text{if } c=0 \text{ and } u>0 \\
	(0,0), & \text{else}
\end{cases}
\]
Row level propagation rule is defined as:
\[rowD(_g\gamma_F(Q),t,I) = unit(\sum_{t'.g=t.g}rowD(Q,t',I))\]
Attribute level annotations for group by attributes are picked from one of the tuples $t'$ from the group where $rowD(_g\gamma_F(Q),t,I)=unit(rowD(Q,t',I))$. The naive heuristic is to pick a tuple with most number of certain group by attributes. Without completeness information, aggregation result attributes are annotated as uncertain so that the property of c-soundness holds in aggregation operators.\\
A similar situation happens with the set difference operator where we need to set all output row level determinism to uncertain since we do not know if the input is complete. One way to optimize this issue and potentially produce less conservative results by sacrificing performance, propagating extra information in the rewriting which recording whether the input of an operator contains tuples that are conditionally eliminated (p-completeness).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> range.tex <==
\section{UAA-realtion with range}
\label{sec:range}
In this section we introduce a more informative model on top of attribute uncertainty annotated database.
\subsection{Range annotated PDBs}
We consider the domain of real numbers and boolean values. In case of boolean values, the range can be either certain: $(F,F)$, $(T,T)$ or uncertain: $(F,T)$ assuming $F < T$. For an attribute $x$, we use $\ubMarker{x}$ to denote the upper bond of $x$ and $\lbMarker{x}$ to denote the lower bond of $x$. An attribute interval is a range $I_A=[\lbMarker{A},\ubMarker{A}]$ A range annotated relation $R$ is a relation s.t. each tuple is annotated by a tuple $R(t)=(k_c, k_b, k_p, I_{A1}, I_{A2},...,I_{An})$ where $k_c$ is the certain labeling, $k_b$ is the best guess labeling, $k_p$ is the possible labeling and $I_{A1}, I_{A2},...,I_{An}$ are the attribute ranges for each attribute.
\subsection{Tuple matching}
Define matching $t' \tmatches t$ as true iff $\forall{i \in [1,n]}:t(a_i) \in I_{t'(a_i)}$ \\
A tuple matching $TM(R',R,t',t)=k$ is the mappings from an annotated tuple $R'(t')$ and a possible world tuple $R(t)$ to a semiring value $k$. \\
As a constrain, any tuple matching need to fully match all certain tuples from annotated relation:
$$\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t)=R'(t').k_c$$
A annotated relation $R'$ is c-sound if:
$$\forall_{D(R) \in \mathbb{D}}:\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \leq R(t)$$
A annotated relation $R'$ is p-complete if:
$$\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t)=R'(t').k_p$$
$$\forall_{D(R) \in \mathbb{D}}:\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \geq R(t)$$

%%%
%\subsection{Certain tuples based tuple matching}
%In certain tuples based tuple matching, we match annotated tuples to certain tuples in all possible worlds.\\
%An annotated relation $R'$ is c-sound if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \leq certain(\mathbb{D})(t)$$
%A annotated relation $R'$ is c-complete if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \geq certain(\mathbb{D})(t)$$
%%%

%\subsection{Expressions}
%An attribute $x$ is certain iff the upper bound and lower bound of the attribute are equal.
%Comparison and boolean operators can be defined as:
%\begin{enumerate}
%\item \[ \begin{cases}
%\ubMarker{(a>b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \\
%\ubMarker{(a>b)} = F & \text{else}
%\end{cases}
%\]
%\[ \begin{cases}
%\lbMarker{(a>b)} = T & \text{if } \lbMarker{a}>\ubMarker{b} \\
%\lbMarker{(a>b)} = F & \text{else}
%\end{cases}
%\]
%\item \[ \begin{cases}
%\ubMarker{(a=b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
%\ubMarker{(a=b)} = F & \text{else}
%\end{cases}
%\]
%\[
%\begin{cases}
%\lbMarker{(a=b)} = T & \text{if } \ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} \\
%\lbMarker{(a=b)} = F & \text{else}
%\end{cases}
%\]
%\item \[ \ubMarker{(p \wedge q)} = \ubMarker{p} \wedge \ubMarker{q} \]
%\[ \lbMarker{(p \wedge q)} = \lbMarker{p} \wedge \lbMarker{q} \]
%\item \[ \ubMarker{(p \vee q)} = \ubMarker{p} \vee \ubMarker{q} \]
%\[ \lbMarker{(p \vee q)} = \lbMarker{p} \vee \lbMarker{q} \]
%\end{enumerate}


\subsection{Expressions}
An attribute $x$ is certain iff the upper bound and lower bound of the attribute are equal.
Comparison and boolean operators can be defined as:
\begin{enumerate}

\item \[\ubMarker{(a>b)} = \ubMarker{a}>\lbMarker{b}\] \\
\[\lbMarker{(a>b)} = \lbMarker{a}>\ubMarker{b}\]


\item \[\ubMarker{(a=b)} = \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b}\] \\

\[\lbMarker{(a=b)} = (\ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} )\] \\

\item \[ \ubMarker{(p \wedge q)} = \ubMarker{p} \wedge \ubMarker{q} \]
\[ \lbMarker{(p \wedge q)} = \lbMarker{p} \wedge \lbMarker{q} \]
\item \[ \ubMarker{(p \vee q)} = \ubMarker{p} \vee \ubMarker{q} \]
\[ \lbMarker{(p \vee q)} = \lbMarker{p} \vee \lbMarker{q} \]
\end{enumerate}
For projection expressions $a$ and $b$, we define result annotation of each operators:
\begin{enumerate}
	\item $ \ubMarker{(a+b)} = \ubMarker{a} + \ubMarker{b} $ \\
	$ \lbMarker{(a+b)} = \lbMarker{a} + \lbMarker{b} $
    \item $ \ubMarker{(a-b)} = \ubMarker{a} - \lbMarker{b} $ \\
	$ \lbMarker{(a-b)} = \lbMarker{a} - \ubMarker{b} $
	\item $ \ubMarker{(a \cdot b)} = max(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b}) $ \\
	$ \lbMarker{(a \cdot b)} = min(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b}) $
	\item $x \leftarrow \text{if } e \text{ then } a \text{ else } b$
	\[ \begin{cases}
\ubMarker{x} = \ubMarker{a},\lbMarker{x} = \lbMarker{a} & \text{if } \ubMarker{e}=T \wedge \lbMarker{e}=T \\
\ubMarker{x} = \ubMarker{b},\lbMarker{x} = \lbMarker{b} & \text{if } \ubMarker{e}=F \wedge \lbMarker{e}=F \\
\ubMarker{x} = max(\ubMarker{a},\ubMarker{b}),\lbMarker{x} = min(\lbMarker{a},\lbMarker{b}) & \text{else}
\end{cases}
\]
\end{enumerate}

\subsection{Query semantics}
We annotate each tuple $t$ using upper and lower bounds $\ubMarker{t}$ and $\lbMarker{t}$.

\subsubsection{Row bounds}

\begin{enumerate}
\item selection
\[LB([\selection_\theta(R)](t)=LB(R(t)) \otimes \lbMarker{(\theta(t))} \]
\[UB([\selection_\theta(R)](t)=UB(R(t)) \otimes \ubMarker{(\theta(t))} \]

\item join
\[ LB([R_1 \join R_2](t)) = LB(R_1(t)) \otimes LB(R_2(t)) \]
\[ UB([R_1 \join R_2](t)) = UB(R_1(t)) \otimes UB(R_2(t)) \]

\item Union
\[ LB([R_1 \union R_2](t)) =
	LB(R_1(t)) \oplus  LB(R_2(t))\]
\[ UB([R_1 \union R_2](t)) = UB(R_1(t)) \oplus UB(R_2(t)) \]

\item Projection
\[ LB([\projection_{U}(R)](t)) = \sum_{t=t'[U]}LB(R(t')) \]
\[ UB([\projection_{U}(R)](t)) = \sum_{t=t'[U]}UB(R(t')) \]

\item Set difference
\[ LB[R_1 - R_2](t) = \{LB(R_1(t))-\sum_{R_1(t) \matches R_2(t')} UB(R_2(t'))\}^+ \]
\[ UB[R_1 - R_2](t) = \{UB(R_1(t))-\sum_{R_1(t) \equiv R_2(t')} LB(R_2(t'))\}^+ \]



%\item Sum Aggregation with group by
%\[ [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{sum(A)} = \sum_{t' \in R, t[g] \in t'[g]}LB(R(t'))*R(t').\lbMarker{A} \]
%\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]

\end{enumerate}

\subsubsection{Attribute bound}
\begin{enumerate}

\item Union
\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\lbMarker{a_i} = \min(R_1(t).\lbMarker{a_i},R_2(t).\lbMarker{a_i}) \]
\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\ubMarker{a_i} = \max(R_1(t).\ubMarker{a_i},R_2(t).\ubMarker{a_i}) \]

\item Projection
\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]
\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\ubMarker{a_i} = \max_{t=t'[U]} R(t').\ubMarker{a_i} \]

\item Count Aggregation without group by
\[ [ \aggregation{}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{t' \in R}LB(R(t')) \]
\[ [ \aggregation{}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{t' \in R}UB(R(t')) \]

\item Count Aggregation with group by
\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]

\[ [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{R(t')[g] \equiv t[g]}LB(R(t')) \]
\[ [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{R(t')[g] \matches t[g]}UB(R(t')) \]


\item Sum Aggregation without group by
\begin{align*}
[ & \aggregation{}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{t' \in R}\{LB(R(t'))*R(t').\lbMarker{A}\}^+ + \{UB(R(t'))*R(t').\lbMarker{A}\}^-
\end{align*}
\begin{align*}
[ & \aggregation{}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{t' \in R}\{UB(R(t'))*R(t').\ubMarker{A}\}^+ + \{LB(R(t'))*R(t').\ubMarker{A}\}^-
\end{align*}

\item Sum Aggregation with group by
\item \[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
\[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]
\begin{align*}
[ & \aggregation{g}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{R(t')[g] \equiv t[g]}\{LB(R(t'))*R(t').\lbMarker{A}\}^+ + \\ & \sum_{R(t')[g] \matches t[g]} \{UB(R(t'))*R(t').\lbMarker{A}\}^-
\end{align*}
\begin{align*}
[ & \aggregation{g}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{R(t')[g] \matches t[g]}\{UB(R(t'))*R(t').\ubMarker{A}\}^+ + \\ & \sum_{R(t')[g] \equiv t[g]} \{LB(R(t'))*R(t').\ubMarker{A}\}^-
\end{align*}

\end{enumerate}


\subsection{Examples}
\begin{figure}[ht]
	\centering
	\begin{subtable}{0.4\linewidth}
	\centering
	\caption{R-D1}
	\begin{tabular}{ |c|c|l}
				\cline{1-2}
		\textbf{A}  & \textbf{B}  &  \\
		\cline{1-2}
		1 & 1 & 2\\
%				\cline{1-3}
		1 & 2 & 3\\
%				\cline{1-3}
		2 & 3 & 1\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}
	\begin{subtable}{0.4\linewidth}
	\centering
	\caption{R-D2}
	\begin{tabular}{ |c|c|l}
				\cline{1-2}
		\textbf{A}  & \textbf{B}  &  \\
		\cline{1-2}
		1 & 1 & 3\\
%				\cline{1-3}
		1 & 2 & 2\\
%				\cline{1-3}
		1 & 3 & 2\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}

	\vspace*{0.5 cm}

	\begin{subtable}{\linewidth}
	\centering
	\caption{UADB BG=D1 \\ Similar to tuple level}
	\begin{tabular}{ |c|c|l}
				\cline{1-2}
		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
		\cline{1-2}
		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
%				\cline{1-3}
		$1^{[1,1]}$ & $2^{[2,2]}$ & (2,3,3)\\
%				\cline{1-3}
		$2^{[2,2]}$ & $3^{[3,3]}$ & (0,1,1)\\
		$1^{[1,1]}$ & $3^{[3,3]}$ & (0,0,2)\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}

	\vspace*{0.5 cm}

	\begin{subtable}{\linewidth}
	\centering
	\caption{UADB one-liner}
	\begin{tabular}{ |c|c|l}
				\cline{1-2}
		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
		\cline{1-2}
		$1^{[1,2]}$ & $1^{[1,3]}$ & (6,6,7)\\
%				\cline{1-3}
				\cline{1-2}
	\end{tabular}
	\end{subtable}

	\vspace*{0.5 cm}

	\begin{subtable}{\linewidth}
	\centering
	\caption{UADB BG=D1}
	\begin{tabular}{ |c|c|l}
				\cline{1-2}
		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
		\cline{1-2}
		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
%				\cline{1-3}
		$1^{[1,1]}$ & $2^{[2,3]}$ & (3,3,3)\\
%				\cline{1-3}
		$2^{[1,2]}$ & $3^{[3,3]}$ & (1,1,1)\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}

	\vspace*{0.5 cm}

	\begin{subtable}{\linewidth}
	\centering
	\caption{UADB GB=D1 tuple matchings}
	\begin{tabular}{ |c|}
				\cline{1-1}
		\textbf{Certain matching}\\
		\cline{1-1}
		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 2$\\
%				\cline{1-3}
		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D1(1,2) = 3$\\
%				\cline{1-3}
		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D1(2,3) = 1$\\
				\cline{1-1}
		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 2$\\
%				\cline{1-3}
		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,2) = 2$\\
%				\cline{1-3}
		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,3) = 1$\\
		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D2(1,3) = 1$\\
			\cline{1-1}
		\textbf{Possible matching} \\
		\cline{1-1}
		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 1$\\
		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 1$\\
		\cline{1-1}
	\end{tabular}
	\end{subtable}

\caption{A UADB instance correspond to possible worlds semantics}
\label{figexp1}
\end{figure}

\subsection{Rewriting}
\begin{enumerate}
\item Selection
\[ [\selection_{\theta}(A_1,A_2,...,A_n)]=\selection_{\ubMarker{\theta}}(A_1,\lbMarker{A_1},\ubMarker{A_1},...,\lbMarker{\theta} \leftarrow C_R, \theta \leftarrow D_R )\]

\item Join
\begin{align*}
[R \join P]=(R \join P)[R.A_1, \lbMarker{R.A_1},\ubMarker{R.A_1},..., \\ P.A_1, \lbMarker{P.A_1},\ubMarker{P.A_1},..., \\ min(R.C_R,P.C_R) \leftarrow C_R, min(R.D_R,P.D_R) \leftarrow D_R]
\end{align*}

\item Projection
\[ [\projection_{U}(R)]=\projection_{U}(R)[U,\lbMarker{U},\ubMarker{U},...] \]

\item Set Difference
\[ LB[R-P]=R - \projection_{R}(\selection_{R.C_R=T \wedge R.A \matches P.A}(R \join P)) \]
\[ D[R-P]=\selection_{D_R=T}(R)-\selection_{D_R=T}(P) \]
\[ UB[R-P]=R - \selection_{C_R=T \wedge \lbMarker{A}=\ubMarker{A}}(P) \]

\item Aggregation without groupby
\begin{align*}
 [\aggregation{}{sum(A)}(R)]=\aggregation{}{sum(A),sum(\lbMarker{A}),sum(\ubMarker{A}),min(C_R),max(D_R)} ( \\
 \projection_{A,(\lbMarker{A}<0 \vee C_R=T)?\lbMarker{A}:0,(\ubMarker{A}>0 \vee C_R=T)?\ubMarker{A}:0}(R) )
\end{align*}

\item Aggregation with groupby
\begin{align*}
UB[\aggregation{g}{sum(A)}(R)]= \\
\aggregation{R_1.tid}{sum(\lbMarker{R_2.A}),sum(\ubMarker{R_2.A})} ( \\
 \projection_{R_1.g,...,R_2.g,...,(\lbMarker{R_2.A}<0 \vee C_R=T)?\lbMarker{R_2.A}:0,...} ( \\
 \selection_{R_1.g \matches R_2.g}(\rename(R_1,R) \join \rename(R_2,R))))
\end{align*}


\end{enumerate}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-aggregation-tech.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Aggregation}
\BG{We previously claimed that this works for bags and sets. Does it work for a more general class of semirings?
  Maybe all semirings where the symbolic semimodule elements can always be reduced to a concrete value?}

We now introduce a semantics for aggregation over \abbrUAADBs that preserves
bounds.  One major challenge in of defining aggregation over $\semK$-relations
which also applies to our problem setting is that one has to take the
annotations of tuples into account when calculating the aggregation function
results. For instance, under bag semantics (semiring $\semN$) the multiplicity
of a tuple affects the result of \lstinline!SUM! aggregation.  We first review
the aggregation semantics for $\semK$-relations from~\cite{AD11d} that studies
how $\semK$ tuple annotations can be factored into the calculation of aggregation
functions.  Towards this goal , then discuss its applicability to
\abbrUAADB-relations, and then introduce a bound preserving semantics for an
important class of semirings that does not require the introduction of symbolic
expressions as values (which is required to handle aggregation over
$\semK$-relations in general).  We have to overcome two major challenges: (i)
since the values of group-by attributes may be uncertain, a tuple's group
membership may be uncertain too and (ii) we are aggregating over range-bounded
values. To address (ii) we can utilitze the expression semantics for
range-bounded values from \Cref{sec:expression}. However, additional
complications arise when taking the $\uaaK{\semK}$-annotations of tuples into
account. For (i) we will reason about all possible group memberships of
range-annotated tuples to calculate bounds on group-by values, aggregation
function results, and number of result groups.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background}
\label{sec:background-1}
Amsterdamer et al.~\cite{AD11d} introduced a semantics for aggregation queries
over $\semK$-relations that commutes with homomorphisms and under which
aggregation results can be encoded with polynomial space. Contrast this with the
aggregation semantics for c-tables
from~\cite{DBLP:journals/jiis/LechtenborgerSV02} where aggregation results may
be of size exponential in the input size.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Aggregation Monoids} \cite{AD11d} deals with aggregation functions that
are commutative monoids $(\monoid, \amadd, \amzero)$, i.e., where
the values from
$\monoid$ that are the input to aggregation are combined through an operation
$\amadd$ which has a neutral element $\amzero$.\footnote{A monoid is a
  mathematical structure $(\monoid, \amadd, \amzero)$ where $\amadd$ is a
  commutative and associative binary operation over $\monoid$, and $\amzero$ is
  the neutral element of $\monoid$. For instance,
  $\msum \defas (\mathbb{R}, +, 0)$, i.e., addition over the reals can be used
  for sum aggregation.} Most standard aggregation
functions (\aggsum, \aggmin, \aggmax, and \aggcount) can be expressed as monoids
or, in the case of \aggavg, can be derived from multiple monoids (count and
sum). As an example consider the monoids for \aggsum and \aggmin:
$\msum \defas (\mathbb{R}, +, 0)$ and $\mmin \defas (\mathbb{R}, \min,
\infty)$. The result of aggregation over a set of $\monoid$ values is then defined as
combining the values from the set using the addition operation of the
monoid $\monoid$. Note that bound-preserving evaluation of these monoids over
range-annotated values is already supported though the range-annotated
expression semantics from \Cref{sec:expression}. For instance, $\msum$ simply
uses the addition operation we defined. Even though we did not define $\aggmin$
and $\aggmax$ explicitly, we can express them using the operators
from~\Cref{def:expr-syntax}, e.g., $\min(v,w) \defas \ifte{v \leq w}{v}{w}$. In
the following, we use $\rangeMon$ to denote the range-annotated version of
$\monoid$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}\label{lem:range-annotated-monoids}
$\rangeMof{\msum}$, $\rangeMof{\mmin}$, $\rangeMof{\mmax}$ are monoids.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  Addition in $\rangeDom$ is applied point-wise. Thus, addition in $\rangeDom$
  is commutative and associative and has neutral element $\uv{0}{0}{0}$. Thus,
  $\rangeMof{\msum}$ is a monoid. For $\rangeMof{\mmin}$ if we substitute the
  definition of $\ifte{v \leq w}{v}{w}$ and $v \leq w$ and simplify the
  resulting expression we get
  $\min(\uv{a_1}{a_2}{a_3}, \uv{b_1}{b_2}{b_3}) =
  \uv{\min(a_1,b_1)}{\min(a_2,b_2)}{\min(a_3,b_3)}$. That is, the operation is
  again applied pointwise and commutativity, associativity, and identity of the
  neutral element ($\uv{\infty}{\infty}{\infty}$) follow from the fact that
  $\mmin$ is a monoid. The proof for max is symmetric.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Based on \Cref{lem:range-annotated-monoids} we can state the following
corollary:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Corollary}[Aggregation Functions Preserve Bounds]\label{cor:aggregation-functions-preserve}
  Let $\mathcal{S} = \{c_1, \ldots, c_n\} \subseteq \rangeDom$ be a set of
  range-annotated values and $S = \{d_1, \ldots d_n\} \subseteq \dataDomain$ be
  a set of values such that $c_i$ bounds $d_i$, and
  $\rangeMon \in \{\rangeMof{\msum}, \rangeMof{\mmax}, \rangeMof{\mmin}\}$, then
  using the addition operation of $\rangeMon$ ($\monoid$) we have that
  $\sum \mathcal{S} $ bounds $\sum S $.
\end{Corollary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  The corollary follows immediately from \Cref{theo:expr-bound}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \centering
  \begin{align}
    k \smbpair_{\monoid} (m_1 \amadd m_2) & = k \smbpair_{\semK} m_1 \amadd k \smbpair_{\semK} m_2 \\
    (k_1 \addK k_2) \smbpair_{\monoid} m  & = k_1 \smbpair_{\semK} m \amadd k_2 \smbpair_{\semK} m \\
    \oneK \smbpair_{\monoid} m            & = m                                                    \\
    \zeroK \smbpair_{\monoid} m           & = \amzero                                              \\
    k \smbpair_{\monoid} \amzero          & = \amzero                                              \\
    (k_1 \multK k_2) \smbpair_{\monoid} m & = k_1 \smbpair_{\monoid} (k_2 \smbpair_{\monoid} m)
  \end{align}
  \caption{Semimodule laws (semiring $\semK$ paired with monoid $\monoid$)}
  \label{fig:semimodule-laws}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Semimodules and Tensor Construction}
%
As mentioned above, one challenge of supporting aggregation over
$\semK$-relations is that the annotations of tuples have to be factored into the
aggregation computation. For instance, consider an $\semN$-relation $R(A)$ with
two tuples $(30) \mapsto 2$ and $(40) \mapsto 3$, i.e., there are two duplicates
of tuple $(30)$ and $3$ duplicates of tuple $(40)$. Computing the sum over $A$
we expect to get $30 \cdot 2 + 40 \cdot 3 = 180$. More generally speaking, we
need an operation $\smbpair_{\monoid}: \semK \times \monoid \rightarrow \monoid$
that combines semiring elements with values from the aggregation function's
domain as in the $\semN$-relation example above. As observed in~\cite{AD11d}
this operation has to be a semimodule, i.e., it has to fulfill equational laws shown in \Cref{fig:semimodule-laws}. % such as
% including
% $(k \addK k') \smbpair_{\semK} m = k \smbpair_{\semK} m \amadd k'
% \smbpair_{\semK} m$.
Note that in the example above we made use of the fact that
$\smbpair_{\semN,\msum}$ is $\cdot$ to get
$30 \smbpair_{\semN} 2 = 30 \cdot 2 = 60$.  While $\smbpair$ is well defined for
for semirings $\semN$ and $\semB$ (if we only consider idempotent aggregation
functions such as \aggmin and \aggmax), Amsterdamer et al. demonstrated that
there is no meaningful way to define such an operation for all combinations of
semirings and standard aggregation function monoids.\footnote{To be more
  precise, if aggregation function results are concrete values from the
  aggregation monoid, then it is not possible to retain the important property
  that queries commute with homomorphisms. Intuitively, that is the case because
  applying a homomorphism to the input may change the aggregation function
  result. Hence, it is necessary to delay the computation of concrete
  aggregation results by keeping the computation symbolic. For instance,
  consider an $\semNX$-relation $R(A)$ (provenance polynomials) with a single
  tuple $(30) \mapsto x_1$. If we compute the sum over $A$, then under a
  homomorphism $h_1: x_1 \to 1$ we get a result of $30 \cdot 1 = 30$ while under
  a homomorphism $h_2: x_1 \to 2$ we get $30 \cdot 2 = 60$.} The solution
presented in~\cite{AD11d} uses monoids whose elements are symbolic expressions
that pair semiring values with monoid elements. Such monoids are compatible with
a larger class of semirings including, e.g., the provenance polynomial
semiring. Given a semiring $\semK$ and aggregation monoid $\monoid$, the
symbolic commutative monoid has as domain bags of elements from
$\semK \times \monoid$ with bag union as addition (denoted as $\akmadd$) and the
emptyset as neutral element. This structure is then extended to a
$\semK$-semimodule $\asm$ by defining
$k \smbpair_{\asm} \sum k_i \smpair m_i \defas \sum (k \multK k_i) \smpair m_i$
and taking the quotient (the structure whose elements are equivalent classes)
wrt. the semimodule laws. For some semirings, e.g., $\semN$ and $\semB$, the
symbolic expressions from $\asm$ correspond to concrete aggregation result
values from $\monoid$.\footnote{That is the case when $\monoid$ and $\asm$ are
  isomorphic.} However, this is not the case for every semiring and aggregation
monoid. For instance, for most provenance semirings these expressions cannot be
reduced to concrete values. Only by applying homomorphisms to semirings for
which this construction is isomorphic to the aggregation monoid is it possible
to map such symbolic expressions back to concrete values. For instance,
computing the sum over the $\semNX$-relation $R(A)$ with tuples
$(30) \mapsto x_1$ and $(20) \mapsto x_2$ yields the symbolic expression
$30 \smpair x_1 \kmadd{\semNX}{\msum} 20 \smpair x_2$. If the input tuple
annotated with $x_1$ occurs with multiplicity $2$ and the input tuple annotated
with $x_2$ occurs with multiplicity $4$ then this can be expressed by applying a
homomorphism $h: \semNX \to \semN$ defined as $h(x_1) = 2$ and $h(x_2) =
4$. Applying this homomorphism to the symbolic aggregation expression
$30 \smpair x_1 \kmadd{\semNX}{\msum} 20 \smpair x_2$, we get the expected
result $30 \cdot 2 + 20 \cdot 4 = 140$. If we want to support aggregation for
$\uaaK{\semK}$-relations with this level of generality then we would have to
generalize range-annotated values to be symbolic expressions from $\asm$ and
would have to investigate how to define an order over such values to be able to
use them as bounds in range-annotated values. For instance, intuitively we may
bound $(x_1 + x_2) \smpair 3 \kmadd{\semNX}{\msum} x_3 \smpair 2$ from below
using $x_1 \smpair 3 \kmadd{\semNX}{\msum} x_3 \smpair 1$ since
$x_1 \ordOf{\semNX} x_1 + x_2$ and $2 < 3$.  Then we would have to show that
aggregation computations preserve such bounds to show that queries with
aggregation with this semantics preserve bounds. We trade generality for
simplicity by limiting the discussion to semirings where $\asm$ is isomorphic to
$\monoid$. This still covers the important cases of bag semantics and set
semantics ($\semN$ and $\semB$), but has the advantage that we are not burdening
the user with interpreting bounds that are complex symbolic expressions. For
instance, consider an aggregation without group-by over a relation with millions
of rows. The resulting bound expressions for the aggregation result value may
contain millions of terms which would render them completely useless for human
consumption. Additionally, while query evaluation is still be \ptime when using
$\asm$, certain operations like joins on aggregation results are
inefficient.\footnote{Comparing symbolic expressions requires an extension of
  annotations to treat these comparisons symbolically. The reason is that since
  an aggregation result cannot be mapped to a concrete value, it is also not
  possible to determine whether such a values are equal. The net result is that
  joins on such values may degenerate to cross products.}

 % \BG{Give more motivation for why we limit ourselves here}
 % \BG{Some thoughts for the future if we want to have semimodule expressions as bounds:
 %  \textbullet We need an order that is preserved under queries and under taking homomorphisms
 %  \textbullet It seems that if  both the aggregation monoid $\monoid$ and the semiring $\semK$ are naturally ordered it is possible to define such an order. Since each element $km \in \asm$ is an equivalence class of bags of pairs $k_i \smpair m_i$ (functions $\semK \times \monoid \to \semN$) wrt. to laws that require addition to compatible with the aggregation computation, e.g., $(k_1 \addK k_2) \smpair m = k_1 \smpair m \akmadd k_2 \smpair m$, we can split out equal parts and define $k_1 \ordOf{\asm} k_2$ as: there exist $k_1'$ and $k_2'$ which belong to the same equivalence class as $k_1$ and $k_2$ and $\forall k \in \semK, m \in \monoid: k_1'(k, m) < k_2'(k,m)$. For instance, $k_1 = (x_1 + x_2) \smpair 5 \ordOf{\asm} x_1 \smpair 7 \akmadd x_2 \smpair 5 = k_2$ because using $k_1' = x_1 \smpair 5 \akmadd x_2 \smpair 5$ and $k_2' = x_1 \smpair 5 \akmadd x_1 \smpair 2 \akmadd x_2 \smpair 5$, $k_1'(x_1, 5)  = 1 = k_2'(x_1, 5)$, $k_1'(x_1, 2) = 0 \leq 1 k_2'(x_1, 2)$, and $k_1'(x_2, 5) = 1 = k_2'(x_2, 5)$.
 %  \textbullet Looks like checking whether $k \ordOf{\asm} k'$ is computationally hard (subset sum, probably) unless every semiring element can be written as a sum of $\oneK$ elements ($\oneK$ is a generator for the semiring). However, that would not prevent us from creating bounds (we are constructing an element smaller than a given $k$ instead of having to check for two arbitrary elements whether $k \ordOf{\asm} k'$.
 %  }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Applying Semimodules for $\uaaK{\semK}$-Relations}
\label{sec:semim-uaaks-relat}

As we will demonstrate in the following, even though it may be possible to
define $\uaaK{\semK}$-semimodules, such semimodules cannot be bound preserving
and, thus, would be useless for our purpose. We then demonstrate that it is
possible to define bound preserving operations that combine $\uaaK{\semN}$ (or
$\uaaK{\semB}$) elements with $\rangeDom$ elements and that this is sufficient
for defining a bound preserving semantics for aggregation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}[Bound preserving $\uaaK{\semN}$-semimodules are impossible]\label{lem:bound-preserving-impossible}
The semimodule for $\uaaK{\semN}$ and $\msum$, if it exists, cannot be bound preserving.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  For sake of contadiction assume that this semimodule exists and is bound preserving.
  Consider $k = \ut{1}{1}{2}$ and $m = \uv{0}{0}{0}$. Then by semimodule law \ref{eq:semimodule-with-m-zero-yields-m-zero} we have $k \smbpair_{\uaaK{\semN},\msum} m = m = \uv{0}{0}{0}$. Now observe that for $m_1 = \uv{-1}{-1}{-1}$ and $m_2 = \uv{1}{1}{1}$ we have $m = m_1 + m_2$. Let $m_1' = k \smbpair_{\uaaK{\semN},\msum} m_1$. We know that $m_1' = \uv{l_1}{-1}{u_1}$ for some $l_1$ and $u_1$. Since the semimodule is assumed to be bound preserving we know that $l_1 \leq -2$ and $u_1 \geq -1$ ($-1 \cdot 2=-2$ and $-1 \cdot 1 = -1$). Analog, let $m_2' = \uv{l_2}{1}{u_2} = k \smbpair_{\uaaK{\semN},\msum} m_2$. By the same argument we get $l_2 \leq 1$ and $u_2 \geq 2$. Applying semimodule law \ref{eq:semimodule-distributes-over-m-plus} we get $k \smbpair_{\uaaK{\semN},\msum} m = k \smbpair_{\uaaK{\semN},\msum} (m_1 + m_2)  = m_1' + m_2'  = \uv{l_1 + l_2}{0}{u_1 + u_2}$. Let $l' = l_1 + l_2$, $u' = u_1 + u_2$ and $m'' = \uv{l'}{0}{u'}$. Based on the inequalities constraining $l_i$ and $u_i$ we know that $l_1 + l_2 \leq -1$ and $u_1 + u_2 \geq 1$. Thus, we have the contradiction $k \smbpair_{\uaaK{\semN},\msum} m = \uv{0}{0}{0} \neq \uv{l'}{0}{u'} = k \smbpair_{\uaaK{\semN},\msum} m$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We first discuss how $\semK$-semimodules for a monoid $\monoid$ can be extended
for $\uaaK{\semK}$-semimodules.  As it turns out, point-wise application of
$\smbpair_{\semK,\monoid}$ does not always preserve bounds, i.e., the result is
in $\semkq$ but potentially not in $\uaaK{\semK}$.  For instance, consider sum
aggregation ($\msum$) over bag semantics relations (semiring $\semN$). As
mentioned above, the corresponding semimodules $\smbpair_{\semN,\msum}$ is
simply multiplication of a real with a natural number. Consider a
$\uaaK{\semN}$-relation $\rangeRel(A)$ with a single tuple $(\uv{-3}{-2}{-1})$
with annotation $(0,1,1)$ and query $\aggregation{sum(A)}{}(R)$. If
$\smbpair_{\uaaK{\semN},\msum}$ would be defined as point-wise application of
$\smbpair_{\semN,\msum}$, then the result of aggregation would be
$\uv{-3 \cdot 0}{-2 \cdot 1}{-1 \cdot 1} = \uv{0}{-2}{-1}$ which is a not a
valid range-annotated value since it is not the case that $0 \leq -2 \leq -1$.
The reason why point-wise application fails is that $\smbpair_{\semK,\monoid}$
does not preserve the order of the domain $\dataDomain$ based on which we
defined range-annotated values. For example, as we already saw in
\Cref{sec:range-expr-eval}, that multiplication over $\rangeDom$ cannot be
defined pointwise to preserve bounds. Since, $\smbpair_{\semN,\msum}$ is
multiplication it is thus not suprising that pointwise application of
$\smbpair_{\semN,\msum}$ also fails to preserve bounds.  Since we are mainly
looking for a solution that can deal with bags and sets and common aggregation
functions, we define $\smbpair_{\uaaK{\semK}, \monoid}$ such that it works for
these common cases. The idea applied in the definition below is the same as uses
in the definition of multiplication over range-annotated values: evaluate
$\smbpair_{\semK,\monoid}$ over all combinations of values from the input and
then return the minimum and maximum values over this set as bounds.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:range-semimodules}
  Consider a semiring $\semK$ and aggregation monoid $\monoid$ such that $\smbpair_{\semK,\monoid}$ is well defined.
  Let $(\lbMarker{m},m,\ubMarker{m})$ be a range-annotated value from $\rangeDom$ and $(\lbMarker{k},k,\ubMarker{k}) \in \uaaK{\semK}$.
  %Let triple  that  the value domain. Let triple $\semNX^3=(\lbMarker{x},x,\ubMarker{x})$ denote a tuple annotation value in \abbrAUDB.
  We define $\smbpair_{\uaaK{\semK},\monoid}$ as shown below. % range aggregation monoid multiplication computation yields a triple as below.
	\begin{align*}
		(\lbMarker{k},&{k},\ubMarker{k}) \smbpair_{\uaaK{\semK},\monoid} (\lbMarker{m},{m},\ubMarker{m}) = \\
		( & min(\lbMarker{k} \smbpair_{\semK,\monoid} \lbMarker{m},\lbMarker{k} \smbpair_{\semK,\monoid} \ubMarker{m},\ubMarker{k} \smbpair_{\semK,\monoid} \lbMarker{m},\ubMarker{k} \smbpair_{\semK,\monoid} \ubMarker{m}), \\
		& {k} \smbpair_{\semK,\monoid} {m}, \\
		& max(\lbMarker{k} \smbpair_{\semK,\monoid} \lbMarker{m},\lbMarker{k} \smbpair_{\semK,\monoid} \ubMarker{m},\ubMarker{k} \smbpair_{\semK,\monoid} \lbMarker{m},\ubMarker{k} \smbpair_{\semK,\monoid} \ubMarker{m}))
	\end{align*}

\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that, in general there is no guarantee that
$\smbpair_{\uaaK{\semK},\monoid}$ according to \Cref{def:range-semimodules}
preserves bounds. However, as the following theorem demonstrates for common
aggregates over set and bag semantics range-annotated databases this is the
case.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}
  Let $\monoid \in \{\mmin, \mmax\}$ and $\semK \in \{\semB, \semN\}$ or $\monoid = \msum$ and $\semK = \semN$. Then $\smbpair_{\uaaK{\semK},\monoid}$ preserves bounds.
\end{Theorem}
\begin{proof}
We first prove the theorem for $\semN$.
  We have to show for all $\monoid \in \{\mmin, \mmax, \msum\}$ that for any $\vec{k} = \ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}} \in \uaaK{\semN}$ and $\vec{m} = \uv{\lbMarker{m}}{\bgMarker{m}}{\ubMarker{m}} \in \rangeDom$ we have that $\vec{k} \smbpair_{\uaaK{\semN},\monoid} \vec{m}$ bounds $k \smbpair_{\semN,\monoid} m$ for any $k$ bound by $\vec{k}$ and $m$ bound by $\vec{m}$. We prove the theorem for each  $\monoid \in \{\mmin, \mmax, \msum\}$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\monoid = \msum$}
%
We have $k \smbpair_{\semN,\msum} m \defas k \cdot m$. We distinguish four cases:

\proofpara{$\lbMarker{m} < 0$, $\ubMarker{m} < 0$}
%
We have that $\ubMarker{k} \cdot \lbMarker{m} = min(\lbMarker{k} \cdot \lbMarker{m},\lbMarker{k} \cdot \ubMarker{m},\ubMarker{k} \cdot \lbMarker{m},\ubMarker{k} \cdot \ubMarker{m}$) and $\lbMarker{k} \cdot \ubMarker{m} = max(\lbMarker{k} \cdot \lbMarker{m},\lbMarker{k} \cdot \ubMarker{m},\ubMarker{k} \cdot \lbMarker{m},\ubMarker{k} \cdot \ubMarker{m})$.
Thus,
\begin{align*}
\vec{k} \smbpair_{\uaaK{\semN},\monoid} \vec{m} &= \uv{\ubMarker{k} \cdot \lbMarker{m}}{\bgMarker{k} \cdot\bgMarker{m}}{\lbMarker{k} \cdot \ubMarker{m}}
\end{align*}
Now for any $k$ bound by $\vec{k}$ and $m$ bound by $\vec{m}$ we have:
$\ubMarker{k} \cdot \lbMarker{m} \leq k \cdot m$ because $m$ is a negative number and $k \leq \ubMarker{k}$. Analog, $k \cdot m \leq \lbMarker{k} \cdot \ubMarker{m}$, because $m$ is negative and $\ubMarker{m} \geq m$ and $\lbMarker{k} \leq k$. Thus, $\vec{k} \smbpair_{\uaaK{\semN},\monoid} \vec{m}$ bounds $k \smbpair_{\semN,\monoid} m$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\lbMarker{m} \geq 0$, $\ubMarker{m} \geq 0$}
%
We have that $\lbMarker{k} \cdot \lbMarker{m} = min(\lbMarker{k} \cdot \lbMarker{m},\lbMarker{k} \cdot \ubMarker{m},\ubMarker{k} \cdot \lbMarker{m},\ubMarker{k} \cdot \ubMarker{m}$) and $\ubMarker{k} \cdot \ubMarker{m} = max(\lbMarker{k} \cdot \lbMarker{m},\lbMarker{k} \cdot \ubMarker{m},\ubMarker{k} \cdot \lbMarker{m},\ubMarker{k} \cdot \ubMarker{m})$.
Thus,
\begin{align*}
\vec{k} \smbpair_{\uaaK{\semN},\monoid} \vec{m} &= \uv{\lbMarker{k} \cdot \lbMarker{m}}{\bgMarker{k} \cdot\bgMarker{m}}{\ubMarker{k} \cdot \ubMarker{m}}
\end{align*}
Now for any $k$ bound by $\vec{k}$ and $m$ bound by $\vec{m}$ we have:
$\ubMarker{k} \cdot \lbMarker{m} \leq k \cdot m$ because $m$ is a positive number and $k \geq \lbMarker{k}$. Analog, $k \cdot m \leq \ubMarker{k} \cdot \ubMarker{m}$, because $m$ is negative and $\ubMarker{m} \geq m$ and $\ubMarker{k} \geq k$. Thus, $\vec{k} \smbpair_{\uaaK{\semN},\monoid} \vec{m}$ bounds $k \smbpair_{\semN,\monoid} m$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\lbMarker{m} < 0$, $\ubMarker{m} \geq 0$}
%
We have that $\ubMarker{k} \cdot \lbMarker{m} = min(\lbMarker{k} \cdot \lbMarker{m},\lbMarker{k} \cdot \ubMarker{m},\ubMarker{k} \cdot \lbMarker{m},\ubMarker{k} \cdot \ubMarker{m}$) and $\ubMarker{k} \cdot \ubMarker{m} = max(\lbMarker{k} \cdot \lbMarker{m},\lbMarker{k} \cdot \ubMarker{m},\ubMarker{k} \cdot \lbMarker{m},\ubMarker{k} \cdot \ubMarker{m})$.
Thus,
\begin{align*}
\vec{k} \smbpair_{\uaaK{\semN},\monoid} \vec{m} &= \uv{\ubMarker{k} \cdot \lbMarker{m}}{\bgMarker{k} \cdot\bgMarker{m}}{\ubMarker{k} \cdot \ubMarker{m}}
\end{align*}

Now consider some $k$ bound by $\vec{k}$ and $m$ bound by $\vec{m}$. If $m$ is positive, then trivially $\lbMarker{k} \cdot \lbMarker{m}$ bounds $k \cdot m$ from below since $\lbMarker{m}$ is negative. Otherwise, the lower bound holds using the argument for the case of $\lbMarker{m} < 0$, $\ubMarker{m} < 0$. If $m$ is negative, then trivally $\ubMarker{k} \cdot \ubMarker{m}$ bounds $k \cdot m$ from above since $\ubMarker{m}$ is positive. Otherwise, the upper bound holds using the argument for the case of $\lbMarker{m} \geq 0$, $\ubMarker{m} \geq 0$. Thus, $\vec{k} \smbpair_{\uaaK{\semN},\monoid} \vec{m}$ bounds $k \smbpair_{\semN,\monoid} m$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\monoid = \mmin$}
%
We have
\[
  k \smbpair_{\semN,\mmin} m \defas
\begin{cases}
  0 &\mathtext{if} k = 0\\
  m &\mathtext{otherwise}\\
\end{cases}
\]

We distinguish three cases.

\proofpara{$\lbMarker{k} \geq 0$}
%
If $\lbMarker{k} \geq 0$, then $k \smbpair_{\semN,\mmin} m$ returns $m$ and $\vec{k} \smbpair_{\uaaK{\semN}, \mmin} \vec{m}$ returns $\vec{m}$. Since $\vec{m}$ bounds $m$ also $\vec{k} \smbpair_{\uaaK{\semN}, \mmin} \vec{m}$ bounds  $k \smbpair_{\semN,\mmin} m$.

\proofpara{$\lbMarker{k} = 0$, $\ubMarker{k} \geq 0$}
%
Now consider the remaining case: $\lbMarker{k} = 0$. Then the result of $\vec{k} \smbpair_{\uaaK{\semN},\mmin} \vec{m}$ simplifies to $\uv{min(0,\lbMarker{m})}{\bgMarker{k} \cdot \bgMarker{m}}{max(0,\ubMarker{m})}$. Now consider some $k$ bound by $\vec{k}$ and $m$ bound by $\vec{m}$. If $k \neq 0$ then $k \smbpair_{\semN,\mmin} m = m$ and the claim to be proven holds. Otherwise, $k \smbpair_{\semN,\mmin} m = 0$ which is bound by $\uv{min(0,\lbMarker{m})}{\bgMarker{k} \cdot \bgMarker{m}}{max(0,\ubMarker{m})}$.

\proofpara{$\lbMarker{k} = 0$, $\ubMarker{k} = 0$}
In this case $\vec{k} \smbpair_{\uaaK{\semN}, \mmin} \vec{m} = \uv{0}{0}{0}$ and since $k = 0$ because $\vec{k}$ bounds $k$ we have $k \smbpair_{\semN,\mmin} m = 0$ which is trivally bound by $\uv{0}{0}{0}$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\monoid = \mmax$}
%
We have
\[
  k \smbpair_{\semN,\mmax} m \defas
\begin{cases}
  0 &\mathtext{if} k = 0\\
  m &\mathtext{otherwise}\\
\end{cases}
\]
The proof for $\mmax$ is analog to the proof for $\mmin$.

For semiring $\semB$ and $\monoid = \mmin$ or $\monoid = \mmax$ observe that $k \smbpair_{\semB,\monoid} m$ is the identity for $m$ if $k \neq \zeroOf{\semB}$ and $k \smbpair_{\semB,\monoid} m = 0$ otherwise. Thus, the proof is analog to the proof for semiring $\semN$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bound-Preserving Aggregation}
\label{sec:bound-pres-aggr}
We now define a bound preserving aggregation semantics based on
$\uaaK{\semK}$-semimodules operations.  As mentioned above, the main challenge
we have to overcome is to deal with the uncertainty of group memberships plus
the resulting uncertainty in the number of groups and of which inputs contribute
to a group's aggregation function result values.  In general, the number of
possible groups encoded by an input \abbrUAADB-relation may be very large. Thus,
enumerating all concrete groups is not a viable option.  While \abbrUAADBs can
be used to encode an arbitrary number of groups as a single tuple, we need to
decide how to trade conciseness of the representation for accuracy of the
representation. Furthermore, we need to ensure that the aggregation result in
the \abbrBGW is encoded by the result. There are many possible strategies for
how to group possible aggregation results. We will present a semantics that
works for all grouping strategies that fulfill two basic correctness criteria:
preservation of the groups in the \abbrBGW and accounting for all possible
groups. Intuitively, a grouping strategy defines a set of output tuples and
associates (i) each tuple in the \abbrBGW with one such output and (ii) each
possible group covered by the group-by attribute range annotations of at least
one input tuple with one output. Our aggregation semantics then calculates the
group-by and aggregation function attribute ranges for each tuple in the
$\uaaK{\semK}$ aggregation result as well as bounds on tuple annotations (number
of possible groups).  We introduce a default grouping strategy which creates
one output tuple for each group in the \abbrBGW. For each \abbrBG group we
output one result tuple. All other possible groups that do not appear as the
\abbrBG value of an input tuple will be merged into one of the \abbrBG groups by
merging their group-by values into the range annotation of such a \abbrBG group.
%   We demonstrate how to calculate aggregation results for any such functions as long as they obey
% certain correctness criteria.  We also introduce one default grouping strategy which creates one output tuple for each group in the  \abbrBGW. For each \abbrBG group we output one result tuple. All other
% possible groups that do not appear as the \abbrBG value of an input tuple will
% be merged into one of the \abbrBG groups by merging their group-by values into
% the range annotation of such a \abbrBG group.
We start by formally defining grouping strategies

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Grouping Strategies}
\label{sec:grouping-strategies}

A \textit{grouping strategy} $\gstrat$ is a function that takes as input a n-ary $\uaaK{\semK}$-relation $\rangeRel$ and list of group-by attributes $\gbAttrs$ and returns a triple $(\stratGrps, \stratBG, \stratPoss)$ where $\stratGrps$ is a set of output groups, $\stratBG$
is a  function associating each input tuple $\rangeTup$ from $\rangeRel$ where $\bgMarker{\rangeRel(\rangeTup)} \neq \zeroK$ with an output from $\stratGrps$,
and $\stratPoss$ is a  function associating each input tuple $\rangeTup$ from $\rangeRel$ where $\rangeRel(\rangeTup) \neq \uaaZero{\semK }$ with an output from $\stratGrps$. Note that the elements of  $\stratGrps$ are just unique identifiers for output tuples.  The actual range-annotated output tuples returned by an aggregation operator are not returned by the grouping strategy directly but are constructed by our aggregation semantics based on the information returned by a grouping strategy.
Intuitively, $\stratBG$ takes care of the association of groups in the \abbrBGW with an output while $\stratPoss$ does the same for all possible groups. For $\gstrat$ to be a grouping strategy we require that for any input relation $\rangeRel$ and list of group-by attributes $\gbAttrs$ we have:

\begin{align*}
  % same BG group => same output
  \forall \rangeTup, \rangeTup' \in \rangeDom^n:\,\,\, &\rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semK}}
  \wedge \rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semK}}
  \wedge \bgMarker{\rangeTup.\gbAttrs} = \bgMarker{\rangeTup'.\gbAttrs}\\
  &\rightarrow
  \stratBG(\rangeTup) = \stratBG(\rangeTup')
\end{align*}

This condition ensures that for every tuple that exists in the \abbrBGW, all inputs that exists in the \abbrBGW and belong this group are associated with a single output. Our aggregation semantics relies on this property to produce the correct result in the \abbrBGW. We use function $\stratPoss$ to ensure that every possible group is accounted for by the $\uaaK{\semK}$-relation returned as the result of aggregation. Inuitively, every range-annotated input tuple may correspond to several possible groups based on the range annotations of its group-by attribute values.
Our aggregation semantics takes ensures that an output tuple's group-by ranges bound the group-by attribute ranges of every input associated to it by $\stratPoss$.

% \BG{Based on discussion with Oliver:
%   \textbullet explain that there are many options
%   \textbullet extend the idea to have a ``default grouping'' for lower bound computation and group-by attribute uncertainty
%   \textbullet explain that we present only one choice of these two parameters and reason why this one is good
%   \textbullet explain that the remainder of the approach works for any reasonable choice for these parameters (figure out what are the requirements, e.g., best groups have to be present individually)
%   }

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Default Grouping Strategy}
\label{sec:defa-group-stratg}

As mentioned above, our default grouping strategy, denoted as $\gsdef$, creates one output tuple for every \abbrBG group, i.e., an input tuple's group-by values in the \abbrBGW. Note that also for input
  tuples whose \abbrBG annotation is $\zeroK$, we still use their \abbrBG values
  to group them. Only tuples that are not possible (annotated with $\uaaZero{\semK} = \ut{\zeroK}{\zeroK}{\zeroK}$) are not considered. The possible groups of an input tuple are associated with the output that corresponds to the tuple's group-by values in the \abbrBGW.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Default Grouping Strategy]
Consider a query $\query \defas \aggregation{\gbAttrs}{f(A)}(\rangeRel)$. % We use $\ggrouping(\gbAttrs,\rangeRel)$ to denote the set of groups in the \abbrBGW for relation $\rangeRel$ grouping on $\gbAttrs$: % The best guess grouping can be defined as below.
% \begin{align*}
% 	\ggrouping(\gbAttrs,\rangeRel) = \{ t.\gbAttrs \mid \exists \rangeTup: \bgMarker{\rangeTup} = t \wedge \rangeRel(\rangeTup) \neq \uaaZero{\semK} \}
% \end{align*}
The default grouping strategy $\gsdef$ is defined as shown below. Here, let $\rangeTup \in \rangeDom^n$ such that $\rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semK}}$ and $\rangeTup' \in \rangeDom^n$ such that $\bgMarker{\rangeRel(\rangeTup')} \neq \zeroK$.
\begin{align*}
  \gsdef(\gbAttrs, \rangeRel) & \defas (\gsdefG, \gsdefBG, \gsdefP)                                                                                       \\
 \gsdefG                      & \defas \{ t.\gbAttrs \mid \exists \rangeTup: \bgMarker{\rangeTup} = t \wedge \rangeRel(\rangeTup) \neq \uaaZero{\semK} \} \\ %\ggrouping(\gbAttrs, \rangeRel) \\
  \gsdefBG(\rangeTup')        & \defas \bgMarker{\rangeTup'.\gbAttrs}                                                                                     \\
  \gsdefP(\rangeTup)          & \defas \bgMarker{\rangeTup.\gbAttrs}
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Note that one range-annotated input tuple may belong to multiple groups since
% its group-by values may bound multiple \abbrBG groups.
For instance, consider
three tuples $\rangeTup_1 \defas (\uv{1}{2}{2})$ and
$\rangeTup_2 \defas (\uv{2}{2}{4})$ and $\rangeTup_3 \defas (\uv{2}{3}{4})$ over schema $\rel(A)$.
Furthermore, assume that $\rangeRel(\rangeTup_1) = \ut{1}{1}{1}$, $\rangeTup(\rangeTup_2) = \ut{0}{0}{1}$, and
$\rangeTup(\rangeTup_3) = \ut{0}{0}{3}$.
Grouping on $A$,
the default strategy will generate  two output groups $\agroup_1$ for \abbrBG group $(2)$ and
$\agroup_2$ for \abbrBG group $(3)$.
Tuple $\rangeTup_1$ is the only tuple that is present in the \abbrBGW. Function $\gsdefBG$ assigns $\rangeTup_1$ to $\agroup_1$.
Based on their \abbrBG group-by values, the possible grouping function $\gsdefP$ assigns $\rangeTup_1$ and $\rangeTup_2$ to $\agroup_1$ and $\rangeTup_3$ to $\agroup_2$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Aggregation Semantics}
\label{sec:aggr-semant}

We now introduce an aggregation semantics that is parameterized by a grouping strategy.
For simplicity we define aggregation without group-by as a special case of aggregation with group-by (the only difference is how tuple annotations are handled). We first define how to construct a result tuple $\aout$ for each output group $\asgrp$ returned by the grouping strategy and then present how to calculate tuple annotations. The construction of an output tuple is divided into two steps: (i) determine range annotations for the group-by attributes and (ii) determine range annotations for the  aggregation function result attributes. % for each output created by the grouping strategy.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[\capitalBG Grouping]
% Consider a query $\query \defas \aggregation{\gbAttrs}{f(A)}(\rangeRel)$. We use $\ggrouping(\gbAttrs,\rangeRel)$ to denote the set of groups for relation $\rangeRel$ grouping on $\gbAttrs$: % The best guess grouping can be defined as below.
% \begin{align*}
% 	\ggrouping(\gbAttrs,\rangeRel) = \{ t \mid \exists \rangeTup: \bgMarker{\rangeTup} = t \wedge \rangeRel(\rangeTup) \neq \uaaZero{\semK} \}
% \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% A \termBG grouping $\ggrouping(\gbAttrs,\rangeRel)$ for group-by attributes
% $\gbAttrs$ over relation $\rangeRel$ yields a set of distinct tuples with arity
% of $\gbAttrs$ by extracting \abbrBG values from non-zero annotated tuples of
% $\rangeRel$ projecting on $\gbAttrs$.  Next we associate with each group in
% $\ggrouping(\gbAttrs,\rangeRel)$ the set of all input tuples which may belong
% to the group in some possible world.
% % \label{sec:bound-pres-aggr}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Possible Tuple Grouping]
% Let $\aggregation{\gbAttrs}{f(A)}$ be an aggregation query. Consider a group $\agroup \in \ggrouping(\gbAttrs,\rangeRel)$. We define $\tgrouping(\agroup)$, the set of tuples from $\rangeRel$ associated with group $\agroup$, as shown below.
%   % use $\tgrouping(t_g)$ to denote the set of possible grouping tuples on a best guess grouping $t_g$, the group of tuples for aggregation on each best guess grouping can be defined as below.
% \begin{align*}
% 	\tgrouping(\agroup) = \{ \rangeTup | \agroup \tmatch \rangeTup.\gbAttrs  \}
% \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Both input tuples belong to $\tgrouping(\rangeTup_1)$
% and $\tgrouping(\rangeTup_2)$. Next, we construct the group-by range annotations for  an output tuple
% $\aout \in \stratGrps$.
% for each group $\agroup$ in $\ggrouping(\gbAttrs,\rangeRel)$.
% We define the construction of a tuple $\aout \in \stratGrps$ in two steps. First, we calculate
% bounds on the group-by values of $\aout$.
To ensure that all possible
groups an input tuple $\rangeTup$ with $\stratPoss(\rangeTup) = \aout$ belongs to are contained in
$\aout.\gbAttrs$ we have to merge the group-by attribute bounds of all
of these tuples. Furthermore, we set $\bgMarker(\aout.\gbAttrs)$ to the unique group $\agroup$ in \abbrBGW for all tuples $\rangeTup$ such that $\stratBG(\rangeTup) = \aout$.
%After we have a set of groupings. Each grouping need to consider all tuples possibly matches into account to form the group.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Range-bounded Groups]
Consider a result group $\asgrp \in \stratGrps(\gbAttrs, \rangeRel)$ for a grouping strategy $\gstrat$ and an aggregation with group-by attributes $\gbAttrs$ over a $\uaaK{\semK}$-relation $\rangeRel$. The bounds for the group-by attributes values of $\aout$ are defined as shown below. Let $\agroup$ be the unique element from the set $\{ \bgMarker{\rangeTup.\gbAttrs} \mid \bgMarker{\rangeRel(\rangeTup)} \neq \zeroK \wedge \stratBG(\rangeTup) = \aout \}$.
\begin{align*}
  \forall_{a \in \gbAttrs} & : \lbMarker{\aout.a} = \min_{\rangeTup: \stratPoss(\rangeTup) = \aout} \lbMarker{\rangeTup.a} \\
  \forall_{a \in \gbAttrs} & : \bgMarker{\aout.a} = \agroup.a \\
  \forall_{a \in \gbAttrs} & : \ubMarker{\aout.a} = \max_{\rangeTup: \stratPoss(\rangeTup) = \aout} \ubMarker{\rangeTup.a} \\
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that in the definition above, $\min$ and $\max$ are the minimum and maximum
wrt. to the order over the data domain $\dataDomain$ which we used to define
range-annotated values.  Reconsider the three example tuples and two result groups from above.
The group-by range annotation for output tuple $\outof{\agroup_1}$ is
$\uv{\min(1,2)}{2}{\max{2,4}} = \uv{1}{2}{4}$. Observe that $\uv{1}{2}{4}$ bounds
any group $\rangeTup_1$ and $\rangeTup_2$ may belong to in some possible world.
To calculate bounds on the result of an aggregation function for one group, we have to reason about the minimum and maximum possible aggregation function result based on the bounds of aggregation function input values, their row annotations, and their possible and guaranteed group memberships (even when a value of the aggregation function input attribute is certain the group membership of the tuple it belongs too may be uncertain). To calculate a conservative lower bound on the aggregation function result for an output tuple $\aout$, we use $\smbpair_{\uaaK{\semK},\monoid}$ to pair each tuple $\rangeTup$ with $\stratPoss(\rangeTup) = \asgrp)$ with its annotation and then extract the lower bound from the resulting range-annotated value.
For some tuples their  group membership is uncertain because either their group-by values are uncertain or they may not exist in all possible worlds (their certain annotation is $\zeroK$).
We take this into account by taking the minimum of the neutral element of the aggregation monoid and this value for such tuples. Towards this goal we introduce a predicate $\uncertg{\gbAttrs}{\rangeRel}{\rangeTup}$ that is defined as shown below.
\begin{align*}
  \uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \defas (\exists a \in \gbAttrs: \lbMarker{\rangeTup.a} \neq \ubMarker{\rangeTup.a}) \vee \lbMarker{\rangeRel(\rangeTup)} = \zeroK
\end{align*}
We then sum up the resulting values in the aggregation monoid. Note that here summation is assumed to  use addition in $\monoid$. % The result for each tuple belong to the group $\tgrouping(\agroup)$.
The upper bound calculation is analog (using the upper bound and maximum instead). The \abbrBG result is a calculated using standard $\semK$-relational semantics. In the definition we will use $\rangeTup \toverlaps \rangeTup'$ to denote that the range annotations of tuples $\rangeTup$ and $\rangeTup'$ with the same schema $(A_1, \ldots, A_n)$ overlap on each attribute $A_i$, i.e.,
\begin{align*}
\rangeTup \toverlaps \rangeTup' \defas \bigwedge_{i \in \{1, \ldots, n\}} [ \lbMarker{\rangeTup.A_i}, \ubMarker{\rangeTup.A_i} ] \cap  [ \lbMarker{\rangeTup'.A_i}, \ubMarker{\rangeTup'.A_i} ] \neq \emptyset
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Aggregation Function Result Bounds]
  Consider an output $\asgrp \in \stratGrps$ for a grouping strategy $\gstrat$, input $\rangeRel$, group-by attributes $\gbAttrs$, and aggregation function $f(A)$ with monoid $\monoid$.
  We use $\tgrouping(\asgrp)$ to denote the set of input tuples whose group-by attribute bounds overlap with $\aout.\gbAttrs$, i.e., they may be belong to a group represented by $\aout$:
  \begin{align*}
    \tgrouping(\asgrp) \defas \{ \rangeTup \mid \rangeRel(\rangeTup) \neq \uaaZero{\semK} \wedge \rangeTup.\gbAttrs \toverlaps \aout.\gbAttrs\}
  \end{align*}
  The bounds on the aggregation function result for tuple $\aout$ are defined as:
  \begin{align*}
  \lbMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}\\
  \lbagg{\rangeTup}     &= \begin{cases}
                            min(\amzero,\lbMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK},\monoid} \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \lbMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK},\monoid} \rangeTup.A)} &\mathtext{otherwise}\\
                          \end{cases}\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \bgMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \bgMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK},\monoid} \rangeTup.A)} \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \ubMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \ubagg{\rangeTup}\\
  \ubagg{\rangeTup}     &= \begin{cases}
                            max(\amzero,\ubMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK},\monoid} \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \ubMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK},\monoid} \rangeTup.A)}&\mathtext{otherwise}\\
                          \end{cases}
  % \lbMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}min(\amzero,\lbMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)}) \\
  %  \bgMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}\bgMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)} \\
  %  \ubMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}max(\amzero,\ubMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)}) \\
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
  For instance, consider calculating the sum of $A$ grouping on $B$ for a relation $R(A,B)$  which consists of two tuples $\rangeTup_3 \defas (\uv{3}{5}{10},\uv{3}{3}{3})$ and $\rangeTup_4 \defas (\uv{-4}{-3}{-3},\uv{2}{3}{4})$ which are both annotated with $(1,2,2)$ (appear certainly once and may appear twice). Consider calculating the aggregation function result bounds for the result tuple $\aout$ for the output group $\asgrp$ which  corresponds to \abbrBG group $\agroup \defas (3)$. The lower bound on {\upshape \lstinline!sum(A)!} is calculated as shown below:
  \begin{align*}
    &\sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}\\
    = &\lbMarker{\uv{3}{5}{10} \cdot (1,2,2)} + min(0, \lbMarker{\uv{-4}{-3}{-3} \cdot (1,2,2)})\\
    = &\lbMarker{\uv{3}{10}{20}} + min(0, \lbMarker{\uv{-8}{-6}{-3}})\\
    =&3 + min(0,-8) = -5
  \end{align*}
The aggregation result is guaranteed to be greater than or equal to $-5$ since $\rangeTup_3$ certainly belongs to $\agroup$ and at least contributions $3$ to the sum and $\rangeTup_4$ contributions at least $-8$. While it is possible that $\rangeTup_4$ does not belong to $\agroup$ this can only increase the final result ($3 + 0 > 3 + -8$).
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% As shown in the example above, we can tighten the bounds on aggregation function result if we take into account that some tuples certainly belong to a particular group (their group-by values are certain). This can be realized by only conditionally applying the minimum (maximum) operation in the calculation of the bounds when a tuple has uncertain group-by values.
% \BG{We apply this in our implementation? This should be cheap?}
% \BG{Should define a predicate that checks whether tuple's values are certain. Then this could be included into the definition without causing to much complexity increase.}
Having defined how each output tuple of aggregation is constructed we still need to calculate the row annotation for each result tuple. For aggregation without group-by there will be exactly one result tuple independent of what the input is.
In this case there exists a single possible and \abbrBG output group (the empty tuple $()$). Thus, any grouping strategy is bound to assign all \abbrBG input tuples to this one output through $\stratBG$ and all input tuples to this output through $\stratPoss$.   % $\ggrouping(\emptyset, \rangeRel)$ will consist of a single group $()$ containing all input tuples.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Aggregation Without Group-By]\label{def:aggr-op-semantics-wo-gb}
  Consider a query $\query \defas \aggregation{}{f(A)}(\rangeRel)$ and grouping strategy $\gstrat$. Let
$\gstrat(\emptyset,\rangeRel) = (\stratGrps, \stratBG, \stratPoss)$,
  and $\rangeTup$  be a range-annotated tuple with the same schema as $\query$ and $\asgrp$ denote the single output group in $\stratGrps$. Then
  \begin{align*}
    \lbMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    =     \bgMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    =     \ubMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    \\
    \defas \begin{cases}
      \oneK &\text{if}\,\,\, \rangeTup = \aout\\
      \zeroK & \text{otherwise}
    \end{cases}
  \end{align*}
% We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For aggregation with group-by we have to additionally determine the maximum number of distinct groups each output tuple could correspond to to calculate the upper bound on the possible annotation of a tuple. We compute the bound for an output $\aout$ based on $\ggrouping$ making the worst-case assumption that (i) each input tuple $\rangeTup$ from $\ggrouping(\asgrp)$ occurs with the maximal multiplicity possible ($\ubMarker{\rangeRel(\rangeTup)}$) and that each tuple $\tup$ encoded by $\rangeTup$ belongs to a separate group and (ii) that the set of groups produrrced from  two inputs $\rangeTup$ and $\rangeTup'$ do not overlap. We can improve this bound by partitioning the input into two sets: tuples with uncertain group-by attribute values and tuple's whose group membership is certain. For the latter we can compute the maximum number of groups for an output $\aout$ by simplying counting the number of groups using \abbrBG values for each input tuple that overlap with the group-by bounds of $\aout$. For the first set we still apply the worst-case assumption.
To determine the lower bound on the certain annotation of a tuple we have to reason about which input tuples certainly belong to the group. These are inputs whose group-by attributes are certain. For such tuples we sum up their tuple annotation lower bounds.
We then need to derive the annotation of a result tuple from the annotations of the relevant input tuples. For this purpose, \cite{AD11d} did extend semirings with an additional operator $\duprem_\semK$ which has to obey the laws $\duprem_\semK(\zeroK) = \zeroK$ and $\duprem_\semK(n\,\oneK) = \oneK$ for any $n \geq 1$. $\duprem_\semN$ and $\duprem_\semB$ are uniquely determined by theses laws: $\duprem_\semN(k) = 1$ if $k\neq 0$ and $\duprem_\semN(k) = 0$ otherwise; $\duprem_\semB(\btrue) = \btrue$ and $\duprem_\semB(\bfalse) = \bfalse$. However, for some semirings, these laws do not uniquely determine $\duprem_{\semK}$.\footnote{Geerts et al.~\cite{Geerts:2010bz} did introduce an alternative semantics for duplicate elimination for $\semK$-relations which is defined for semirings $\semK$ that are finitely generates (where each element can be derived by applying the operations of the semiring to  elements from a subset of $\semK$ called a "generator"). A separate duplicate elimination operator is defined for each element from a generator (which is assumed to be minimal). For instance, $\semNX$ the semiring of provenance polynomials is generated by $X$.}  % We lift $\duprem$ from $\semK$ to $\uaaK{\semK}$ by applying it pointwise.
For our purpose we require that $\duprem_{\semK}(k_1 \addK k_2) \ordK k_1 \addK k_2$. This is necessary for our upper tuple annotation bound to be correct.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Aggregation With Group-By]\label{def:aggr-op-semantics-gb}
  Consider a query $\query \defas \aggregation{\gbAttrs}{f(A)}(\rangeRel)$ and grouping strategy $\gstrat$. Let $\gsdef(\rangeRel,\gbAttrs) = (\stratGrps, \stratBG, \stratPoss)$.
% We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK \lbMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i} \vee \lbMarker{\rangeTup.a_1} \ordK \ubMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i}$. Using these predicates we define set difference as shown below.%

\begin{align*}
	\lbMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas
	\begin{cases}
      \duprem_{\semK}(\sum_{\rangeTup': \stratBG(\rangeTup') = \asgrp}\lbMarker{\rangeRel(\rangeTup')}) &\text{if } \exists \asgrp \in \stratGrps: \rangeTup = \aout\\
      % {\agroup \in \ggrouping(\gbAttrs,\rangeRel)}: \rangeTup = \aout(\agroup)\\
      % &\,\,\,\,\,\,\wedge \left( \sum_{\rangeTup' \in \tgrouping(\agroup)} \\
	\zeroK & \text{otherwise}
	\end{cases}\\
%%%%%%%%%%%%%%%%%%%%
  \bgMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas
	\begin{cases}
      \duprem_{\semK}(\sum_{\rangeTup': \stratBG(\rangeTup') = \asgrp} \bgMarker{\rangeRel(\rangeTup')}) &\text{if } \exists \asgrp \in \stratGrps: \rangeTup = \aout\\
      % &\wedge \left(  \right) \geqK \zeroK\\
	\zeroK & \text{otherwise}
  \end{cases}\\
  %max( \sum_{\bgMarker{\rangeTup.\gbAttrs} = \bgMarker{\rangeTup'.\gbAttrs}}\bgMarker{\rangeRel(\rangeTup')}\\
%%%%%%%%%%%%%%%%%%%%
     \ubMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas
\begin{cases}
\sum_{\rangeTup': \stratPoss(\rangeTup') = \asgrp}
% \duprem_{\semK}(
\ubMarker{\rangeRel(\rangeTup')} &\mathtext{if } \exists \asgrp \in \stratGrps: \rangeTup = \aout\\
  \zeroK &\text{otherwise}
\end{cases}
%%%%%%%%%%%%%%%%%%%%
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Optimizing Bounds}
% \label{sec:optimizing-bounds}

% The bounds provided by the  general aggregation semantics introduced above can be improved if we take the semantics of the aggregation function into account. In the following we provide better bounds for \aggsum, and \BG{What else?}

% unless the aggregation domain is extended to be symbolic expressions over semiring elements paired with monoid values combined by an abstract addition operation.


% hand demonstrated how to  keep the size of a query result polynomial in the input size of the query by representing the result of aggregation function results as symbolic expressions that pair semiring values with values of the aggregation domain. For instance, without going too much into technical detail, in semiring $\semNX$ the result of a sum aggregation may be $3 \otimes x_1 +_{sum} 2 \otimes x_2$ which intuitively means that the final result of the sum of value $3$ subject to variable $x_1$ and value $2$ subject to variable $x_2$.


% \BG{Is a a more general semantics we can define and then refine for tighter bounds? What about min/max?}

% \BG{Fix notation in the rewrites. Explain notation that is new (attribute names and such)}
% \BG{Define aggregation as an operator, not just aggregation function results}
% %\subsubsection{Row bounds}
% %

% We start with a more general form of the aggregation rule by using polynomial representations. In the real use cases we consider the limitation on the polynomial such that the polynomial can be evaluated into a concrete value.\SF{Do we?} In this case the definition of upper and lower bounds are clear.

% \BG{Not sure whether we need to reiterate this here, but keep it for now:}
% Recall that $\rangeTup[A]$ outputs projection of tuple $\rangeTup$ on a set of attributes $A$.

% \BG{Probably use $f(a)$ instead of $f$ to indicate what attribute we are aggregating over.}

% \BG{We still have to define the aggregation function result for a set of tuples to be able to restrict $\rangeTup$ to tuples that should be in the result instead of just tuples that have the right GB values.}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Aggregation Operator]\label{def:aggr-op-semantics}
% Let $\rangeTup$ and $\rangeTup'$ be range-annotated tuples where $\rangeTup$ has the same arity as $\aggregation{G}{f}(\rangeRel)$ and $\rangeTup'$ has the same arity as $\rangeRel$. Let $G$ be a set of group by attributes and $f$ be the aggregation function.  We define aggregation as shown below.
%    %We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK \lbMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i} \vee \lbMarker{\rangeTup.a_1} \ordK \ubMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i}$. Using these predicates we define set difference as shown below.%
%    \begin{align*}
% 	\lbMarker{\aggregation{G}{f}(\rangeRel)(\rangeTup)} &\defas
% 	\begin{cases}
% 	1_k & \text{if } \exists_{\rangeTup'}:\bgMarker{\rangeTup[G]}=\bgMarker{\rangeTup'[G]} \\
% 		& \text{ and } \forall_{a \in G}:\lbMarker{\rangeTup'.a}=\ubMarker{\rangeTup'.a} \\
% 		& \text{ and } \lbMarker{\combine(\rangeRel)(\rangeTup)} > 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 	\bgMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup)} &\defas \sum_{\bgMarker{\rangeTup[g]} = \bgMarker{\rangeTup'[g]}}\bgMarker{\combine(\rangeRel)(\rangeTup')}
% 	\end{align*}
% 	\begin{align*}
% 	\ubMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup)} &\defas \sum_{\rangeTup[g] \matches \rangeTup'[g]}\ubMarker{\combine(\rangeRel)(\rangeTup')}
% 	\end{align*}
% \end{Definition}

% \begin{Definition}[Aggregation group by attributes]\label{def:aggr-grpby-attr-semantics}
% 	With similar notations, we define aggregation group by attribute bounds as shown below.
% 	\begin{align*}
% 		\forall_{a \in g}:\lbMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup).a} &\defas \minOf{\rangeTup[G] \matches \rangeTup'[G]}\combine(\rangeRel)(\lbMarker{\rangeTup'.a}) \\
% 		\forall_{a \in g}:\ubMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup).a} &\defas \maxOf{\rangeTup[G] \matches \rangeTup'[G]}\combine(\rangeRel)(\ubMarker{\rangeTup'.a})
% 	\end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[General aggregation result attributes]\label{def:aggr-gen-attr-semantics}
% 	Define operator $\{k\}^{+}$ and $\{k\}^{-}$ over value $k$ s.t.
% 	\begin{align*}
% 		\{k\}^{+} =
% 	\begin{cases}
% 	k & \text{if } k \text{ contributes to } \ubMarker{f} \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 		\{k\}^{-} =
% 	\begin{cases}
% 	k & \text{if } k \text{ contributes to } \lbMarker{f} \text{ but not } \ubMarker{f} \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	Use $a_f$ to denote the attribute used by function $f$. We define general aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \lbMarker{f} \defas \\ & \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a_f}\}^+ \oplus \sum_{\rangeTup'[g] \matches \rangeTup[g]} \{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a_f}\}^- \\
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \bgMarker{f} \defas \\ & \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\bgMarker{a_f} \\
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \ubMarker{f} = \\ & \sum_{\rangeTup'[g] \matches \rangeTup[g]}\{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a_f}\}^+ \oplus \sum_{\rangeTup'[g] \equiv \rangeTup[g]} \{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a_f}\}^-
% 	\end{align*}

% \end{Definition}


% \begin{Definition}[Sum aggregation result attributes]\label{def:sum-aggr-attr-semantics}
% 	Define operator $\{k\}^{+}$ and $\{k\}^{-}$ over value $k \in \semK$ s.t.
% 	\begin{align*}
% 		\{k\}^{+} =
% 	\begin{cases}
% 	k & \text{if } k > 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 		\{k\}^{-} =
% 	\begin{cases}
% 	k & \text{if } k < 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	We define sum aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \lbMarker{sum(a)} \defas \\ & \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a}\}^+ + \sum_{\rangeTup'[g] \matches \rangeTup[g]} \{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a}\}^- \\
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \bgMarker{sum(a)} \defas \\ & \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\bgMarker{a} \\
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \ubMarker{sum(a)} = \\ & \sum_{\rangeTup'[g] \matches \rangeTup[g]}\{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a}\}^+ +\sum_{\rangeTup'[g] \equiv \rangeTup[g]} \{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a}\}^-
% 	\end{align*}

% \end{Definition}

% \begin{Definition}[Count aggregation result attributes]\label{def:Count-aggr-attr-semantics}
% 	For count function, all values may contribute to both upper and lower bounds and all attribute values is assigned to $1_k$. The semantics can be simplified. We define count aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \lbMarker{count(a)} \defas \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \bgMarker{count(a)} \defas \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \ubMarker{count(a)} \defas \sum_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}

% \end{Definition}

% \begin{Definition}[Min/Max aggregation result attributes]\label{def:MinMax-aggr-attr-semantics}
% 	For min/max function, all values may contribute to both upper and lower bounds, so the semantics can be simplified. We define Min/Max aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \lbMarker{min(a)} \defas \min_{\rangeTup'[g] \matches \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \bgMarker{min(a)} \defas \min_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \ubMarker{max(a)} \defas \min_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}
% 	\begin{align*}
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \lbMarker{max(a)} \defas \max_{\rangeTup'[g] \matches \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \bgMarker{max(a)} \defas \max_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \ubMarker{max(a)} \defas \max_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}
% \end{Definition}



% %\begin{enumerate}
% %%\item selection
% %%\[\lbMarker{[\selection_\theta(R)](t)}=\lbMarker{R(t)} \otimes \lbMarker{(\theta(t))} \]
% %%\[\ubMarker{[\selection_\theta(R)](t)}=\ubMarker{R(t)} \otimes \ubMarker{(\theta(t))} \]
% %%
% %%\item join
% %%\[ \lbMarker{[R_1 \join R_2](t)} = \lbMarker{R_1(t)} \otimes \lbMarker{R_2(t)} \]
% %%\[ \ubMarker{[R_1 \join R_2](t)} = \ubMarker{R_1(t)} \otimes \ubMarker{R_2(t)} \]
% %%
% %%\item Union
% %%\[ \lbMarker{[R_1 \union R_2](t)} =
% %%	\lbMarker{R_1(t)} \oplus  \lbMarker{R_2(t)}\]
% %%\[ \ubMarker{[R_1 \union R_2](t)} = \ubMarker{R_1(t)} \oplus \ubMarker{R_2(t)} \]
% %%
% %%\item Projection
% %%\[ \lbMarker{[\projection_{U}(R)](t)} = \sum_{t=t'[U]}\lbMarker{R(t')} \]
% %%\[ \ubMarker{[\projection_{U}(R)](t)} = \sum_{t=t'[U]}\ubMarker{R(t')} \]
% %%
% %%\item Set difference
% %%\[ \lbMarker{[R_1 - R_2](t)} = \lbMarker{R_1(t)} \ominus \sum_{R_1(t) \matches R_2(t')} \ubMarker{R_2(t')} \]
% %%\[ \ubMarker{[R_1 - R_2](t)} = \ubMarker{R_1(t)} \ominus \sum_{R_1(t) \equiv R_2(t')} \lbMarker{R_2(t')} \]
% %
% %%\subsubsection{Attribute bound}
% %%\begin{enumerate}
% %
% %%\item Union
% %%\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\lbMarker{a_i} = \min(R_1(t).\lbMarker{a_i},R_2(t).\lbMarker{a_i}) \]
% %%\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\ubMarker{a_i} = \max(R_1(t).\ubMarker{a_i},R_2(t).\ubMarker{a_i}) \]
% %%
% %%\item Projection
% %%\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]
% %%\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\ubMarker{a_i} = \max_{t=t'[U]} R(t').\ubMarker{a_i} \]
% %
% %
% %
% %\item Count Aggregation without group by
% %\[ [ \aggregation{}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{t' \in R}\lbMarker{R(t')} \]
% %\[ [ \aggregation{}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{t' \in R}\ubMarker{R(t')} \]
% %
% %\item Count Aggregation with group by
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]
% %
% %\[ [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{R(t')[g] \equiv t[g]}\lbMarker{R(t')} \]
% %\[ [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{R(t')[g] \matches t[g]}\ubMarker{R(t')} \]
% %
% %
% %\item Sum Aggregation without group by
% %\begin{align*}
% %[ & \aggregation{}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{t' \in R}\{\lbMarker{R(t')}*R(t').\lbMarker{A}\}^+ + \{\ubMarker{R(t')}*R(t').\lbMarker{A}\}^-
% %\end{align*}
% %\begin{align*}
% %[ & \aggregation{}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{t' \in R}\{\ubMarker{R(t')}*R(t').\ubMarker{A}\}^+ + \{\lbMarker{R(t')}*R(t').\ubMarker{A}\}^-
% %\end{align*}
% %
% %\item Sum Aggregation with group by
% %\[ [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{sum(A)} = \sum_{t' \in R, t[g] \in t'[g]}LB(R(t'))*R(t').\lbMarker{A} \]
% %\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]
% %\begin{align*}
% %[ & \aggregation{g}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{R(t')[g] \equiv t[g]}\{\lbMarker{R(t')}*R(t').\lbMarker{A}\}^+ + \\ & \sum_{R(t')[g] \matches t[g]} \{\ubMarker{R(t')}*R(t').\lbMarker{A}\}^-
% %\end{align*}
% %\begin{align*}
% %[ & \aggregation{g}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{R(t')[g] \matches t[g]}\{\ubMarker{R(t')}*R(t').\ubMarker{A}\}^+ + \\ & \sum_{R(t')[g] \equiv t[g]} \{\lbMarker{R(t')}*R(t').\ubMarker{A}\}^-
% %\end{align*}
% %
% %\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Examples}

The following example illustrates the application of the aggregation semantics we have defined in this section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}[Aggregation]\label{def:aggregation}
Consider the relation shown in \Cref{fig:AU-aggregation} which records addresses (street, street number, number of inhabitants). For the street attribute, instead of showing range annotations we mark values in red to indicate that their bound encompass the whole domain of the street attribute. Street values $v$ in black are certain $\lbMarker{v} = \bgMarker{v} = \ubMarker{v}$. In this example, we are uncertain about particular street numbers and the number of inhabitants at certain addresses. Furthermore, several tuples may represent more than one address. Finally, we are uncertain about the street for the address represented by the second tuple. Consider the aggregation query without group-by shown in \Cref{fig:AU-agg-example-no-GB}. We are calculating the number of inhabitants. In the \abbrBGW there are 7 inhabitants ($1 \cdot 1 + 2 \cdot 1 + 2 \cdot 2$).
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\centering

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|c|cc}
		\textbf{street}  & \textbf{number}          & \thead{\#inhab} & \underline{$\uaaK{\semN}$} \\
		\cline{1-4}
      \cMarker{Canal}    & $\uv{165}{165}{165}$     & $\uv{1}{1}{1}$  & (1,1,2)                    \\
%				\cline{1-3}
		\uMarker{Canal}  & $\uv{154}{153}{156}$     & $\uv{1}{2}{2}$  & (1,1,1)                    \\
%				\cline{1-3}
		\cMarker{State}  & $\uv{623}{623}{629}$     & $\uv{2}{2}{2}$  & (2,2,3)                    \\
		\cMarker{Monroe} & $\uv{3574}{3550}{3585}$  & $\uv{2}{3}{4}$  & (0,0,1)                    \\
%				\cline{1-3}
	\end{tabular}
	\caption{Input Relation address}
        \label{fig:AU-agg-example-input}
  \end{subtable}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subtable}{\linewidth}
	\centering
\begin{lstlisting}
SELECT sum(#inhab) AS pop FROM address;
\end{lstlisting}
	\begin{tabular}{ cc}
%				\cline{1-2}
 \textbf{pop}   & \underline{$\uaaK{\semN}$} \\
\cline{1-1}
 $\uv{6}{7}{14}$ & (1,1,1)                    \\
%				\cline{1-2}
	\end{tabular}
	\caption{Aggregation without Group-by}
    \label{fig:AU-agg-example-no-GB}
  \end{subtable}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subtable}{\linewidth}
	\centering
\begin{lstlisting}
SELECT street, count(*) AS cnt
FROM address GROUP BY street;
\end{lstlisting}
	\begin{tabular}{ c|cc}
			%	\cline{1-2}
		\textbf{street}  & \textbf{cnt}   & \underline{$\uaaK{\semN}$} \\
		\cline{1-2}
		\uMarker{Canal}  & $\uv{1}{2}{3}$ & (1,1,2)                    \\
		\cMarker{State}  & $\uv{2}{2}{4}$ & (1,1,1)                    \\
		\cMarker{Monroe} & $\uv{1}{1}{2}$ & (0,0,1)                    \\
			%	\cline{1-2}
	\end{tabular}
    \caption{Aggregation with Group-by}
    \label{fig:AU-agg-example-GB}
  \end{subtable}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\caption{Aggregation over \abbrUAADBs}
\label{fig:AU-aggregation}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preservation of bounds}

We now demonstrate that our aggregation semantics for \abbrUAADBs is bound-preserving.
\BG{Have to say something more, or this is ok?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}\label{theo:aggregation-preserves-bounds}
Let $\query \defas \aggregation{\gbAttrs}{f(A)}(\rel)$ and $\prel$ be an incomplete $\semK$-relation that is bound by an $\uaaK{\semK}$-relation $\rangeRel$. Then $\query(\rangeRel)$ bounds $\query(\prel)$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
\BG{TODO}
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

From \Cref{theo:aggregation-preserves-bounds}\iftechreport{, \Cref{theo:set-difference-prese},}\ifnottechreport{,\cite[Theorem X]{techreport} (bound preservation for set difference)} and \Cref{lem:ra-plus-preserves-bounds} follows our main technical result: Our query semantics for $\raAgg$ queries preserves bounds.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Corollary}[Preservation of bounds for $\raAgg$]\label{cor:preservation-of-boun}
  Let $\query$ be an $\raAgg$ query and $\pdb$ an incomplete $\semK$-database that is bound by an $\uaaK{\semK}$-database $\rangeDB$. Then $\query(\rangeDB)$ bounds $\query(\pdb)$.
  $$ \pdb \dbbounds \rangeDB \Rightarrow \query(\pdb) \dbbounds \query(\rangeDB)$$
\end{Corollary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}

% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "tech_report"
%%% End:


==> uaa-aggregation.tex <==
%!TEX root=./uaadb.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Aggregation}\label{sec:aggregation}

We now introduce a bound preserving semantics for aggregation over $\uaaN$-relations
that is based on results from~\cite{AD11d} that we review below. \revm{We leave a generalization to other semirings to future work. See~\cite{techreport} for a discussion of the challenges involved with that. Importantly, our semantics has \ptime data complexity.}
% The semantics of~\cite{AD11d}
% % One major challenge in defining aggregation over $\semK$-relations
% % which also applies to our problem setting is that one has to
% takes tuple annotations into account when calculating aggregation function
% results. For instance, under bag semantics (semiring $\semN$) the multiplicity
% of a tuple affects the result of $\aggsum$ aggregation.
% However, additional complications arise for $\uaaN$-relations, because the techniques from~\cite{AD11d} are not directly applicable and we have to deal with uncertain group memberships.


% of tuples across possible worlds.
% For \abbrUAADBs we have to overcome two major new challenges: (i)
% since the values of group-by attributes may be uncertain, a tuple's group
% membership may be uncertain too and (ii) we are aggregating over range-bounded
% values.
% To address (ii) we  utilitze our expression semantics for
% range-bounded values from \Cref{sec:expression}. However, additional
% complications arise when taking the $\uaaK{\semN}$-annotations of tuples into
% account. For (i) we will reason about all possible group memberships of
% range-annotated tuples to calculate bounds on group-by values, aggregation
% function results, and number of result groups.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Background}
% \label{sec:background-1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Aggregation Monoids}
%
The semantics for aggregation queries
over $\semK$-relations from~\cite{AD11d} deals with aggregation functions that
are commutative monoids $\tuple{\monoid, \amadd, \amzero}$, i.e., where
the values from
$\monoid$ that are the input to aggregation are combined through an operation
$\amadd$ which has a neutral element $\amzero$. \revm{Abusing notation, we will use $\monoid$ to both denote the monoid and its domain.}
% \footnote{A monoid is a
  % mathematical structure $(\monoid, \amadd, \amzero)$ where $\amadd$ is a
  % commutative and associative binary operation over $\monoid$, and $\amzero$ is
  % the neutral element of $\monoid$. For instance,
  % $\msum \defas (\mathbb{R}, +, 0)$, i.e., addition over the reals can be used
  % for sum aggregation.}
Standard aggregation functions \aggsum, \aggmin, \aggmax, and \aggcount are
monoids. \aggavg can be derived from \aggsum and \aggcount. % (\msum and
% \aggsum).
As an example, consider the monoids for $\aggsum$ and $\aggmin$:
$\msum \defas \tuple{\mathbb{R}, +, 0}$ and $\mmin \defas \tuple{\mathbb{R}, \min,
\infty}$.
%The result of aggregation over a set of $\monoid$ values is defined as the sum of these values in  $\monoid$.
For $\monoid \in \{\msum, \mmin, \mmax\}$ (\aggcount uses \msum), we define a corresponding monoid  $\rangeMon$ using
range-annotated expression semantics (\Cref{sec:expression}). \revm{Note that this gives us aggregation functions which can be applied to range-annotated values and are bound preserving, i.e., the result of the aggregation function bounds all possible results for any set of values bound by the inputs.}
For example, $\aggmin$ is expressed as $\min(v,w) \defas \ifte{v \leq w}{v}{w}$.
% we can define  $\monoid$
% ($\msum$)
% Note that bound-preserving evaluation of these monoids over
% range-annotated values is already supported though the range-annotated
% expression semantics from \Cref{sec:expression}.
% For instance, $\msum$ simply
%uses the addition operation we defined.
% Even though we did not define $\aggmin$
% and $\aggmax$ explicitly, we can express them using the operators
%  from~\Cref{sec:expression}, e.g., $\min(v,w) \defas \ifte{v \leq w}{v}{w}$. In
%  the following, we use $\rangeMon$ to denote the range-annotated version of
%  $\monoid$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}\label{lem:range-annotated-monoids}
$\rangeMof{\msum}$, $\rangeMof{\mmin}$, $\rangeMof{\mmax}$ are monoids.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  Proven by unfolding of definitions to show that the addition operations of these monoids is  pointwise application of the operation of the monoids they originated from.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Based on \Cref{lem:range-annotated-monoids} we have that aggregation functions
% over range-annotated values preserve bounds.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
%   \centering
%   \begin{align}
%     k \smbN{\monoid} (m_1 \amadd m_2) & = k \smbN{\monoid} m_1 \amadd k \smbN{\monoid} m_2 \label{eq:semimodule-distributes-over-m-plus}\\
%     % (k_1 \addN k_2) \smbN{\monoid} m  & = k_1 \smbN{\monoid} m \amadd k_2 \smbN{\monoid} m \\
%     % \oneN \smbN{\monoid} m            & = m                                                    \\
%     % \zeroN \smbN{\monoid} m           & = \amzero            \label{eq:semimodule-with-m-zero-yields-m-zero}                                  \\
%     k \smbN{\monoid} \amzero          & = \amzero                                              %\\
%     % (k_1 \multN k_2) \smbN{\monoid} m & = k_1 \smbN{\monoid} (k_2 \smbN{\monoid} m)
%   \end{align}\\[-3mm]
%   \caption{Semimodule laws excerpt (semiring $\semN$, monoid $\monoid$)}
%   \label{fig:semimodule-laws}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Semimodules}
%
Aggregation over
$\semK$-relations  has to take the annotations of tuples into account for computing
aggregation results. For instance, consider an $\semN$-relation $R(A)$ with
tuples $\tuple{30} \mapsto 2$ and $\tuple{40} \mapsto 3$, (i.e., respectively 2 and 3 duplicates).
The sum over $A$ should be $30 \cdot 2 + 40 \cdot 3 = 180$.
More generally speaking, we
need an operation $\smbpair_{\monoid}: \semN \times \monoid \rightarrow \monoid$
that combines the tuple multiplicities with domain values.
As observed in~\cite{AD11d}
this operation has to fulfill the algebraic laws of semimodules. %, i.e., it has to fulfill a set of algebraic laws. % , two of which are shown for $\semN$ in \Cref{fig:semimodule-laws}.
% \BGdel{Note that in the example above we made use of the fact that
% $\smbN{\msum}$ is $\cdot$ to get
% $30 \smbN{\msum} 2 = 30 \cdot 2 = 60$.}
% In the following, we will use $\smbpair_{\monoid}$ to denote $\smbN{\monoid}$.
Note that  $\smbpair$ is  well-defined % for
% all semirings, but it is defined
for $\semN$ and all of the monoids we consider:\\[-3mm]
% We discuss the general case in \cite{techreport}.
%We show the definition for $\smbN{\monoid}$ for all considered monoids below:
%
\begin{align*}
  k \smbN{\msum} m                        & = k \cdot m             &
  k \smbN{\mmin} m = k \smbN{\mmax} m & =
  \begin{cases}
    m                                         & \text{if}\,\,\,k \neq 0 \\
    0                                         & \text{else}             \\
  \end{cases}
\end{align*}

\revm{Unfortunately, as the following lemma shows, it is not possible to use semimodules for aggregation over $\uaaN$-relations, because such semimodules, if they exist, cannot be bound preserving.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Applying Semimodules to $\uaaK{\semN}$-Relations}
% \label{sec:semim-uaaks-relat}


\BG{DEL: As we will demonstrate, even though it may be possible to
define $\uaaN$-semimodules, such semimodules cannot be bound preserving.
% and, thus, would be useless for our purpose.
We show that it is
possible to define bound preserving operations $\mysmbNAU{\monoid}$ that combine $\uaaN$
elements with $\rangeDom$ elements and that this is sufficient for defining a
bound preserving aggregation semantics.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}\label{lem:bound-preserving-impossible}
$\smbpair_{\uaaK{\semN},\msum}$, if it is well-defined, is not bound preserving.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  Assume that this semimodule exists and is bound preserving. We lead this assumption to a contradiction by deriving two different results for the expression $\ut{1}{1}{2} \smbNAU{\msum} \uv{0}{0}{0}$ using semimodule laws: (i) the obvious $\uv{0}{0}{0}$ and (ii) $\uv{-1}{0}{1} = \ut{1}{1}{2} \smbNAU{\msum} (\uv{-1}{-1}{-1} \addN \uv{1}{1}{1})$
  (full proof in \cite{techreport}).
  %show in \Cref{fig:semimodule-laws} under the assumption that the inputs are bounded .
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iftechreport{Intuitively, an aggregate's bounds may be affected by order of operations, becoming weaker than strictly necessary.
While a stronger constraint is not efficiently enforceable, we can still require that the aggregate preserve bounds.
A naive non-semimodule definition of $\amysmbNAU$ might use point-wise application of
$\smbN{\monoid}$. However, this does not always preserve bounds. For instance, consider sum
aggregation ($\msum$) over
a $\uaaK{\semN}$-relation $\rangeRel(A)$ with a single tuple $\tuple{\uv{-3}{-2}{-1}}$
with annotation $\ut{0}{1}{1}$ and query $\aggnogb{sum(A)} (R)$. If
$\mysmbNAU{\msum}$ would be defined as point-wise application of
$\smbN{\msum}$, then the result of aggregation would be
$\uv{-3 \cdot 0}{-2 \cdot 1}{-1 \cdot 1} = \uv{0}{-2}{-1}$ which is not a
valid range-annotated value because $0 > -2$.
}
% The reason why point-wise application fails is that $\smbN{\msum}$
% does not preserve the order of the domain $\dataDomain$ based on which we
% defined range-annotated values.
% As we already saw in \Cref{sec:range-expr-eval},
% that multiplication over $\rangeDom$ cannot be defined pointwise to preserve
% bounds.
\revm{In spite of this negative result, not everything is lost. Observe that it not necessary for the operation that combines semiring elements (tuple annotations) with elements of the aggregation monoid to follow semimodule laws. After all, what we care about is that the operation is bound-preserving.
Below we define operations $\mysmbNAU{\monoid}$ that are not semimodules, but are bound-preserving.
To achieve bound-preservation we can rely on the bound-preserving expression semantics we have defined in~\Cref{sec:expression}.
For example, }
% We show that it is
% possible to define bound preserving operations $\mysmbNAU{\monoid}$ that combine $\uaaN$
% elements with $\rangeDom$ elements and that this is sufficient for defining a
% bound preserving aggregation semantics.
since $\smbN{\msum}$ is multiplication, we can define
$\mysmbNAU{\msum}$ using multiplication for range-annotated values. % \revm{which we did already prove to be bound preserving}.
This approach of computing the bounds as the  minimum and maximum over all pair-wise combinations of value and tuple-annotation bounds also works for $\mmin$ and $\mmax$.
In~\cite{techreport} we prove that $\amysmbNAU$ is in fact bound preserving.
% The idea applied in
% the definition below is the same as uses in the definition of multiplication
% over range-annotated values: evaluate $\smbpair_{\semK,\monoid}$ over all
% combinations of values from the input and then return the minimum and maximum
% values over this set as bounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:range-semimodules}
  Consider a monoid $\monoid \in \{\msum, \mmin, \mmax\}$. % such that $\smbN{\monoid}$ is well defined.
  Let $\uv{\lbMarker{m}}{m}{\ubMarker{m}}$ be a range-annotated value from $\rangeDom$ and $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \in \uaaK{\semN}$.
  %Let triple  that  the value domain. Let triple $\semNX^3=(\lbMarker{x},x,\ubMarker{x})$ denote a tuple annotation value in \abbrAUDB.
We define $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \amysmbNAU \uv{\lbMarker{m}}{m}{\ubMarker{m}} =$
%  We define $\amysmbNAU$ as shown below. % range aggregation monoid multiplication computation yields a triple as below.
  % \begin{flalign*}
  %     \ut{\lbMarker{k}}{k}{\ubMarker{k}} \amysmbNAU \uv{\lbMarker{m}}{m}{\ubMarker{m}} =
  % \end{flalign*}
%%%%%%%%%%%%%%%%%%%%
  \begin{align*}
		[& min(\lbMarker{k} \smbN{\monoid} \lbMarker{m},\lbMarker{k} \smbN{\monoid} \ubMarker{m},\ubMarker{k} \smbN{\monoid} \lbMarker{m},\ubMarker{k} \smbN{\monoid} \ubMarker{m}), \\
		& {k} \smbN{\monoid} {m}, \\
		& max(\lbMarker{k} \smbN{\monoid} \lbMarker{m},\lbMarker{k} \smbN{\monoid} \ubMarker{m},\ubMarker{k} \smbN{\monoid} \lbMarker{m},\ubMarker{k} \smbN{\monoid} \ubMarker{m})]
	\end{align*}

\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Note that, in general there is no guarantee that
% $\smbpair_{\uaaK{\semK},\monoid}$ according to \Cref{def:range-semimodules}
% preserves bounds. However,


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Lemma}\label{theo:uaa-semimodules-preserve-bounds}
% $\amysmbNAU$ is bound preserving for $\monoid \in \{\mmin, \mmax, \msum\}$. % we have that .
% \end{Lemma}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}[Proof Sketch]
% We have to show for all $\monoid \in \{\mmin, \mmax, \msum\}$ that for any $\vec{k} = \ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}} \in \uaaK{\semN}$ and $\vec{m} = \uv{\lbMarker{m}}{\bgMarker{m}}{\ubMarker{m}} \in \rangeDom$ we have that $\vec{k} \amysmbNAU \vec{m}$ bounds $k \smbN{\monoid} m$ for any $k$ bound by $\vec{k}$ and $m$ bound by $\vec{m}$. The claim is proven by substitution of definitions and case distinctions (are the annotation bounds $0$ or not and are one or both bounds of $\vec{m}$ negative). See~\cite{techreport} for the full proof.
% \end{proof}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bound-Preserving Aggregation}
\label{sec:bound-pres-aggr}
We now define a bound preserving aggregation semantics based on the
$\amysmbNAU$ operations. % As mentioned above, the main
% challenge we have to overcome is to deal with the uncertainty of group
% memberships plus the resulting uncertainty in the number of groups and of which
% inputs contribute to a group's aggregation function result values.
% In general,
% the number of possible groups encoded by an input \abbrUAADB-relation may be
% very large.
% Thus, enumerating all concrete groups is not a viable option.  While
Since \abbrUAADBs can be used to encode an arbitrary number of groups as a single
tuple, we need to decide how to trade conciseness of the representation for
accuracy. Furthermore, we need to ensure that the aggregation result in the
\abbrBGW is encoded by the result. There are many possible strategies for how to
group possible aggregation results. In this paper, we limit the discussion to a default strategy  that we introduce next (see~\cite{techreport} for a general treatment). % we formalize grouping strategies and define a semantics for aggregation that preserves bounds for any such grouping semantics.
% We define our aggregation semantics in three steps: (i) we introduce our default grouping strategy that matches \abbrBG and possible input groups to output tuples (each output tuple will represent exactly one group in the  \abbrBGW and one or more possible groups);
Afterwards,  we demonstrate how to calculate group-by attribute and aggregation result ranges for output tuples.
% based on the assignment of input tuples to output tuples; (iii) we calculate the multiplicities and bounds for aggregation function results for each output tuple. % based on the grouping strategy.


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Grouping Strategy}
Our \textit{grouping strategy}
takes as input an n-ary $\uaaK{\semN}$-relation $\rangeRel$ and a list of group-by attributes $\gbAttrs$ and returns a pair $(\stratGrps, \stratPoss)$ where $\stratGrps(\gbAttrs, \rangeRel)$ is a set of output tuples --- one for every \abbrBG group (an input tuple's group-by values in the \abbrBGW), and
$\stratPoss$ assigns each input tuple to one output based on its \abbrBG group-by values.
Even if the \abbrBG annotation of an input tuple is $0$, we still use its \abbrBG values
  to assign it to an output tuple.
  Only tuples that are not possible (annotated with $\uaaZero{\semN} = \ut{0}{0}{0}$) are not considered.
  \revm{Since output tuples are identified by their \abbrBG group-by values, we will use these values to  identify elements from $\stratGrps$.}
  % All possible groups of an input tuple are associated with the output that corresponds to the tuple's group-by values in the \abbrBGW.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{Definition}% [Default Grouping Strategy]
    \label{def:default-grouping-strategy}
Consider a query $\query \defas \aggregation{\gbAttrs}{f(A)}(\rangeRel)$.
  Let $\rangeTup \in \rangeDom^n$. % such that $\rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semN}}$ and $\rangeTup' \in \rangeDom^n$ such that $\bgMarker{\rangeRel(\rangeTup')} \neq \zeroN$.
 The default grouping strategy $\gsdef \defas (\gsdefG,  \gsdefP)$ is defined as:
\begin{align*}
 \gsdefG(\gbAttrs, \rangeRel)                      & \defas  \{ t.\gbAttrs \mid \exists \rangeTup: \bgMarker{\rangeTup} = t \wedge \rangeRel(\rangeTup) \neq \uaaZero{\semN} \} &
  % \gsdefBG(\rangeTup')        & \defas \bgMarker{\rangeTup'.\gbAttrs}  &
  \gsdefP(\rangeTup)          & \defas \bgMarker{\rangeTup.\gbAttrs}
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Note that one range-annotated input tuple may belong to multiple groups since
% its group-by values may bound multiple \abbrBG groups.
For instance, consider
three tuples $\rangeTup_1 \defas \tuple{\uv{1}{2}{2}}$ and
$\rangeTup_2 \defas \tuple{\uv{2}{2}{4}}$ and $\rangeTup_3 \defas \tuple{\uv{2}{3}{4}}$ of a relation $\rangeRel(A)$.
Furthermore, assume that $\rangeRel(\rangeTup_1) = \ut{1}{1}{1}$, $\rangeRel(\rangeTup_2) = \ut{0}{0}{1}$, and
$\rangeRel(\rangeTup_3) = \ut{0}{0}{3}$.
Grouping on $A$,
the default strategy will generate  two output groups $\agroup_1$ for \abbrBG group $(2)$ and
$\agroup_2$ for \abbrBG group $(3)$.
% Tuple $\rangeTup_1$ is the only tuple that is present in the \abbrBGW. Function $\gsdefBG$ assigns $\rangeTup_1$ to $\agroup_1$.
Based on their \abbrBG group-by values, $\gsdefP$ assigns $\rangeTup_1$ and $\rangeTup_2$ to $\agroup_1$ and $\rangeTup_3$ to $\agroup_2$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Aggregation Semantics}
%
We now introduce an aggregation semantics based on this grouping strategy.  For
simplicity we define aggregation without group-by as a special case of
aggregation with group-by (the only difference is how tuple annotations are
handled). We first define how to construct a result tuple $\aout$ for each
output group $\asgrp$ returned by the grouping strategy and then present how to
calculate tuple annotations. The construction of an output tuple is divided into
two steps: (i) determine range annotations for the group-by attributes and (ii)
determine range annotations for the aggregation function result attributes.  To
ensure that all possible groups that an input tuple $\rangeTup$ with
$\gsdefP(\rangeTup) = \asgrp$ belongs to are contained in $\aout.\gbAttrs$ we
have to merge the group-by attribute bounds of all of these tuples. Furthermore,
we use the unique \abbrBG group-by values common to all input tuples assigned to $\aout$ (i.e., $\bgMarker{\aout.\gbAttrs} = \asgrp$) \revm{as the output's \abbrBG group-by value.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Range-bounded Groups]
  \label{def:range-bounded-groups}
Consider a result group $\asgrp \in \gsdefG(\gbAttrs, \rangeRel)$ for an aggregation with group-by attributes $\gbAttrs$ over a $\uaaK{\semN}$-relation $\rangeRel$. The bounds for the group-by attributes values of $\aout$ are defined as shown below. % Let $\agroup$ be the unique element from the set $\{ \bgMarker{\rangeTup.\gbAttrs} \mid \bgMarker{\rangeRel(\rangeTup)} \neq 0 \wedge \stratPoss(\rangeTup) = \aout \}$.
For all $a \in \gbAttrs$ we define:\\[-5mm]
%%%%%%%%%%%%%%%%%%%%
\begin{align*}
\lbMarker{\aout.a} &= \min_{\rangeTup: \stratPoss(\rangeTup) = \asgrp} \lbMarker{\rangeTup.a} &
\bgMarker{\aout.a} &= \agroup.a &
\ubMarker{\aout.a} &= \max_{\rangeTup: \stratPoss(\rangeTup) = \asgrp} \ubMarker{\rangeTup.a}
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that in the definition above, $\min$ and $\max$ are the minimum and maximum
wrt. to the order over the data domain $\dataDomain$ which we used to define
range-annotated values.  Reconsider the three example tuples and two result groups from above.
The group-by range annotation for output tuple $\outof{\agroup_1}$ is
$\uv{\min(1,2)}{2}{\max(2,4)} = \uv{1}{2}{4}$. Observe that $\uv{1}{2}{4}$ bounds
every group $\rangeTup_1$ and $\rangeTup_2$ may belong to in some possible world.
To calculate bounds on the result of an aggregation function for one group, we have to reason about the minimum and maximum possible aggregation function result based on the bounds of aggregation function input values, their associated row annotations, and their possible and guaranteed group memberships. % Even when an aggregation function input value is certain, which group the tuple belongs may be uncertain.
To calculate a conservative lower bound of the aggregation function result for an output tuple $\aout$, we use $\amysmbNAU$ to pair the aggregation function value of each tuple $\rangeTup$ for which $\stratPoss(\rangeTup) = \asgrp$ holds with the tuple's annotation and then extract the lower bound from the resulting range-annotated value.
The group membership of a contributing tuple is uncertain if either its group-by values are uncertain or if it need not exist in all possible worlds (its certain multiplicity is $0$).
We thus take the minimum of the neutral element of the aggregation monoid and the result of $\amysmbNAU$ for such tuples. We introduce an \emph{uncertain group} predicate $\uncertg{\gbAttrs}{\rangeRel}{\rangeTup}$ for this purpose:\\[-5mm]
% that is defined as shown below.
%
\begin{align*}
  \uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \defas (\exists a \in \gbAttrs: \lbMarker{\rangeTup.a} \neq \ubMarker{\rangeTup.a}) \vee \lbMarker{\rangeRel(\rangeTup)} = 0
\end{align*}
%
We then sum up the resulting values in the aggregation monoid. Note that here summation is addition in $\monoid$. % The result for each tuple belong to the group $\tgrouping(\agroup)$.
The upper bound calculation is analogous (using the upper bound and maximum instead). The \abbrBG result is calculated using standard $\semN$-relational semantics. We use $\rangeTup \toverlaps \rangeTup'$ to denote that the range annotations of tuples $\rangeTup$ and $\rangeTup'$ with the same schema $(A_1, \ldots, A_n)$ overlap on each attribute $A_i$, i.e.,\\[-4mm]
%
\begin{align*}
\rangeTup \toverlaps \rangeTup' \defas \bigwedge_{i \in \{1, \ldots, n\}} [ \lbMarker{\rangeTup.A_i}, \ubMarker{\rangeTup.A_i} ] \cap  [ \lbMarker{\rangeTup'.A_i}, \ubMarker{\rangeTup'.A_i} ] \neq \emptyset
\end{align*}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Aggregation Function Result Bounds]
  \label{def:agg-function-bounds}
  Consider input $\rangeRel$, set of group-by
  attributes $\gbAttrs$, an output $\asgrp \in \gsdefG(\gbAttrs, \rangeRel)$,
  and aggregation function $f(A)$ with monoid $\monoid$.
  We use $\tgrouping(\asgrp)$ to denote the set of inputs with group-by
  attribute bounds overlaping $\aout.\gbAttrs$, i.e., belonging to a
  group represented by $\aout$:\\[-5mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    \tgrouping(\asgrp) \defas \{ \rangeTup \mid \rangeRel(\rangeTup) \neq \uaaZero{\semN} \wedge \rangeTup.\gbAttrs \toverlaps \aout.\gbAttrs\}
  \end{align*}
  %%%%%%%%%%%%%%%%%%%%
  The aggregation function result bounds for tuple $\aout$ are defined as: \\[-3mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    \lbMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}
  &\ubMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \ubagg{\rangeTup}
  \end{align*}\\[-6mm]
  \begin{align*}
     \bgMarker{\aout.f(A)} &= \sum_{\rangeTup \in \tgrouping(\asgrp)} \bgMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}
  \end{align*}\\[-6mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
  \lbagg{\rangeTup}     &= \begin{cases}
                            min(\amzero,\lbMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \lbMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)} &\mathtext{otherwise}\\
                          \end{cases}\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \ubagg{\rangeTup}     &= \begin{cases}
                            max(\amzero,\ubMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}) &\mathtext{if }\uncertg{\gbAttrs}{\rangeRel}{\rangeTup} \\
                            \ubMarker{(\rangeRel(\rangeTup) \amysmbNAU \rangeTup.A)}&\mathtext{otherwise}\\
                          \end{cases}
  % \lbMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}min(\amzero,\lbMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)}) \\
  %  \bgMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}\bgMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)} \\
  %  \ubMarker{\aout(\agroup).f(A)} &= \sum_{\rangeTup.\gbAttrs \tmatch \aout(\agroup).\gbAttrs}max(\amzero,\ubMarker{(\rangeRel(\rangeTup) \smbpair_{\uaaK{\semK}} \rangeTup.A)}) \\
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
  For instance, consider calculating the sum of $A$ grouping on $B$ for a relation $R(A,B)$, which consists of two tuples $\rangeTup_1 \defas \tuple{\uv{3}{5}{10},\uv{3}{3}{3}}$ and $\rangeTup_2 \defas \tuple{\uv{-4}{-3}{-3},\uv{2}{3}{4}}$ that are both annotated with \ut{1}{2}{2} (appear certainly once and may appear twice). Consider calculating the aggregation function result bounds for the result tuple $\aout$ for the output group $\asgrp \defas \tuple{3}$. The lower bound $\sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}$ on {\upshape \lstinline!sum(A)!} is calculated (\Cref{def:range-semimodules}) as:
  \begin{align*}
    % &\sum_{\rangeTup \in \tgrouping(\asgrp)} \lbagg{\rangeTup}\\
    = &\lbMarker{\left(\ut{1}{2}{2} \cdot \uv{3}{5}{10}  \right)} + min(0, \lbMarker{\left(\ut{1}{2}{2} \cdot \uv{-4}{-3}{-3}\right)})\\
    = &\lbMarker{\uv{3}{10}{20}} + min(0, \lbMarker{\uv{-8}{-6}{-3}})
    =3 + min(0,-8) = -5
  \end{align*}
The aggregation result is guaranteed to be greater than or equal to $-5$ since $\rangeTup_1$ certainly belongs to $\asgrp$   \revc{(no minimum operation), because its group-by attribute value $\uv{3}{3}{3}$ is certain and the tuple certainly exists ($\lbMarker{\ut{1}{2}{1}} > 0$). This tuple} contributes $3$ to the sum and $\rangeTup_2$ contributions at least $-8$. While it is possible that $\rangeTup_2$ does not belong to $\asgrp$ this can only increase the final result ($3 + 0 > 3 + -8$).
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% As shown in the example above, we can tighten the bounds on aggregation function result if we take into account that some tuples certainly belong to a particular group (their group-by values are certain). This can be realized by only conditionally applying the minimum (maximum) operation in the calculation of the bounds when a tuple has uncertain group-by values.
% \BG{We apply this in our implementation? This should be cheap?}
% \BG{Should define a predicate that checks whether tuple's values are certain. Then this could be included into the definition without causing to much complexity increase.}
We still need to calculate the multiplicity annotation for each result tuple. For aggregation without group-by, there is always exactly one result tuple.
In this case there exists a single possible \abbrBG output group (the empty tuple \revm{$\tuple{}$} ) and all input tuples are assigned to it through $\gsdefP$. Let \revm{$\rangeTup_{\tuple{}}$} denote this single output tuple.
Recalling that all remaining tuples have multiplicity $\zeroN$, we define:  % $\ggrouping(\emptyset, \rangeRel)$ will consist of a single group $()$ containing all input tuples.
  \begin{align*}
    \lbMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    =     \bgMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    =     \ubMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
    \defas \begin{cases}
      \oneN &\text{if}\,\,\, \rangeTup = \revm{\rangeTup_{\tuple{}}}\\
      \zeroN & \text{otherwise}
    \end{cases}
  \end{align*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Aggregation Without Group-By]\label{def:aggr-op-semantics-wo-gb}
%   Consider a query $\query \defas \aggregation{}{f(A)}(\rangeRel)$. Let
% $\gsdef(\emptyset,\rangeRel) = (\gsdefG, \gsdefP)$,
%   and $\rangeTup$  be a range-annotated tuple with the same schema as $\query$ and $\asgrp$ denote the single output group in $\gsdefG$. Then
%   \begin{align*}
%     \lbMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
%     =     \bgMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
%     =     \ubMarker{\aggregation{}{f(A)}(\rangeRel)(\rangeTup)}
%     \defas \begin{cases}
%       \oneN &\text{if}\,\,\, \rangeTup = \aout\\
%       \zeroN & \text{otherwise}
%     \end{cases}
%   \end{align*}
% % We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to calculate the upper bound on the possible \revm{multiplicity for a result tuple of a group-by aggregation}, we have to determine the maximum number of distinct groups this output tuple could correspond to.
We compute the bound for an output $\aout$ based on $\ggrouping$ making the worst-case assumption that
(i) each input tuple $\rangeTup$ with $\gsdefP(\rangeTup) = \asgrp$ has the maximal multiplicity possible ($\ubMarker{\rangeRel(\rangeTup)}$);
(ii) each tuple $\tup$ encoded by $\rangeTup$ is in a separate group; and
(iii) groups produced from two inputs $\rangeTup$ and $\rangeTup'$ do not overlap.
We can improve this bound by partitioning the input into two sets: tuples with uncertain group-by values and tuples with certain group membership.
When calculating the maximum number of groups for an output $\aout$, the set of input tuples with certain group-by values that fall into the group-by bounds of $\aout$ only contribute the number of distinct \abbrBG group-by values from this set to the bound.
% For the latter we can compute the maximum number of groups for an output $\aout$ by simplying counting the number of groups using \abbrBG values for each input tuple that overlaps with the group-by bounds of $\aout$.
%
For the first set we still apply the worst-case assumption.
To determine the lower bound on the certain annotation of a tuple we have to reason about which input tuples certainly belong to a group. These are inputs whose group-by attributes are certain. For such tuples we sum up their tuple annotation lower bounds.
We then need to derive the annotation of a result tuple from relevant input tuple annotations. \cite{AD11d} extended semirings with a duplicate elimination operator $\duprem_\semN$ for this purpose which is
defined as $\duprem_\semN(k) = 0$ if $k = 0$ and $\duprem_{\semN}(k) = 1$ otherwise.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Aggregation With Group-By]
  \label{def:aggr-op-semantics-gb}
 Let $\query \defas \aggregation{\gbAttrs}{f(A)}(\rangeRel)$ and $\gsdef(\rangeRel,\gbAttrs) = (\gsdefG, \gsdefP)$.
% We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK \lbMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i} \vee \lbMarker{\rangeTup.a_1} \ordK \ubMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i}$. Using these predicates we define set difference as shown below.%
Consider a tuple $\rangeTup$ such that $\exists \asgrp \in \gsdefG$ with $\rangeTup = \aout$. Then,\\[-4mm]
%
\begin{align*}
	\lbMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas  \duprem_{\semN}\left(\sum_{\rangeTup': \gsdefP(\rangeTup') = \asgrp \wedge \neg\, \uncertg{\gbAttrs}{\rangeRel}{\rangeTup'}}\lbMarker{\rangeRel(\rangeTup')}\right) \\
%%%%%%%%%%%%%%%%%%%%
  \bgMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas       \duprem_{\semN}\left(\sum_{\rangeTup': \gsdefP(\rangeTup') = \asgrp} \bgMarker{\rangeRel(\rangeTup')}\right)\\
%%%%%%%%%%%%%%%%%%%%
     \ubMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} &\defas
\sum_{\rangeTup': \gsdefP(\rangeTup') = \asgrp} \ubMarker{\rangeRel(\rangeTup')}
%%%%%%%%%%%%%%%%%%%%
\end{align*}
For any tuple $\rangeTup$ such that $\neg \exists \asgrp \in \gsdefG$ with $\rangeTup = \aout$, we define
\[
  \lbMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} =
  \bgMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)} =
  \ubMarker{\aggregation{\gbAttrs}{f(A)}(\rangeRel)(\rangeTup)}
  = 0
\]
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[t]
  \centering

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subtable}{\linewidth}
  \centering
  \begin{tabular}{ c|c|cc}
    \textbf{street}  & \textbf{number}          & \thead{\#inhab} & \underline{$\uaaK{\semN}$} \\
    \cline{1-3}
      \cMarker{Canal}    & $\uv{165}{165}{165}$     & $\uv{1}{1}{1}$  & (1,1,2)                    \\
%       \cline{1-3}
    \uMarker{Canal}  & $\uv{154}{153}{156}$     & $\uv{1}{2}{2}$  & (1,1,1)                    \\
%       \cline{1-3}
    \cMarker{State}  & $\uv{623}{623}{629}$     & $\uv{2}{2}{2}$  & (2,2,3)                    \\
    \cMarker{Monroe} & $\uv{3574}{3550}{3585}$  & $\uv{2}{3}{4}$  & (0,0,1)                    \\
%       \cline{1-3}
  \end{tabular}\\[-1mm]
  \caption{Input relation address}
        \label{fig:AU-agg-example-input}
  \end{subtable}\\[-1mm]
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{subtable}{\linewidth}
%   \centering
% \begin{lstlisting}
% SELECT sum(#inhab) AS pop FROM address;
% \end{lstlisting}
%   \begin{tabular}{ cc}
% %       \cline{1-2}
%  \textbf{pop}   & \underline{$\uaaK{\semN}$} \\
% \cline{1-1}
%  $\uv{6}{7}{14}$ & (1,1,1)                    \\
% %       \cline{1-2}
%   \end{tabular}
%   \caption{Aggregation without Group-by}
%     \label{fig:AU-agg-example-no-GB}
%   \end{subtable}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subtable}{\linewidth}
  \centering
    \begin{minipage}{0.49\linewidth}
\begin{lstlisting}
SELECT street,
       count(*) AS cnt
FROM address
GROUP BY street;
\end{lstlisting}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
      \centering
  \begin{tabular}{ c|cc}
      % \cline{1-2}
    \textbf{street}  & \textbf{cnt}   & \underline{$\uaaK{\semN}$} \\
    \cline{1-2}
    \uMarker{Canal}  & $\uv{1}{2}{3}$ & (1,1,2)                    \\
    \cMarker{State}  & $\uv{2}{2}{4}$ & (1,1,1)                    \\
    \cMarker{Monroe} & $\uv{1}{1}{2}$ & (0,0,1)                    \\
      % \cline{1-2}
  \end{tabular}
  \end{minipage}\\[-3mm]
    \caption{Aggregation with Group-by}
    \label{fig:AU-agg-example-GB}
  \end{subtable}\\[-3mm]
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Aggregation over \abbrUAADBs}
\label{fig:AU-aggregation}
\trimfigurespacing
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Optimizing Bounds}
% \label{sec:optimizing-bounds}

% The bounds provided by the  general aggregation semantics introduced above can be improved if we take the semantics of the aggregation function into account. In the following we provide better bounds for \aggsum, and \BG{What else?}

% unless the aggregation domain is extended to be symbolic expressions over semiring elements paired with monoid values combined by an abstract addition operation.


% hand demonstrated how to  keep the size of a query result polynomial in the input size of the query by representing the result of aggregation function results as symbolic expressions that pair semiring values with values of the aggregation domain. For instance, without going too much into technical detail, in semiring $\semNX$ the result of a sum aggregation may be $3 \otimes x_1 +_{sum} 2 \otimes x_2$ which intuitively means that the final result of the sum of value $3$ subject to variable $x_1$ and value $2$ subject to variable $x_2$.


% \BG{Is a a more general semantics we can define and then refine for tighter bounds? What about min/max?}

% \BG{Fix notation in the rewrites. Explain notation that is new (attribute names and such)}
% \BG{Define aggregation as an operator, not just aggregation function results}
% %\subsubsection{Row bounds}
% %

% We start with a more general form of the aggregation rule by using polynomial representations. In the real use cases we consider the limitation on the polynomial such that the polynomial can be evaluated into a concrete value.\SF{Do we?} In this case the definition of upper and lower bounds are clear.

% \BG{Not sure whether we need to reiterate this here, but keep it for now:}
% Recall that $\rangeTup[A]$ outputs projection of tuple $\rangeTup$ on a set of attributes $A$.

% \BG{Probably use $f(a)$ instead of $f$ to indicate what attribute we are aggregating over.}

% \BG{We still have to define the aggregation function result for a set of tuples to be able to restrict $\rangeTup$ to tuples that should be in the result instead of just tuples that have the right GB values.}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Aggregation Operator]\label{def:aggr-op-semantics}
% Let $\rangeTup$ and $\rangeTup'$ be range-annotated tuples where $\rangeTup$ has the same arity as $\aggregation{G}{f}(\rangeRel)$ and $\rangeTup'$ has the same arity as $\rangeRel$. Let $G$ be a set of group by attributes and $f$ be the aggregation function.  We define aggregation as shown below.
%    %We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK \lbMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i} \vee \lbMarker{\rangeTup.a_1} \ordK \ubMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i}$. Using these predicates we define set difference as shown below.%
%    \begin{align*}
% 	\lbMarker{\aggregation{G}{f}(\rangeRel)(\rangeTup)} &\defas
% 	\begin{cases}
% 	1_k & \text{if } \exists_{\rangeTup'}:\bgMarker{\rangeTup[G]}=\bgMarker{\rangeTup'[G]} \\
% 		& \text{ and } \forall_{a \in G}:\lbMarker{\rangeTup'.a}=\ubMarker{\rangeTup'.a} \\
% 		& \text{ and } \lbMarker{\combine(\rangeRel)(\rangeTup)} > 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 	\bgMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup)} &\defas \sum_{\bgMarker{\rangeTup[g]} = \bgMarker{\rangeTup'[g]}}\bgMarker{\combine(\rangeRel)(\rangeTup')}
% 	\end{align*}
% 	\begin{align*}
% 	\ubMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup)} &\defas \sum_{\rangeTup[g] \matches \rangeTup'[g]}\ubMarker{\combine(\rangeRel)(\rangeTup')}
% 	\end{align*}
% \end{Definition}

% \begin{Definition}[Aggregation group by attributes]\label{def:aggr-grpby-attr-semantics}
% 	With similar notations, we define aggregation group by attribute bounds as shown below.
% 	\begin{align*}
% 		\forall_{a \in g}:\lbMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup).a} &\defas \minOf{\rangeTup[G] \matches \rangeTup'[G]}\combine(\rangeRel)(\lbMarker{\rangeTup'.a}) \\
% 		\forall_{a \in g}:\ubMarker{\aggregation{g}{f}(\rangeRel)(\rangeTup).a} &\defas \maxOf{\rangeTup[G] \matches \rangeTup'[G]}\combine(\rangeRel)(\ubMarker{\rangeTup'.a})
% 	\end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[General aggregation result attributes]\label{def:aggr-gen-attr-semantics}
% 	Define operator $\{k\}^{+}$ and $\{k\}^{-}$ over value $k$ s.t.
% 	\begin{align*}
% 		\{k\}^{+} =
% 	\begin{cases}
% 	k & \text{if } k \text{ contributes to } \ubMarker{f} \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 		\{k\}^{-} =
% 	\begin{cases}
% 	k & \text{if } k \text{ contributes to } \lbMarker{f} \text{ but not } \ubMarker{f} \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	Use $a_f$ to denote the attribute used by function $f$. We define general aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \lbMarker{f} \defas \\ & \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a_f}\}^+ \oplus \sum_{\rangeTup'[g] \matches \rangeTup[g]} \{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a_f}\}^- \\
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \bgMarker{f} \defas \\ & \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\bgMarker{a_f} \\
% 		& \aggregation{g}{f}(\rangeRel)(\rangeTup). \ubMarker{f} = \\ & \sum_{\rangeTup'[g] \matches \rangeTup[g]}\{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a_f}\}^+ \oplus \sum_{\rangeTup'[g] \equiv \rangeTup[g]} \{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a_f}\}^-
% 	\end{align*}

% \end{Definition}


% \begin{Definition}[Sum aggregation result attributes]\label{def:sum-aggr-attr-semantics}
% 	Define operator $\{k\}^{+}$ and $\{k\}^{-}$ over value $k \in \semK$ s.t.
% 	\begin{align*}
% 		\{k\}^{+} =
% 	\begin{cases}
% 	k & \text{if } k > 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	\begin{align*}
% 		\{k\}^{-} =
% 	\begin{cases}
% 	k & \text{if } k < 0_k \\
% 	0_k & \text{else}
% 	\end{cases}
% 	\end{align*}
% 	We define sum aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \lbMarker{sum(a)} \defas \\ & \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a}\}^+ + \sum_{\rangeTup'[g] \matches \rangeTup[g]} \{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\lbMarker{a}\}^- \\
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \bgMarker{sum(a)} \defas \\ & \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\bgMarker{a} \\
% 		& \aggregation{g}{sum(a)}(\rangeRel)(\rangeTup). \ubMarker{sum(a)} = \\ & \sum_{\rangeTup'[g] \matches \rangeTup[g]}\{\ubMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a}\}^+ +\sum_{\rangeTup'[g] \equiv \rangeTup[g]} \{\lbMarker{\rangeRel(\rangeTup')}*\rangeRel(\rangeTup').\ubMarker{a}\}^-
% 	\end{align*}

% \end{Definition}

% \begin{Definition}[Count aggregation result attributes]\label{def:Count-aggr-attr-semantics}
% 	For count function, all values may contribute to both upper and lower bounds and all attribute values is assigned to $1_k$. The semantics can be simplified. We define count aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \lbMarker{count(a)} \defas \sum_{\rangeTup'[g] \equiv \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \bgMarker{count(a)} \defas \sum_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{count(a)}(\rangeRel)(\rangeTup). \ubMarker{count(a)} \defas \sum_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}

% \end{Definition}

% \begin{Definition}[Min/Max aggregation result attributes]\label{def:MinMax-aggr-attr-semantics}
% 	For min/max function, all values may contribute to both upper and lower bounds, so the semantics can be simplified. We define Min/Max aggregation result attribute bounds as shown below.
% 	\begin{align*}
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \lbMarker{min(a)} \defas \min_{\rangeTup'[g] \matches \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \bgMarker{min(a)} \defas \min_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{min(a)}(\rangeRel)(\rangeTup). \ubMarker{max(a)} \defas \min_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}
% 	\begin{align*}
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \lbMarker{max(a)} \defas \max_{\rangeTup'[g] \matches \rangeTup[g]}\lbMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \bgMarker{max(a)} \defas \max_{\bgMarker{\rangeTup'[g]} = \bgMarker{\rangeTup[g]}}\bgMarker{\rangeRel(\rangeTup')} \\
% 		& \aggregation{g}{max(a)}(\rangeRel)(\rangeTup). \ubMarker{max(a)} \defas \max_{\rangeTup'[g] \matches \rangeTup[g]}\ubMarker{\rangeRel(\rangeTup')}
% 	\end{align*}
% \end{Definition}



% %\begin{enumerate}
% %%\item selection
% %%\[\lbMarker{[\selection_\theta(R)](t)}=\lbMarker{R(t)} \otimes \lbMarker{(\theta(t))} \]
% %%\[\ubMarker{[\selection_\theta(R)](t)}=\ubMarker{R(t)} \otimes \ubMarker{(\theta(t))} \]
% %%
% %%\item join
% %%\[ \lbMarker{[R_1 \join R_2](t)} = \lbMarker{R_1(t)} \otimes \lbMarker{R_2(t)} \]
% %%\[ \ubMarker{[R_1 \join R_2](t)} = \ubMarker{R_1(t)} \otimes \ubMarker{R_2(t)} \]
% %%
% %%\item Union
% %%\[ \lbMarker{[R_1 \union R_2](t)} =
% %%	\lbMarker{R_1(t)} \oplus  \lbMarker{R_2(t)}\]
% %%\[ \ubMarker{[R_1 \union R_2](t)} = \ubMarker{R_1(t)} \oplus \ubMarker{R_2(t)} \]
% %%
% %%\item Projection
% %%\[ \lbMarker{[\projection_{U}(R)](t)} = \sum_{t=t'[U]}\lbMarker{R(t')} \]
% %%\[ \ubMarker{[\projection_{U}(R)](t)} = \sum_{t=t'[U]}\ubMarker{R(t')} \]
% %%
% %%\item Set difference
% %%\[ \lbMarker{[R_1 - R_2](t)} = \lbMarker{R_1(t)} \ominus \sum_{R_1(t) \matches R_2(t')} \ubMarker{R_2(t')} \]
% %%\[ \ubMarker{[R_1 - R_2](t)} = \ubMarker{R_1(t)} \ominus \sum_{R_1(t) \equiv R_2(t')} \lbMarker{R_2(t')} \]
% %
% %%\subsubsection{Attribute bound}
% %%\begin{enumerate}
% %
% %%\item Union
% %%\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\lbMarker{a_i} = \min(R_1(t).\lbMarker{a_i},R_2(t).\lbMarker{a_i}) \]
% %%\[ \forall_{a_i \in U } : [R_1 \union R_2](t).\ubMarker{a_i} = \max(R_1(t).\ubMarker{a_i},R_2(t).\ubMarker{a_i}) \]
% %%
% %%\item Projection
% %%\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]
% %%\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\ubMarker{a_i} = \max_{t=t'[U]} R(t').\ubMarker{a_i} \]
% %
% %
% %
% %\item Count Aggregation without group by
% %\[ [ \aggregation{}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{t' \in R}\lbMarker{R(t')} \]
% %\[ [ \aggregation{}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{t' \in R}\ubMarker{R(t')} \]
% %
% %\item Count Aggregation with group by
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)](t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]
% %
% %\[ [ \aggregation{g}{count(A)}(R) ](t).\lbMarker{count(A)} = \sum_{R(t')[g] \equiv t[g]}\lbMarker{R(t')} \]
% %\[ [ \aggregation{g}{count(A)}(R) ](t).\ubMarker{count(A)} = \sum_{R(t')[g] \matches t[g]}\ubMarker{R(t')} \]
% %
% %
% %\item Sum Aggregation without group by
% %\begin{align*}
% %[ & \aggregation{}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{t' \in R}\{\lbMarker{R(t')}*R(t').\lbMarker{A}\}^+ + \{\ubMarker{R(t')}*R(t').\lbMarker{A}\}^-
% %\end{align*}
% %\begin{align*}
% %[ & \aggregation{}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{t' \in R}\{\ubMarker{R(t')}*R(t').\ubMarker{A}\}^+ + \{\lbMarker{R(t')}*R(t').\ubMarker{A}\}^-
% %\end{align*}
% %
% %\item Sum Aggregation with group by
% %\[ [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{sum(A)} = \sum_{t' \in R, t[g] \in t'[g]}LB(R(t'))*R(t').\lbMarker{A} \]
% %\[ \forall_{a_i \in U } : [\projection_{U}(R)](t).\lbMarker{a_i} = \min_{t=t'[U]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\lbMarker{a_i} = \min_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\lbMarker{a_i} \]
% %\[ \forall_{a_i \in g } : [ \aggregation{g}{sum(A)}(R) ](t).\ubMarker{a_i} = \max_{[\projection_{g}(R)(t[g]) \matches R(t')[g]} R(t').\ubMarker{a_i} \]
% %\begin{align*}
% %[ & \aggregation{g}{sum(A)}(R) ](t). \lbMarker{sum(A)} = \\ & \sum_{R(t')[g] \equiv t[g]}\{\lbMarker{R(t')}*R(t').\lbMarker{A}\}^+ + \\ & \sum_{R(t')[g] \matches t[g]} \{\ubMarker{R(t')}*R(t').\lbMarker{A}\}^-
% %\end{align*}
% %\begin{align*}
% %[ & \aggregation{g}{sum(A)}(R) ](t). \ubMarker{sum(A)} = \\ & \sum_{R(t')[g] \matches t[g]}\{\ubMarker{R(t')}*R(t').\ubMarker{A}\}^+ + \\ & \sum_{R(t')[g] \equiv t[g]} \{\lbMarker{R(t')}*R(t').\ubMarker{A}\}^-
% %\end{align*}
% %
% %\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Examples}

The following example illustrates the application of the aggregation semantics we have defined in this section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{ex:aggregation}
  Consider the relation shown in \Cref{fig:AU-aggregation} which records addresses (street, street number, number of inhabitants).
  Following~\cite{Yang:2015:LOA:2824032.2824055}, uncertain text fields are marked in red to indicate that their bound encompasses the whole domain.
  Street values $v$ in black are certain, i.e.,  $\lbMarker{v} = \bgMarker{v} = \ubMarker{v}$.
  We are uncertain about particular street numbers, number of inhabitants at certain addresses, and one street name. Furthermore, several tuples may represent more than one address. % Finally, we are uncertain about the street for the address represented by the second tuple.
  % Consider the aggregation query without group-by shown in \Cref{fig:AU-agg-example-no-GB}. We are calculating the number of inhabitants. In the \abbrBGW there are 7 inhabitants ($1 \cdot 1 + 2 \cdot 1 + 2 \cdot 2$).
  % As another example
  For the query shown in \Cref{fig:AU-agg-example-GB}
 consider the second result tuple (group \textit{State}). This tuple certainly exists since the 3rd tuple in the input appears twice in every world and its group-by value is certain. Thus, the count for group \textit{State} is at least two. The second input tuple could also belong to this group and, thus, the count could be $4$ (the upper bound).
 Note also the multiplicity of the first output tuple (group \textit{Canal}): \uv{1}{1}{2}.
 In the \abbrBGW the first two input tuples belong to this group.
 However, the second input tuple need not be in this group in all worlds, and in fact may not belong to any existing group.
 Thus, in some possible worlds this one \abbrAUDB tuple may represent 2 distinct output tuples.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Preservation of bounds}\label{sec:preserve-bounds-agg}

We are ready to state the main result of this section: our aggregation semantics for \abbrUAADBs is bound-preserving.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}\label{theo:aggregation-preserves-bounds}
  Let $\query \defas \aggregation{\gbAttrs}{f(A)}(\rel)$ or $\query \defas \aggregation{}{f(A)}(\rel)$.
$\uaaN$-relational query semantics preserves bounds for $\query$.
  % and $\prel$ be an incomplete $\semK$-relation that is bound by an $\uaaK{\semK}$-relation $\rangeRel$. Then $\query(\rangeRel)$ bounds $\query(\prel)$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  The claim is proven by demonstrating that for every possible world $\rel$ of the input incomplete $\semN$-relation $\prel$ and a tuple matching $\TM$ based on which $\rangeRel$ bounds $\rel$, we can construct a tuple matching based on which $\query(\rangeRel)$ bounds $\query(\rel)$. For each aggregation result $\tup$ in $\rel$, we show that there is a result in $\query(\rangeRel)$ that bounds the values of $\tup$, because our aggregation semantics computes aggregation function results based on the minimum and maximum contribution of each possible input tuple, and group-by attribute bounds are generated by conservatively merging the group-by bounds of input tuples.
 See~\cite{techreport} for the full proof.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our main technical result follows from \Cref{theo:aggregation-preserves-bounds}\iftechreport{, \Cref{theo:set-difference-prese},}\ifnottechreport{,~\cite[Thm. 3]{techreport} (bound preservation for set difference)} and \Cref{lem:ra-plus-preserves-bounds} : Our query semantics for $\raAgg$ queries preserves bounds.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Corollary} %[Preservation of bounds for $\raAgg$]
  \label{cor:preservation-of-boun}
$\uaaN$-semantics preserves bounds for $\raAgg$.
  % Let $\query$ be an $\raAgg$ query and $\pdb$ an incomplete $\semN$-database that is bound by an $\uaaK{\semN}$-database $\rangeDB$. Then $\query(\rangeDB)$ bounds $\query(\pdb)$.
%  $$ \pdb \dbbounds \rangeDB \Rightarrow \query(\pdb) \dbbounds \query(\rangeDB)$$
\end{Corollary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}

% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-correctness.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Expression Evaluation over $\mathcal{U}^+$ is c-sound]
\label{theo:expr-c-sound}
  Let $\pdb$ be a probabilistic database and $\db$ be a c-sound UAA-database wrt. $\pdb$, then for any tuple $t \in \db$, and some expression $e$. If $det([[ e(t) ]]) = T$, then in every possible world $D_i \in \pdb$ there has to exist a tuple $t'$ with $t \tmatches t'$ such that $[[e(t')]] = val([[e(t)]])$. % evaluates to the same result in every possible world.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
	We prove this theorem using induction over the structure of an expression under the assumption that the input to the expression is c-sound.

	\proofpara{Base case}
	When the expression is only a single attribute value $e=t.A$, output is c-sound following from the c-soundness assumption that we made for the input.

	\proofpara{Induction step} \\
	For expression operator $op(arg_1,arg_2,\ldots, arg_n)$, \\assume $arg_1(t),arg_2(t),\ldots, arg_n(t)$ is c-sound.
	\begin{itemize}
		\item CASE 1: For $op=\{+,-,=,>,<,||\}$ operations $op(l,r)$, the result is certain only if both of the input is certain $det(l(t))=det(r(t))=T$. Given $l(t)$ and $r(t)$ are c-sound which means $l(t)$ and $r(t)$ return same value for all $D_i \in \pdb$ where exist $t' \in D_i$ st. $t \tmatches t'$. So $op(l,r)(t)$ also returns same value for all $D_i \in \pdb$ where $t$ matching exists. So these operations are c-sound.
		\item CASE 2: For $op=\{*\}$ operation $op(l,r)$, the result is certain only if both of the input is certain or one of the values is $0^T$, $det(l(t))=det(r(t))=T \vee l(t)=0^T \vee r(t)=0^T$. Case $det(l(t))=det(r(t))=T$ is same as CASE 1 so under this case the operator is c-sound. For case $l(t)=0^T \vee r(t)=0^T$, we know either $r(t)$ or $l(t)$ is $0$ for all $D_i \in \pdb$ where exist $t' \in D_i$ st. $t \tmatches t'$. So $l*r=0$ for all $D_i \in \pdb$ where matching $t$ exists. So case $l(t)=0^T \vee r(t)=0^T$ is c-sound and overall the operator is c-sound.
		\item CASE 3: For $op={\wedge}$ operation $op(l,r)$, the result is certain iff both the input is certain or one of the values is $F^T$, $det(l(t))=det(r(t))=T \vee l(t)=F^T \vee r(t)=F^T$. Similar to CASE 2 where in this case we have $l \wedge F=F \wedge r=F$ for all $D_i \in \pdb$ where matching $t$ exists. So the operator is c-sound.
		\item CASE 4: For $op=\{\vee\}$ operation $op(l,r)$, the result is certain iff both the input is certain or one of the values is $T^T$, $det(l(t))=det(r(t))=T \vee l(t)=T^T \vee r(t)=T^T$. Similar to CASE 2 where in this case we have $l \vee T=T \vee r=T$ for all $D_i \in \pdb$ where matching $t$ exists. So the operator is c-sound.
		\item CASE 5: For $op=\{if\}$ operation $op(arg_{if},arg_{then},arg_{else})$, the result is certain iff the if condition is certain and corresponding consequence value is certain according to the condition, $ arg_{if}(t)=T^T \wedge det(arg_{then}(t))=T \vee (\neg arg_{if})(t)=T^T \wedge det(arg_{else}(t))=T$. For the case $arg_{if}(t)=T^T \wedge det(arg_{then}(t))=T$, by assumption we know $arg_{then}(t)$ is c-sound which means $arg_{then}(t)$ returns same value for all $D_i \in \pdb$ where there exists $t' \in D_i$ st. $t \tmatches t'$. So $arg_{then}(t)$ itself as the output is c-sound. The same logic applies to case of $arg_{else}(t)$. Thus the operator is c-sound.
	\end{itemize}
	So by induction, we conclude that our expression evaluation model is c-sound by the fact that any expression is recursively starting with the base case which is c-sound, and given the input is c-sound, the results of all the operators are c-sound .
\end{proof}

Based on this result, we now proceed to prove that query evaluation preserves c-soundness, i.e., if the input to a query is c-sound wrt. a probabilistic database $\pdb$ then so is the output wrt. evaluating the query over $\pdb$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Query Evaluation Preserves c-Soundness in UAA-relation]\label{theo:UAA-are-c-sound}
  Let $\pdb$ be a probabilistic database and $\db$ be a UAA-database corresponding to $\pdb$ that is c-sound. Given a query $\query$, the result $\query(\db)$ is c-sound wrt. $\query(\pdb)$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  We prove this theorem using induction over the structure of a query under the assumption that the input to the query is c-sound.

  \proofpara{Base case}
  When the query $\query$ is of the form $\query=R$, i.e., it consists of a single relation access, then c-soundness of the output follows from the c-soundness assumption that we have made for the input.

\proofpara{Induction step} Assume that the query is of the form $op(\query_1)$ for some operator $op$ and assume that the result $\query_1$ is c-sound.
	\begin{itemize}
		\item For union operation $Q_1 \cup Q_2$, the result tuple $t$ with annotation $(u,c)$ is produced by adding annotation $(u_1,c_1)$ of $t' \in Q_1$ and annotation $(u_2,c_2)$ of $t' \in Q_2$ where $t'\tmatches t$ so that $c=c_1+c_2$. By assumption we know $Q_1(t')$ and $Q_2(t')$ is c-sound which means $c_1 \leqslant c_1^*$ and $c_2 \leqslant c_2^*$. By propagation rule we have $c=c_1+c_2 \leqslant c_1^*+c_2^*=c^*$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
		\item For join operation $Q_1 \times Q_2$, the result tuple $t$ with annotation $(u,c)$ is produced by multiplying annotation $(u_1,c_1)$ of $t_1 \tmatches t[SCHEMA(Q_1)] \in Q_1$ and annotation $(u_2,c_2)$ of $t_2 \tmatches t[SCHEMA(Q_1)] \in Q_2$ so that $c=c_1 \times c_2$. By assumption we know $t_1$ and $t_2$ are c-sound which means $c_1 \leqslant c_1^*$ and $c_2 \leqslant c_2^*$. By propagation rule we have $c=c_1 \times c_2 \leqslant c_1^* \times c_2^*=c^*$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
		\item For projection operation $\projection_{U}(Q)$, the result tuple $t$ with annotation $(u,c)$ is produced by adding all tuples $t_i$ with annotation $(u_i,c_i)$ respectively where $t_i \in Q \wedge t_i[U] \tmatches t$. By assumption we know all $t_i$s are c-sound which means $\forall_{i}(c_i \leqslant c_i^*)$. By propagation rule we have $c=\sum_{i}(c_i) \leqslant \sum_{i}(c_i^*)=c^*$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
		\item For selection operation $\selection_{\theta}(Q)$, the result tuple $t$ with annotation $(u,c)$ has $c>0$ iff $t \models \theta$. By assumption we know $Q(t')$ where $t' \tmatches t$ with annotation $(u_o,c_o)$ is c-sound which means $c_o \leqslant c_o^*$. By propagation rule we have $c=c_o \leqslant c_o^*=c^* \vee c=0$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
	\end{itemize}
	So by induction, we conclude that our query rewriting rules are c-sound by the fact that any operator recursively starst with the base case which is c-sound, and therefore the results of all operators are c-sound.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-queries.tex <==
%!TEX root=./uaadb.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\abbrUAADB Query Semantics}
\label{sec:uaadb-query-semantics}

We now introduce a semantics for $\raPlus$ queries over \abbrUAADBs that preserves bounds, i.e., if the input of a query $\query$ bounds an incomplete $\semN$-database $\pdb$, then the output bounds $\query(\pdb)$. 
\reva{
\abbrUAADBs follow the standard K-relational semantics for all $\raPlus$ operations except selection.
  The revised selection operator (described below) remains linear in the size of its input,} \revb{thus implying \ptime query evaluation.} %Conveniently, it turns out that the standard query semantics for $\semN$-relations with a slight extension to deal with uncertain boolean values in conditions is sufficient.  % for this purpose.
 Recall the standard semantics for evaluating selection conditions over $\semN$-relations: The multiplicity of a tuple $t$  in the result of a selection $\selection_{\theta}(R)$ is computed by multiplying $\rel(\tup)$ with $\theta(\tup)$. $\theta(\tup)$ is defined a function $\semB \to \{ 0,1 \}$ that returns $1$ if $\theta$ evaluates to true on $\tup$ and $0$ otherwise.
% In the special case of $\semN$ the $\theta(t)$ returns $1$ is the condition is true and $0$ otherwise.
In $\uaaK{\semN}$-relations, $\tup$ is a tuple of range-annotated values.
% It turns out that \abbrUAADB relations follows the standard k-relational querying semantics by treating range annotations as a vector of semiring values $(\lbMarker{k},k,\ubMarker{k})$.
Using the range-annotated semantics for expressions from \Cref{sec:expression}, selection conditions evaluate to triples of boolean values $\semB^3$.
For example, $\uv{F}{F}{T}$ means that the condition may be false in some worlds, is false in the \abbrBGW, and may be true in some worlds.
To define selection semantics compatible with $\semN$-relational query semantics, these triples must be translated to elements of $\uaaK{\semN}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Boolean to Semiring Mapping]
  \label{def:lift-bool-to-K}
  % Let $\semK$ be a semiring.
  We define function $\rliftK{\semN}:\semB^3 \rightarrow \semN^3$ as:\\[-5mm]
  \begin{align*}
    \rliftK{\semN}(\uv{b_1}{b_2}{b_3}) &\defas \ut{k_1}{k_2}{k_3} \,\,\,\text{where}\,\,\,
    % \forall i \in \{1,2,3\}:
                                       k_i \defas
    \begin{cases} 1 & \text{if }\; b_i = true\\
      0 & \text{otherwise}
    \end{cases}
    \end{align*}
% 	\[ \rliftK{\semK}(b_1,b_2,b_3) = (k_1,k_2,k_3) \text{ s.t. } \\
% 	\forall i \in \{1,2,3\}: k_i = \begin{cases} 1_k & \text{if } b_i = true      \\
% 0_k                                                & \text{otherwise}
% \end{cases} \]
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We use the mapping of range-annotated boolean values to $\uaaK{\semN}$ elements to define evaluation of selection conditions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Conditions over Range-annotated Tuples]
  \label{def:range-selection}
  Let % $\semK$ be a semiring,
  $\rangeTup$ be a range-annotated tuple, and $\theta$ be a boolean condition over variables representing attributes from $\rangeTup$. Furthermore, let $\rval_{\rangeTup}$ denote the range-annotated valuation that maps each variable to the corresponding value from $\rangeTup$. We define $\theta(\rangeTup)$ as: % the result of the condition $\theta$ applied to $\rangeTup$ in  $\semN$ as:
  \begin{align*}
    \theta(\rangeTup) \defas \rliftK{\semN}(\seval{\theta}{\rval_{\rangeTup}})
  \end{align*}
  % For selection operation $\selection_\theta(R)$ following standard semiring querying sematics:
  %   \[ [\selection_\theta(R)](t)=R(t) \otimes \theta(t) \]
  %   Define $(\theta(t))$ is a triple $k^I$ s.t.
  %   \[ \theta(t)=\rliftK{\semK}(\seval{\theta(t)}{\rval}) \]
  \end{Definition}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{Example}\label{ex:selections}
    Consider the example $\uaaK{\semN}$-relation $\rel$ shown below. The single tuple $\rangeTup$ of this relation binds at least one tuple in every possible world, two in the \abbrBGW, and no more than three in any world.

    \begin{center}
      {\upshape
    \begin{tabular}{c|cc}
      \thead{A}    & \thead{B} & \underline{$\uaaK{\semN}$} \\ \cline{1-2}
      \uv{1}{2}{3} & $2$         & $\ut{1}{2}{3}$
    \end{tabular}
    }
  \end{center}

    To evaluate query $\query \defas \selection_{A = 2}(\rel)$ over this relation, we first evaluate the expression $A = 2$ using range-annotated expression evaluation semantics. We get $\uv{1}{2}{3} = \uv{2}{2}{2}$ which evaluates to $\uv{F}{T}{T}$. Using $\rliftK{\semN}$, this value is mapped to $\ut{0}{1}{1}$. To calculate the annotation of the tuple in the result of the selection we then multiply these values with the tuple's annotation in $\rel$ and get:
    $$\rel(\rangeTup) \multOf{\uaaK{\semN}} \theta(\rangeTup) = \ut{1}{2}{3} \cdot \ut{0}{1}{1} = \ut{0}{2}{3}$$
    Thus, the tuple may not exist in every possible world of the query result, appears twice in the \abbrBGW query result, and occurs at most three times in any possible world.
  \end{Example}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Preservation of Bounds}

  For this query semantics to be useful, it has to preserve bounds. Formally, a query semantics is \textit{bound preserving} for a class of queries $\qClass$ if for every query $\query \in \qClass$, incomplete $\semN$-database $\pdb$ and $\uaaK{\semN}$-database $\rangeDB$ that bounds $\pdb$ ($\pdb \dbbounds \rangeDB$), we have $\query(\pdb) \dbbounds \query(\rangeDB)$.
% The annotations propagate through standard querying semantics by mapping the expression outputs to a triple of semiring values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{Theorem}% [\raPlus Queries Preserve Bounds]
    \label{lem:ra-plus-preserves-bounds}
$\uaaK{\semN}$-relational  semantics preserves bounds  for $\raPlus$.
  % Let $\pdb$ be an incomplete $\semK$-database, $\query$ be a $\raPlus$ query, and $\rangeDB$ be an $\uaaK{\semK}$-database that bounds $\db$. Then $\query(\rangeDB)$ bounds $\query(\pdb)$.
  % Under $\raPlus$, given $R$ is lower bounded by $R^I$ w.r.t. $TM_{R,R^I}$, there exist $TM'_{Q(R),Q(R^I)}$ s.t. $Q(R)$ is lower bounded by $Q(R^I)$.
\end{Theorem} %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{proof}[Proof Sketch]
  Intuitively, this is true because expressions are evaluated using  range-annotated expression semantics, which preserves bounds on values, and queries are evaluated in a direct-product semiring $\uaaK{\semN}$ whose operations are defined point-wise.
  Concretely, we use \cite[Lemma 2]{FH19}: addition and multiplication preserve order in $\semN$ (e.g., if $k_1 \leq k_2$ and $k_3 \leq k_4$ then $k_1 + k_3 \leq k_2 + k_4$), and induction over the structure of  a query under the assumption that $\rangeDB$ bounds $\pdb$ to prove the theorem. (full proof in \cite{techreport})
\end{proof}
% \BG{mention set difference is in the tech report}
% OK: ^---- this is implicit in the fact that the tech report covers other semantics as well.
%\begin{Lemma}
%\ubMarker{k} is subadditive and submultiplicative
%\begin{proof}
%Recall that $\pwAdd$ and $\pwMult$ are defined element-wise and that $\pwPossible(\pwe{k}) = \LubK(\pwe{k})$. Furthermore, $k_1 \ordK k_2$ iff $\exists k': k_1 \addK k' = k_2$. Consider an arbitrary $\pwe{k_1}, \pwe{k_2} \in \pwkDom$.  Let $k_{lub_1} = \LubK(\pwe{k_1})$ and $k_{lub_2} = \LubK(\pwe{k_2})$. Based on the definition of $\LubK$ this implies that for any $i$, $k_{lub_1} \geqK \pwe{k_1}[i]$ which in turn implies that $\pwe{k_1}[i] \addK k' = k_{glb_1}$ for some $k'$. Analog, we can find a $k''$ such that $\pwe{k_2}[i] \addK k'' = k_{glb_2}$.
%
%  \proofpara{Subadditivity}
%Let $k_{lub} = \LubK(\pwe{k_1} \pwAdd \pwe{k_2})$. We are going to prove that $k_{lub_1} \addK k_{lub_2}$ is an upper bound for $(\pwe{k_1} \pwAdd \pwe{k_2})$, i.e., that $\forall i \in \pwDom: k_{lub_1} \addK k_{lub_2} \geqK (\pwe{k_1} \pwAdd \pwe{k_2})[i]$. Since, $k_{lub}$ is the least upper bound this implies that $k_{lub_1} \addK k_{lub_2} \geqK k_{lub}$. Consider an arbitrary $i \in \pwDom$. Based on the discussion above we have:
%
%\noindent\resizebox{1\linewidth}{!}{
%  \begin{minipage}{1.05\linewidth}
%\begin{align*}
%&k_{lub_1} \addK k_{lub_2} = (\pwe{k_1}[i] \addK k') \addK (\pwe{k_2}[i] \addK k'')  \\
%&= (\pwe{k_1} \pwAdd \pwe{k_2})[i] \addK k' \addK k'' \geqK (\pwe{k_1} \pwAdd \pwe{k_2})[i]
%\end{align*}
%\end{minipage}
%}
%
%Thus, $k_{lub_1} \addK k_{lub_2}$ is an upper bound and since $k_{lub_1} = \pwPossible(\pwe{k_1})$ and $k_{lub_2} = \pwPossible(\pwe{k_2})$  it follows that $\pwPossible$ is subadditive:
%\begin{align*}
%\pwCertain(\pwe{k_1}) \addK \pwCertain(\pwe{k_2}) \ordK \pwCertain(\pwe{k_1} \pwAdd \pwe{k_2})
%\end{align*}
%
%\proofpara{Submultiplicativity}
%We use an analogous argument to prove submultiplicativity. Let $k_{lub} = \pwPossible(\pwe{k_1} \multK \pwe{k_2})$. We will prove that $k_{lub_1} \multK k_{lub_2}$ is an upper bound for $(\pwe{k_1} \pwMult \pwe{k_2})$ which implies submultiplicativity. Consider $i \in \pwDom$:
%
%\noindent\resizebox{1\linewidth}{!}{
%  \begin{minipage}{1.15\linewidth}
%\begin{align*}
%&(k_{lub_1} \multK k_{lub_2})
%= (\pwe{k_1}[i] \addK k') \multK (\pwe{k_2}[i] \addK k'')\\
%= &(\pwe{k_1}[i] \multK \pwe{k_2}[i]) \addK (\pwe{k_1}[i] \multK k'') \addK (k' \multK \pwe{k_2}[i])  \addK (k' \multK k'')\\
%\geqK &(\pwe{k_1} \pwMult \pwe{k_2})[i] \qedhere
%\end{align*}
%\end{minipage}
%}
%\end{proof}
%\end{Lemma}

%\begin{enumerate}
%\item Addition
%\[ (\lbMarker{k_1},k_1,\ubMarker{k_1}) \oplus (\lbMarker{k_2},k_2,\ubMarker{k_2}) = (\lbMarker{k_1} \oplus \lbMarker{k_2}, k_1 \oplus k_2, \ubMarker{k_1} \oplus \ubMarker{k_2})\]
%\item Multiplication
%\[ (\lbMarker{k_1},k_1,\ubMarker{k_1}) \otimes (\lbMarker{k_2},k_2,\ubMarker{k_2}) = (\lbMarker{k_1} \otimes \lbMarker{k_2}, k_1 \otimes k_2, \ubMarker{k_1} \otimes \ubMarker{k_2})\]
%\end{enumerate}

\ifnottechreport{
\subsection{\reva{Join Optimizations}}
\label{sec:joinOpt}
% \subsection{Optimizations for Joins}
One potential performance bottleneck of query evaluation over \abbrUAADBs is that equi-joins may degenerate into cross products if the bounds of join attribute values are loose. For example, this happens when the join attribute bounds of every tuple from the LHS overlaps with the join attribute bounds of every tuple from the RHS.
We now develop an optimization for joins that splits each input relation $\rangeRel$ of the join into two parts: $\splitbg(\rangeRel)$ and $\splitpos(\rangeRel)$ as follows. If the equijoin is on attributes $\tuple{a_1, \ldots, a_n}$:
\begin{eqnarray*}
  \lbatt{\splitbg(\rangeRel)(\rangeTup)} &\defas&
    \begin{cases}
      \lbatt{\rangeRel(\rangeTup)} & \textbf{if } \forall i : \lbatt{\rangeTup.a_i} = \bgatt{\rangeTup.a_i} = \ubatt{\rangeTup.a_i} \\
      0 & \textbf{otherwise}
    \end{cases}
\\
  \bgatt{\splitbg(\rangeRel)(\rangeTup)} &\defas& \ubatt{\splitbg(\rangeRel)(\rangeTup)} \;\defas\; \bgatt{\rangeRel(\rangeTup)}
\\
\lbatt{\splitpos(\rangeRel)(\rangeTup)}  &\defas&  \bgatt{\splitpos(\rangeRel)(\rangeTup)}  \;\defas\; 0
\\
  \ubatt{\splitpos(\rangeRel)(\rangeTup)} &\defas& \ubatt{\rangeRel(\rangeTup)}
\end{eqnarray*}
This operation ensures (i) that any relation $\rel$ bound by $\rangeRel$ is also bound by both $\splitpos(\rangeRel)$ and $\splitbg(\rangeRel) \cup \splitpos(\rangeRel)$, (ii) that the join attributes of $\splitbg(\rangeRel)$ are all certain, and (iii) that $\bgatt{\splitbg(\rangeRel)} = \bgatt{\rangeRel}$.
Properties (i) and (iii) allow us to compute a bounding \abbrUAARel for the join $\rangeRel_1 \bowtie \rangeRel_2$ as\\[-3mm]
%
\[
      (\splitbg(\rangeRel_1) \bowtie \splitbg(\rangeRel_2) )
 \cup (\splitpos(\rangeRel_1) \bowtie \splitpos(\rangeRel_2))
\]
% \[
%       \left(\splitbg(\rangeRel_1) \bowtie \splitbg(\rangeRel_2) \right)
%  \cup \left(\splitpos(\rangeRel_1) \bowtie \splitpos(\rangeRel_2)\right)
% \]
Thanks to property (ii), the first join is a classical relational join and can be evaluated efficiently.
\revc{The latter join remains expensive, but tuples in this join can be compressed:
Based on a join compression size $\CT$ and join attribute $A$, we construct $\CT$ buckets $[\lbatt{b_i}, \ubatt{b_i}]$ over the domain of $A$ such that (i) for every tuple in $\rangeTup \in \splitpos(\rangeRel_i)$, there exists an $i$ such that $\lbatt{b_i} \leq \lbatt{\rangeTup.A} \leq \ubatt{\rangeTup.A} \leq \ubatt{b_i}$, and (ii) the number of tuples contained in this way by each bucket is roughly uniform.
The compressed $\splitpos(\rangeRel_i)$ relation has exactly $\CT$ tuples (one for each bucket) with attribute bounds that cover all tuples assigned to the bucket, lower and selected-guess multiplicities of 0, and an upper-bound multiplicity of the number of tuples assigned to the bucket.
For example, \Cref{fig:joinOptimization} shows the overlapping ranges of the join attributes of seven tuples ($a-g$).
To create a compressed representation of size 3 (i.e., $\CT = 3$), these tuples are partitioned into 3 roughly-equally-sized bins ($B_1$, $B_2$, $B_3$), and the resulting attribute bounds are selected as the maximum upper and lower bounds of the component tuples.
}
The compression size allows a trade-off between faster query evaluation and tighter % \emph{upper}
bounds.
We prove that the resulting join operation is correct in~\cite{techreport}.


\begin{figure}
\includegraphics[width=0.9\columnwidth]{figs/join_optimization.pdf}
\caption{\revc{An example of join compression with a compression size of 3: Tuples $a-g$ are compressed into bins $B_1 - B_3$.}}
\label{fig:joinOptimization}
\trimfigurespacing
\end{figure}
}% end \ifnottechreport

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-range.tex <==
\section{Scalar Expressions}
\label{sec:expression}

\BG{Only define $\leq$ and $=$ since $<$, $>$ and $\geq$ can then be defined using logical operators and these two}

We now introduce a semantics for evaluating scalar expressions over a set of variables whose values are uncertain. For that we first define expression syntax and semantics, then generalize to incomplete expressions, and finally introduce range-annotated values as a way to under- and over-approximate incomplete expressions. The techniques established in this section are then used to define \abbrUAADBs as relations whose values are range-annotated in \Cref{sec:uaa-range}.
We assuming independent variables and use $\dataDomain$ to denote the domain assuming boolean values are included in the domain. Furthermore, let $\mathbb{V}$ denote a countable set of variables.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Expression Syntax]\label{def:expr-syntax}
	For any variable $x \in \mathbb{V}$, $x$ is an expression and for any constant $c \in \dataDomain$, $c$ is an expression.
	If $\sexpr_1$, $\sexpr_2$ and $\sexpr_3$ are expressions, then \ldots
    \begin{align*}
      &\sexpr_1 \wedge \sexpr_2
      &&\sexpr_1 \vee \sexpr_2
      && \neg \sexpr_1
      &&\sexpr_1 = \sexpr_2
      &&\sexpr_1 \neq \sexpr_2
      &&\sexpr_1 \leq \sexpr_2
    \end{align*}
    \begin{align*}
      &&\sexpr_1 + \sexpr_2
      &&\sexpr_1 \cdot \sexpr_2
      &&\ifte{\sexpr_1}{\sexpr_2}{\sexpr_3}\\
    \end{align*}
\BG{what else do we need?}
	are also expressions. Given an expression $\sexpr$, we denote the variables in $\sexpr$ by $\vars(\sexpr)$. % $\vars(\sexpr)$ is defined recursively:
    % \begin{align*}
    %   \vars(x) &= \{x\} \\
    %   \vars(\sexpr_1 \wedge \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\sexpr_1 \vee \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\sexpr_1 = \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\sexpr_1 \neq \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\sexpr_1 > \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\sexpr_1 < \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\ifte{\sexpr_1}{\sexpr_2}{\sexpr_3}) &= \vars(\sexpr_1) \cup \vars(\sexpr_2) \cup \vars(\sexpr_3)\\
    %   \vars(\sexpr_1 + \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\sexpr_1 - \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    %   \vars(\sexpr_1 \times \sexpr_2) &= \vars(\sexpr_1) \cup \vars(\sexpr_2)\\
    % \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the following we will also use $\neq$, $\geq$, $<$, and $>$ since these operators can be defined using the expression syntax above, e.g., $e_1 > e_2 = \neg\, (e_1 \leq e_2)$. Assuming that $\dataDomain$ contains negative numbers, subtraction can be expressed using addition and multiplication.
For an expression $\sexpr$, given a valuation $\sval$ that maps variables from $\vars(\sexpr)$ to constants from $\dataDomain$, the expression evaluates to a constant from $\dataDomain$. The semantics of expression evaluation is defined below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Expression Semantics]\label{def:expr-semantics}
  \BG{Since this semantics is obvious we can remove it if we need space}
	Let $\sexpr$ be an expression. Given a valuation  $\sval: \vars(e) \rightarrow \dataDomain$, the result of expression $\sexpr$ over $\sval$ denoted as $\seval{\sexpr}{\sval}$ is defined as:
    \begin{align*}
      \seval{x}{\sval}                                                                 & \defas \sval(x)
                                                                                       & \seval{c}{\sval}                                    & \defas c &
      \seval{\neg \sexpr_1}{\sval}                                                     & \defas \neg \seval{\sexpr_1}{\sval}
    \end{align*}
    \begin{align*}
     \seval{e_1 \wedge e_2}{\sval}                                                     & \defas \seval{e_1}{\sval} \wedge \seval{e_2}{\sval} &
    \seval{e_1 \vee e_2}{\sval}                                                        & \defas \seval{e_1}{\sval} \vee \seval{e_2}{\sval}                                                       \\
                                                          \seval{e_1 + e_2}{\sval}     & \defas \seval{e_1}{\sval} + \seval{e_2}{\sval}                                                          &
	 % \seval{e_1 - e_2}{\sval}                                                        & \defas \seval{e_1}{\sval} - \seval{e_2}{\sval}
                                                          \seval{e_1 \cdot e_2}{\sval} & \defas \seval{e_1}{\sval} \cdot \seval{e_2}{\sval}  \\
	 \seval{e_1 = e_2}{\sval}                                                          & \defas \seval{e_1}{\sval} = \seval{e_2}{\sval}                                                          &
                                                         %                             & \seval{e_1 > e_2}{\sval}                            & \defas \seval{e_1}{\sval} > \seval{e_2}{\sval}    \\
	 \seval{e_1 \leq e_2}{\sval}                                                       & \defas \seval{e_1}{\sval} \leq \seval{e_2}{\sval}
                                                         %                             & \seval{e_1 \neq e_2}{\sval}                         & \defas \seval{e_1}{\sval} \neq \seval{e_2}{\sval} \\
      \end{align*}
      \begin{align*}
      \seval{\ifte{\sexpr_1}{\sexpr_2}{\sexpr_3}}{\sval}                               & \defas \ifte{\seval{\sexpr_1}{\sval}}{\seval{\sexpr_2}{\sval}}{\seval{\sexpr_3}{\sval}}
    \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Incomplete Expression Evaluation}\label{sec:expr-incomplete}

We now define evaluation of expression where the inputs are uncertain. We model uncertain inputs though incomplete valuations which are sets of valuations. Each valuation in such a set called a possible world represents one possible input for the expression. The semantics of expression evaluation is then defined using the well-known possible worlds semantics: the result of evaluating an expression $\sexpr$ over an incomplete valuation $\uval = \{ \sval_1, \ldots, \sval_n \}$ is the set of results obtained by evaluating $\sexpr$ over each $\sval_i$ using the deterministic expression evaluation semantics defined above.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Incomplete Expression Semantics]\label{def:incomplete-expr-sem}
An incomplete valuation $\uval$ is a set $\{ \sval_1, \ldots, \sval_n \}$ where each $\sval_i$ is a valuation.
The result of evaluating an expression $\sexpr$ over $\uval$ denoted as $\seval{\sexpr}{\uval}$ is:
$$\seval{\sexpr}{\uval} \defas \{ \seval{\sexpr}{\sval} \mid \sval \in \uval \}$$
% An incomplete expression evaluation is a valuation with a set of possible variable to value bindings $vars(e) \rightarrow \{\dataDomain\}$ and evaluates to a set of possible values from the domain $\varphi(e) \rightarrow \{\dataDomain\}$
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The incomplete expression evaluation result can be obtained by performing conventional expression evaluating over each possible variable bindings and union their result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
	Consider an expression $\sexpr \defas x+y$ and an incomplete valuation with possible bindings $\uval = \{ (x=1,y=4), (x=2,y=4), (x=1,y=5) \}$. Applying deterministic evaluation semantics for each of the three valuations from $\uval$ we get  $1+4=5$ ,$2+5=6$, and $1+5=6$. Thus, the possible outcomes of this expression are: $\seval{\sexpr}{\uval} = \{5,6\}$.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Range-Annotated Domains}\label{sec:range-dom}

We now define domain values that are annotated with an interval that bounds the value from above and below.
For categorical domains where no sensible order can be defined, we impose an arbitrary order. Note that in worst-case we can just annotate a value with the range covering the whole domain to indicate that is it uncertain.
% values can only be annotated by either certain or uncertain, we assume a random total order for the categorical domain and annotate uncertain attributes using the lowest and largest value from the domain as the lower and upper bound.
% \BG{@Su: adapt notation as in the previous sections}

We will use such values to compactly bound the inputs and outputs of incomplete expressions.
For that we define an expression semantics for valuations that map variables to such annotated values and then prove that if the input bound an incomplete evaluation, then the output produced by this semantics bounds the possible outcomes of the incomplete expression.
\BG{Following may be possible to omit:}
These results for evaluating expressions under uncertainty will then be utilized afterwards to define relations whose values stem from the annotated domain and which are used to bound the possible worlds of an incomplete database from below and above.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Range annotated domain]\label{def:range-domain}
  Given domain $\dataDomain$ that is totally ordered and let $\leq$ denote its order. Then the range-annotated domain $\rangeDom$ is defined as:

$$\{ (\lbMarker{c}, c, \ubMarker{c}) \mid c, \lbMarker{c}, \ubMarker{c} \in \dataDomain \wedge \lbMarker{c} \leq c \leq \ubMarker{c} \}$$

  % a function $\dataDomain \rightarrow I$ where $I=\dataDomain^2$ denotes the highest and lowest possible value of the element. For an element $x \in \rangeDom$, we use $\ubMarker{x}$ to denote the upper bound and $\lbMarker{x}$ to denote the lower bound of the element.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Intuitively, a value from $\aDomain$ encodes a value $c \in \dataDomain$ and two values ($\lbMarker{c}$ and $\ubMarker{c}$) that bound the value from below and above.
To simplify presentation, we alternatively write a range-annotated element $(c_1, c_2, c_3) \in \rangeDom$ as $\uv{c_1}{c_2}{c_3}$.
Furthermore, given $c = (c_1, c_2, c_3) \in \rangeDom$, we write $\lbMarker{c}$ to denote $c_1$, $\ubMarker{c}$ to denote $c_3$ and $\bgMarker{c}$ to denote $c_2$.
We call a value $c \in \aDomain$  certain if $\lbMarker{c}=\bgMarker{c}=\ubMarker{c}$.
Observe, that the definition requires that for any $(c_1, c_2, c_3) \in \rangeDom$ we have $c_1 \leq c_2 \leq c_3$.
% We also set constrain to the bounds so that the value must be in the bound $\lbMarker{x} \leq x \leq \ubMarker{x}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
	For the Boolean domain $\dataDomain=\{\bfalse,\btrue\}$ with order $\bfalse < \btrue$, the corresponding range annotated domain is $\rangeDom=\{\uv{\btrue}{\btrue}{\btrue},\uv{\bfalse}{\btrue}{\btrue},\uv{\bfalse}{\bfalse}{\btrue},\uv{\bfalse}{\bfalse}{\bfalse}\}$
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now introduce valuations that map the variables of an expression to elements from $\rangeDom$ and use such valuations to encode bounds on the possible values of incomplete valuations.
%Instead of using a set of possible bindings to the variable from the original domain, we bind the uncertain variable to a single value from the interval annotated domain $\rangeDom$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Range-annotated valuation]\label{def:range-val}
Let $\sexpr$ be an expression. A range-annotated valuation $\rval$ for $\sexpr$ is a mapping $\vars(\sexpr) \to \rangeDom$.
  % For an uncertain variable with a set of possible bindings $x=\{v_1,v_2,...,v_n\}$. And a binding to the annotated domain $x=v^I$. We call the binding as a sound bound iff the bound fully covers all possible outcomes of the original bindings $\lbMarker{x} \leq min(\{v_1,v_2,...,v_n\}) \wedge \ubMarker{x} \geq max(\{v_1,v_2,...,v_n\})$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Bounding valuations]\label{def:range-expr-bound}
  Let $\uval$ be an incomplete valuation for an expression $\sexpr$ and $\rval$ be a range-annotated valuation for $\sexpr$.
  We say that $\rval$ bounds $\uval$ iff
  \begin{align*}
    \forall x \in \vars(\sexpr): \forall \sval \in \uval: \lbMarker{\rval(x)} \leq \sval(x) \leq \ubMarker{\rval(x)}\\
    \exists \sval \in \uval: \forall x \in \vars(\sexpr): \sval(x) = \bgMarker{\rval(x)}
  \end{align*}
  % For an uncertain variable with a set of possible bindings $x=\{v_1,v_2,...,v_n\}$. And a binding to the annotated domain $x=v^I$. We call the binding as a sound bound iff the bound fully covers all possible outcomes of the original bindings $\lbMarker{x} \leq min(\{v_1,v_2,...,v_n\}) \wedge \ubMarker{x} \geq max(\{v_1,v_2,...,v_n\})$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
Consider incomplete valuation $\uval = \{(x=1),(x=2),(x=3)\}$. The range-annotated binding  $x=2^{[0,3]}$ is a bound for $\uval$, while $x=2^{[0,2]}$ is not a bound.
  \end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Range-annotated Expression Evaluation}\label{sec:range-expr-eval}

We now define a semantics for evaluating expressions over range-annotated valuations. We then demonstrate that this semantics preserves bounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Range-annotated expression evaluation]\label{def:range-expr-eval}
  Let $\sexpr$ be an expression. Given a valuation $\rval: \vars(e) \rightarrow \rangeDom$,
we define $\bgMarker{\rval}$ as the valuation $\bgMarker{\rval}(x) = \bgMarker{\rval(x)}$.
  The result of expression $\sexpr$ over $\rval$ denoted as $\seval{\sexpr}{\rval}$ is defined as:
    \begin{align*}
      \seval{x}{\rval} &\defas (\lbMarker{\sval(x)},\sval(x),\ubMarker{\sval(x)} ) &
      \seval{c}{\rval} &\defas (c,c,c)\\
    \end{align*}
 For any of the following expressions we define $\bgMarker{\seval{e}{\rval}} \defas \seval{e}{\bgMarker{\rval}}$. Let $\seval{e_1}{\rval} = a$, $\seval{e_2}{\rval} = b$, and $\seval{e_3}{\rval} = c$. Then,
    \begin{align*}
%%%%%%%%%%%%%%%%%%%%
	 \lbMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \lbMarker{a} \wedge \lbMarker{b} &
	 \ubMarker{\seval{e_1 \wedge e_2}{\rval}} &\defas \ubMarker{a} \wedge \ubMarker{b}\\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \lbMarker{a} \vee \lbMarker{b} &
      \ubMarker{\seval{e_1 \vee e_2}{\rval}} &\defas \ubMarker{a} \vee \ubMarker{b} \\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \ubMarker{a} &
      \ubMarker{\seval{\neg e_1}{\rval}} &\defas \neg\, \lbMarker{a} \\
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 + e_2}{\rval}} &\defas \lbMarker{a} + \lbMarker{b} &
      \ubMarker{\seval{e_1 + e_2}{\rval}} &\defas \ubMarker{a} + \ubMarker{b}                                                                                                                   \\
    \end{align*}
    \begin{align*}
%%%%%%%%%%%%%%%%%%%%
      \lbMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                                         &\defas \min(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b})\\
      \ubMarker{\seval{e_1 \cdot e_2}{\rval}}                                                                       &\defas \max(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b}) \\
     %%%%%%%%%%%%%%%%%%%%
    \end{align*}
    \begin{align*}
      \lbMarker{\seval{a \leq b}{\rval}} &\defas \ubMarker{a} \leq \lbMarker{b} &
 \ubMarker{\seval{a \leq b}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\lbMarker{\seval{a=b}{\rval}} &\defas (\ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} ) &
                                                                                                 \ubMarker{\seval{a=b}{\rval}} &\defas \lbMarker{a} \leq \ubMarker{b} \wedge \lbMarker{b} \leq \ubMarker{a}
 % \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
    \end{align*}
    \begin{align*}
\lbMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
\lbMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\lbMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
 \min(\lbMarker{b},\lbMarker{c}) & \text{else}
\end{cases}\\
      \ubMarker{\seval{\ifte{e_1}{e_2}{e_3}}{\rval}} &\defas
 \begin{cases}
 \ubMarker{b} & \text{if } \lbMarker{a}= \ubMarker{a}=\btrue \\
\ubMarker{c} & \text{if } \lbMarker{a}= \ubMarker{a}=\bfalse \\
\max(\ubMarker{b},\ubMarker{c}) & \text{else}
\end{cases}
    \end{align*}
\end{Definition}
% Comparison and boolean operators are defined as:
% \begin{enumerate}

% \item \[\ubMarker{(a>b)} = \ubMarker{a}>\lbMarker{b}\] \\
% \[\lbMarker{(a>b)} = \lbMarker{a}>\ubMarker{b}\]

% \item \[\ubMarker{(a=b)} = \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b}\] \\

% \[\lbMarker{(a=b)} = (\ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} )\] \\

% \item \[ \ubMarker{(p \wedge q)} = \ubMarker{p} \wedge \ubMarker{q} \]
% \[ \lbMarker{(p \wedge q)} = \lbMarker{p} \wedge \lbMarker{q} \]
% \item \[ \ubMarker{(p \vee q)} = \ubMarker{p} \vee \ubMarker{q} \]
% \[ \lbMarker{(p \vee q)} = \lbMarker{p} \vee \lbMarker{q} \]
% \end{enumerate}
% For arithmetic and conditional scalar expressions $a$ and $b$, we define expression evaluation in $\rangeDom$ as follows:
% \begin{enumerate}
% 	\item $ \ubMarker{(a+b)} = \ubMarker{a} + \ubMarker{b} $ \\
% 	$ \lbMarker{(a+b)} = \lbMarker{a} + \lbMarker{b} $
%     \item $ \ubMarker{(a-b)} = \ubMarker{a} - \lbMarker{b} $ \\
% 	$ \lbMarker{(a-b)} = \lbMarker{a} - \ubMarker{b} $
% 	\item $ \ubMarker{(a \cdot b)} = max(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b}) $ \\
% 	$ \lbMarker{(a \cdot b)} = min(\ubMarker{a} \cdot \ubMarker{b},\ubMarker{a} \cdot \lbMarker{b},\lbMarker{a} \cdot \ubMarker{b},\lbMarker{a} \cdot \lbMarker{b}) $
% \]
% \end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preservation of Bounds}\label{sec:range-expr-eval-preserves-bounds}

Assuming that an input range-annotated valuation bounds an incomplete valuation, we need to prove that the output of range-annotated expression evaluation also  bounds the possible outcomes produced for the incomplete valuation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Bounding sets of values]\label{def:bounding-vals}
  A value $c \in \rangeDom$ is said to bound a set of values $S = \{c_1, \ldots, c_n\}$ from $\dataDomain$ if:
  \begin{align*}
    \forall c_i \in S: \lbMarker{c} \leq c_i \leq \ubMarker{c}\\
    \exists c_i \in S: c_i = \bgMarker{c}
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Bound Preservation]\label{theo:expr-bound}
  Let $\sexpr$ be an expression, $\uval$ an incomplete valuation for $\sexpr$, and $\rval$ a range-annotated valuation for $\sexpr$ that bounds $\uval$, then $\seval{\sexpr}{\rval}$ bounds $\seval{\sexpr}{\uval}$.

  % with range annotated variable binding $\mathbb{V} \rightarrow \rangeDom$. If all variable bindings are bounds a possible outcomes binding $\mathbb{V} \rightarrow \{\dataDomain\}$. Then the range annotated expression evaluation result also bounds the evaluation result for all possible outcomes.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  We prove this theorem through induction over the structure of an expression under the assumption that $\rval$ bounds $\uval$.

\proofpara{Base case}
If $e \defas c$ for a constant $c$, then $\lbMarker{e} = \bgMarker{e} = \ubMarker{e} = c$ which is also the result of $e$ in any possible world of $\uval$. If $e \defas x$ for a variable $x$, then since $\rval$ bounds $\uval$, the value of $x$ in any possible world is bounded by $\rval(x)$.

\proofpara{Induction step}
Assume that for expressions $e_1$, $e_2$, and $e_3$, we have that their results under $\uval$ are bounded by their result under $\rval$:

\begin{align*}
\forall i \in \{1,2,3\}: \forall c \in \seval{e_i}{\uval}: \lbMarker{\seval{e_i}{\rval}} \leq c \leq \ubMarker{\seval{e_i}{\rval}}\\
\exists \sval \in \uval: \forall i \in \{1,2,3\}: \bgMarker{\seval{e_i}{\rval}} = \seval{e_i}{\sval}
\end{align*}
Note that the second condition trivially holds since $\bgMarker{\seval{e}{\rval}}$ was defined as applying deterministic expression semantics to $\bgMarker{\rval}$. We, thus, only have to prove  that the lower and upper bounds are preserved for all expressions $e$ that combine these expressions using one of the scalar operators.

\proofpara{$e \defas e_1 + e_2$}
Inequalities are preserved under addition. Thus, for any $\sval \in \uval$ we have $\lbMarker{\seval{e_1}{\rval}} + \lbMarker{\seval{e_2}{\rval}} \leq \seval{e_1}{\sval} + \seval{e_2}{\sval} \leq \ubMarker{\seval{e_1}{\rval}} + \ubMarker{\seval{e_2}{\rval}}$.

\proofpara{$e \defas e_1 \cdot e_2$}
We distinguish sixteen cases based on which of $\lbMarker{\seval{e_1}{\rval}}$, $\lbMarker{\seval{e_2}{\rval}}$, $\ubMarker{\seval{e_1}{\rval}}$, and $\lbMarker{\seval{e_2}{\rval}}$ are negative. For instance, if all numbers are positive then clearly $\lbMarker{\seval{e_1}{\rval}} \cdot \lbMarker{\seval{e_2}{\rval}} \leq \seval{e_1}{\sval} \cdot \seval{e_2}{\sval}$. While there are sixteen cases, there are only four possible combinations of lower and upper bounds we have to consider. Thus, if we take the minimal (maximal) value across all these cases, we get a lower (upper) bound on $e$.

\proofpara{$e \defas e_1 \wedge e_2$ and $e \defas e_1 \vee e_2$}
Both $\vee$ and $\wedge$ are monotone in their arguments wrt. the order $F \ordB T$. Thus, applying these operations to combine lower (upper) bounds preserves these bounds.

\proofpara{$e \defas \neg\,e_1$}
We distinguish three cases: (i) $\seval{e_1}{\sval} = \bfalse$ for any $\sval \in \uval$; (ii)$\seval{e_1}{\sval} = \btrue$ for some $\sval \in \uval$ and $\seval{e_1}{\sval} = \btrue$ for some $\sval \in \uval$; and (iii) $\seval{e_1}{\sval} = \btrue$ for any $\sval \in \uval$. In case (i) either $\seval{e_1}{\rval} = (\bfalse,\bfalse,\bfalse)$ in which case $\seval{e}{\rval} = (\btrue,\btrue,\btrue)$ or $\seval{e_1}{\rval} = (\bfalse,\bfalse,\btrue)$ and $\seval{r}{\rval} = (\bfalse,\btrue,\btrue)$. We have $\seval{e}{\sval} = \btrue$ for any $\sval \in \uval$ and, thus, in either case $\seval{e}{\rval}$ bounds $\seval{e}{\uval}$. In case (ii), $\lbMarker{\seval{e}{\rval}} = \bfalse$ and $\ubMarker{\seval{e}{\rval}} = \btrue$ which trivially bound $\seval{e}{\uval}$. The last case is symmetric to (i).

\proofpara{$e \defas e_1 \leq e_2$}
Recall that $\bfalse \leq \btrue$.  $e_1 \leq  e_2$ is guaranteed to evaluate to true in every possible world if the upper bound of $e_1$ is lower than or equal to the lower bound of $e_2$. In this case it is safe to set $\lbMarker{\seval{e}{\rval}} = \btrue$. Otherwise, there may exist a possible world where $e_1 \leq e_2$ evaluates to false and we have to set $\lbMarker{\seval{e}{\rval}} = \bfalse$. Similarly, if the lower bound of $e_1$ is larger than the upper bound of $e_2$ then $e_1 \leq e_2$ evaluates to false in every possible world and $\ubMarker{\seval{e}{\rval}} = \bfalse$ is an upper bound. Otherwise, there may exist a world where $e_1 \leq e_2$ holds and we have to set $\ubMarker{\seval{e}{\rval}} = \btrue$.

\proofpara{$\ifte{e_1}{e_2}{e_3}$}
When $e_1$ is certainly true ($\lbMarker{\seval{e_1}{\rval}} = \lbMarker{\seval{e_1}{\rval}} = \btrue$) of certainly false ($\lbMarker{\seval{e_1}{\rval}} = \lbMarker{\seval{e_1}{\rval}} = \bfalse$) then the bounds $e_2$ (certainly true) or $e_3$ (certainly false) are bounds for $e$. Otherwise, $e$ may evaluate to $e_2$ in some worlds and to $e_3$ in others. Taking the minimum (maximum) of the bounds for $e_2$ and $e_3$ is guaranteed to bound $e$ from below (above) in any possible world.

% 	\begin{itemize}
% 		% \item For operation $a+b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. So $\lbMarker{a}+\lbMarker{b} \leq a+b \leq \ubMarker{a}+\ubMarker{b}$. So the result is bounded.
% 	 	% \item For operation $a-b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. So $\lbMarker{a}-\ubMarker{b} \leq a-b \leq \ubMarker{a}-\lbMarker{b}$. So the result is bounded.
% 	 	% \item For operation $a \cdot b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. If $\lbMarker{a}>0$ and $\lbMarker{b}>0$ then $\lbMarker{a} \cdot \lbMarker{b} \leq a \cdot b$. Else if $\ubMarker{a}<0$ and $\ubMarker{b}<0$ then $\ubMarker{a} \cdot \ubMarker{b} \leq a \cdot b$. Else if $\lbMarker{a}>0$ and $\lbMarker{b}<0$ then $\ubMarker{a} \cdot \lbMarker{b} \leq a \cdot b$ or $\ubMarker{b} \cdot \lbMarker{a} \leq a \cdot b$. Same apply to the upper bounds symmetrically. So the result is bounded.
% 	 	\item For operation $a>b$, by definition $\lbMarker{a} \leq a \leq \ubMarker{a}$ and $\lbMarker{b} \leq b \leq \ubMarker{b}$. So it is possible for $a>b$ to be true iff $\ubMarker{a} > \lbMarker{b}$. It is possible for $a>b$ to be false iff $!(\lbMarker{a} > \ubMarker{b})$. So the result is bounded.
% 	 	\item For operation $a=b$, It is possible for $a=b$ to be true iff the bounds of the two inputs are overlapped. It is possible for $a=b$ to be false iff two values are not certainly equal. So the result is bounded.
% 	 	% \item For operation $a \wedge b$, It is possible for $a \wedge b$ to be true iff $\ubMarker{a}$ and $\ubMarker{b}$ is true. It is possible for $a \wedge b$ to be false iff $\lbMarker{a}$ or $\lbMarker{b}$ is false. So the result is bounded.
% 	 	% \item For operation $a \vee b$, It is possible for $a \vee b$ to be true iff $\ubMarker{a}$ or $\ubMarker{b}$ is true. It is possible for $a \wedge b$ to be false iff $\lbMarker{a}$ and $\lbMarker{b}$ is false. So the result is bounded.
% 	 	\end{itemize}

% \SF{Feels the boolean operators proofs are little shaky, maybe use contradictions?}

We conclude that the result of range-annotated expression evaluation under $\rval$ which bounds an incomplete valuation $\uval$ bounds the result of incomplete expression evaluation for any expression $e$.
% our expression evaluation model is bounded by the fact that any expression is recursively start with the base case which is bounded, and all the operator result is bounded given the input is bounded.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Categorical Domains}
% \label{sec:cate-doms}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\captialUAADBs}
\label{sec:uaa-range}

In this section we define \termUAADBs (\abbrUAADBs) as relations over range-annotated domains and demonstrate how to bound an incomplete $\semK$-relation using this model. Afterwards, we define a metric for how precise the bounds of an incomplete $\semK$-database encoded by a \abbrUAADB are. We then proceed to define a query semantics for \abbrUAADBs and prove that this query semantics preserves bounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\abbrUAADBs}\label{sec:uaadbs}

In addition to allowing for range-annotated values, \abbrUAADBs also differ from \abbrUADBs in that they encode an upper bound of the possible annotation of tuples. Thus, instead of using annotations from $\aDoubleK$, we use $\semkq$ annotations to encode three annotations for each tuple: a lower bound on the certain annotation of the tuple, the annotation of the tuple in the \abbrBGW, and an over-approximation of the tuple's possible annotation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Tuple-level Annotations]\label{def:uaa-tuple-annot}
  Let $\semK$ be an l-semiring and let $\ordK$ denote its natural order. Then the tuple level range-annotated domain $\uaaDom{\domK}$ is defined as:

  $$\{ (\lbMarker{k}, k, \ubMarker{k}) \mid k, \lbMarker{k}, \ubMarker{k} \in \semK \wedge \lbMarker{k} \ordK k \ordK \ubMarker{k} \}$$
We use $\uaaK{\semK}$ to denote semiring $\semkq$ restricted to elements from $\uaaDom{\domK}$.
  \end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



  Similar to the range-annotated domain, a value $(k_1, k_2, k_3)$ from
  $\uaaK{\semK}$ encodes a semiring element from $\semK$ and two elements ($k_1$
  and $k_3$) that bound the element from below and above.  Given an
  $\uaaK{\semK}$-element $k = \ut{k_1}{k_2}{k_3}$ we define
  $\lbMarker{k} = k_1$, $\bgMarker{k} = k_2$, and $\ubMarker{k} = k_3$.  Note
  that $\uaaK{\semK}$ is a semiring since when combining two elements of
  $\uaaK{\semK}$ with $\addOf{\semkq}$ and $\multOf{\semkq}$, the result
  $(k_1, k_2, k_3)$ fulfills the requirement $k_1 \ordK k_2 \ordK k_3$. This is
  the case because in general semiring addition and multiplication preserves
  natural order and these operations in $\semkq$ are defined as pointwise
  application of $\addK$ and $\multK$, e.g.,
  $(\lbMarker{k}, k, \ubMarker{k}) \addOf{\semkq} (\lbMarker{l}, l,
  \ubMarker{l}) = (\lbMarker{l} \addK \lbMarker{l}, k \addK l, \ubMarker{k}
  \addK \ubMarker{l}))$ and
  $k_1 \ordK k_2 \wedge k_3 \ordK k_4 \Rightarrow k_1 \addK k_3 \ordK k_2 \ordK
  k_4$ for any $k_1, k_2, k_3, k_4 \in \semK$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[$\uaaK{\semK}$-relations]\label{def:uaa-rels}
	Given a range-annotated data domain $\rangeDom$ and l-semiring $\semK$, an $\uaaK{\semK}$-relation of arity $n$ is a function $\rel: \rangeDom^n \rightarrow \uaaK{\semK}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As a notational convenience we show certain values, i.e., values $c \in \rangeDom$ where $\lbMarker{c} = \bgMarker{c} = \ubMarker{c} = c'$, as the deterministic value $c'$ they encode.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Extracting \termBGWs}\label{sec:uaab-get-bgw}

Note that the same tuple $\tup$ may appear more than once in a $\uaaK{\semK}$-relation albeit with different value annotations.
We can extract the \termBGW encoded by a $\uaaK{\semK}$-relation by grouping tuples by the \abbrBG annotations of their attribute values and then summing up their tuple-level \abbrBG annotation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:bool-to-K}
We lift function $\bgName$ from values to tuples: $\bgName: \rangeDom^n \to \dataDomain^n$, i.e., given an \abbrUAADB tuple $\rangeTup = (v_1, \ldots, v_n)$, $\bgOf{\rangeTup}$ is defined  as $\bgOf{\rangeTup} = (\bgMarker{v_1}, \ldots, \bgMarker{v_n})$. For a  $\uaaK{\semK}$-relation $\rangeRel$, $\bgOf{\rangeRel}$, the \abbrBGW encoded by $\rangeRel$, is then defined as:
$$\bgOf{\rangeRel}(\tup) \defas \sum_{\bgOf{\rangeTup} = \tup} \bgOf{\rangeRel(\rangeTup)}$$
%  The corresponding $\uaak{\semK}$-relation  $D_{bg}=\{t \rightarrow \sum_{BG(\rangeTup)=t} \rangeTup.k\}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{ex:audb-instance}
Figure~\ref{table:UAAR_inst} shows an instance of a $\uaaK{\semN}$-relation $\rel$ where each attribute is a triple showing the lower bound, best guess and upper bound of the value. Each tuple is annotated by a triple showing the lower bound, best guess and upper bound of the annotation value. Since this is a $\uaaK{\semN}$ relation, the annotations encode multiplicities of tuples. For example, the first tuple represents a tuple $(1,1)$ that appears at least twice in every possible world (its lower bound annotation is $2$), appears twice in the \abbrBGW, and may appear in any possible world at most thrice.
	Figure~\ref{table:UAAR_bg} shows the \abbrBGW encoded by\abbrUAADB produced by summing up the annotations of tuples with identical \abbrBG values. For instance, the first two tuples both represent tuple $(1,1)$ and their annotations sum up to $5$, i.e., the tuple $(1,1)$ appears five times in the chosen \abbrBGW.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
	\centering

    \begin{minipage}{0.485\linewidth}
	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|cc}
      \textbf{A}  & \textbf{B}  & \underline{\semqN} \\
      				\cline{1-2}
		$\uv{1}{1}{1}$ & $\uv{1}{1}{1}$ & \ut{2}{2}{3}\\
		$\uv{1}{1}{1}$ & $\uv{1}{1}{3}$ & \ut{2}{3}{3}\\
		$\uv{1}{2}{2}$ & $\uv{3}{3}{3}$ & \ut{1}{1}{1}\\
	\end{tabular}
	\caption{An example \abbrUAADB instance}
	\label{table:UAAR_inst}
	\end{subtable}
  \end{minipage}
  \begin{minipage}{0.485\linewidth}
	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|cc}
		\textbf{A}  & \textbf{B}  & \underline{$\semN$}  \\
		\cline{1-2}
		$1$ & $1$ & 5\\
		$2$ & $3$ & 1\\
	\end{tabular}
	\caption{Extracted \termBGW}
	\label{table:UAAR_bg}
	\end{subtable}
  \end{minipage}
	\caption{Example \abbrUAADB relation and the \abbrBGW it encodes}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[ht]
%   \BG{F and T should be introduced beforehand}
% 	\centering
% 	\begin{subtable}{0.4\linewidth}
% 	\centering
% 	\caption{R-D1}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  &  \\
% 		\cline{1-2}
% 		1 & 1 & 2\\
% %				\cline{1-3}
% 		1 & 2 & 3\\
% %				\cline{1-3}
% 		2 & 3 & 1\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}
% 	\begin{subtable}{0.4\linewidth}
% 	\centering
% 	\caption{R-D2}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  &  \\
% 		\cline{1-2}
% 		1 & 1 & 3\\
% %				\cline{1-3}
% 		1 & 2 & 2\\
% %				\cline{1-3}
% 		1 & 3 & 2\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB BG=D1 \\ Similar to tuple level}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
% %				\cline{1-3}
% 		$1^{[1,1]}$ & $2^{[2,2]}$ & (2,3,3)\\
% %				\cline{1-3}
% 		$2^{[2,2]}$ & $3^{[3,3]}$ & (0,1,1)\\
% 		$1^{[1,1]}$ & $3^{[3,3]}$ & (0,0,2)\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB one-liner}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,2]}$ & $1^{[1,3]}$ & (6,6,7)\\
% %				\cline{1-3}
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB BG=D1}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
% %				\cline{1-3}
% 		$1^{[1,1]}$ & $2^{[2,3]}$ & (3,3,3)\\
% %				\cline{1-3}
% 		$2^{[1,2]}$ & $3^{[3,3]}$ & (1,1,1)\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB GB=D1 tuple matchings}
% 	\begin{tabular}{ |c|}
% 				\cline{1-1}
% 		\textbf{Certain matching}\\
% 		\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D1(1,2) = 3$\\
% %				\cline{1-3}
% 		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D1(2,3) = 1$\\
% 				\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,2) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,3) = 1$\\
% 		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D2(1,3) = 1$\\
% 			\cline{1-1}
% 		\textbf{Possible matching} \\
% 		\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 1$\\
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 1$\\
% 		\cline{1-1}
% 	\end{tabular}
% 	\end{subtable}
% \BG{Do we need this long example here?}
% \caption{A \abbrUAADB-DB instance correspond to possible worlds semantics}
% \label{fig:exp1}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Encoding Bounds}\label{sec:uaadb-bounds}

We now formally define what it means for an \abbrUAADB to bound a an incomplete $\semK$-relation from above and below. For that we first define bounding of deterministic tuples by range-annotated tuples bound (match).
%We use \abbrUAADB relation to bound all possible worlds from an incomplete database. Starting from bounding a tuple from each possible world to a \abbrUAADB tuple.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Tuple Bounding]\label{def:bounding-tuples}
  Let  $\rangeTup$ be a  range-annotated tuple with schema $(a_1, \ldots, a_n)$ and   $\tup$ be a tuple  with same schema as $\rangeTup$. We say that $\rangeTup$ bounds $\tup$ written as $\tup \tmatch \rangeTup$ iff
  $$\forall{i \in \{1, \ldots ,n\}}:
  \lbMarker{\rangeTup.a_i} \leq \tup.a_i \leq \ubMarker{\rangeTup.a_i}$$
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Bounding $\uaaK{\semK}$ Annotations]\label{def:bounding-annotations}
% 	A value $k \in \uaaK{\semK}$ is said to bound a set of values $S_k = \{k_1, \ldots, k_n\}$ from $\semK$ if:
%   \begin{align*}
%     \forall k_i \in S_k: \lbMarker{k} \leq k_i \leq \ubMarker{k}\\
%     \exists k_i \in S_k: k_i = \bgMarker{k}
%   \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Obviously, one \abbrUAADB tuple can bound multiple different conventional tuples and vice versa. We introduce \textit{tuple matching} as a way to match the tuples and their annotations of a $\uaaK{\semK}$-database (or relation) with that of one possible world.
Based on tuple matchings we then define bounding of possible worlds.
% a mapping between a set of \abbrUAADB tuples and a set of deterministic tuples.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Tuple matching]\label{def:tuple-matching}
  Let $n$-ary \abbrUAADB  $\rangeRel$ and an $n$-ary database $R$. A tuple matching $\TM$ for $\rangeRel$ and $\rel$ is a function $(\rangeDom)^{n} \times \dataDomain^n \to \semK$.
  % $$TM_{R^I,R}(\rangeTup,t)=k$$ is the mappings from an annotated tuple $\rangeTup$ and a possible world tuple $t$ to a semiring element $k$
  \st
$$\forall \rangeTup \in \rangeDom^n: \forall \tup \ntmatch \rangeTup: \TM(\rangeTup,\tup) = \zeroK$$
and
$$\forall \tup \in \dataDomain^n: \sum_{\rangeTup \in \rangeDom^n} \TM(\rangeTup,\tup)=\rel(\tup)$$
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Intuitively, a tuple matching distributes the annotation of a tuple from $\rel$ over one or more matching tuples from $\rangeRel$. That is, multiple tuples from a \abbrUADB may encode the same tuple from an incomplete database. This is possible when the multidimensional rectangles of their attribute-level range annotations overlap. For instance, range-annotated tuples $(\uv{1}{2}{3})$ and $(\uv{2}{3}{5})$ both match the tuple $(2)$.
% The conditions stating that a \abbrUAADB tuple can only match to conventional tuple if the tuple is bounded by the \abbrUAADB tuple. Also all the conventional tuples in relation $\rel$ need to be matched in the tuple matching.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Bounding Possible Worlds]\label{def:bounding-worlds}
  Given an n-ary \abbrUAADB  relation $\rangeRel$ and a n-ary deterministic relation $\rel$ (a possible world of an incomplete $\semK$-relation),  relation $\rangeRel$ is a lower bound for $\rel$ iff there exists a tuple matching $\TM$ for $\rangeRel$ and $\rel$ \st

  \begin{align}\label{eq:lower-bound-db}
    \forall \rangeTup \in \rangeDom^n:\sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \geqK \lbMarker{\rangeRel(\rangeTup)}
  \end{align}

  and is upper bounded by $\rangeRel$ iff there exists a tuple matching $\TM$ for $\rangeRel$ and $\rel$ \st

  \begin{align}\label{eq:upper-bound-db}
    \forall \rangeTup \in \rangeDom^n: \sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \ordK \ubMarker{\rangeRel(\rangeTup)}
  \end{align}

  A relation $\rel$ is bounded by an \abbrUAADB relation $\rangeRel$ written as $\rel \dbbounds \rangeRel$ iff there exists a tuple matching $\TM$ for $\rangeRel$ and $\rel$ that fulfills both \Cref{eq:lower-bound-db,eq:upper-bound-db}.
  \end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Having defined when a possible world is bound by a $\uaaK{\semK}$-relation, we are ready to define bounding of incomplete $\semK$-relations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Bounding incomplete databases]\label{def:bounding-incomplet-dbs}
	Given an incomplete database $\pdb$ and a \abbrUAADB database $\rangeDB$, we say that $\rangeDB$ bounds $\pdb$, written as $\pdb \dbbounds \rangeDB$
  iff
    \begin{align}
    \forall \db \in \pdb: \db \dbbounds \rangeDB\\
    \exists \db \in \pdb: \bgOf{\rangeDB} = \db
    \end{align}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that all bounds we define for relations are extended to databases in the obvious way.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{def:bounding-incomplete-dbs}
  Consider the \abbrUAADB from \Cref{ex:audb-instance} and the two possible world shown below \Cref{ex:audb-instance}. The \abbrUAADB bounds these worlds, since there exist tuple matchings that provides both a lower and an upper bound for the annotations of the tuples of these worlds. For instance, denoting the tuples from this example as
  \begin{align*}
    \rangeTup_1                & \defas (\uv{1}{1}{1}, \uv{1}{1}{1})
                               & \rangeTup_2                & \defas (\uv{1}{1}{1}, \uv{1}{1}{3})
                               & \rangeTup_3                & \defas (\uv{1}{2}{2}, \uv{3}{3}{3}) \\
  \end{align*}
  we can construct a tuple matching $\TM_1$ and $\TM_2$ to bound $\db_1$ and $\db_2$, respectively.
  \begin{align*}
    \TM_1(\rangeTup_1, \tup_1) & = 2
                               & \TM_1(\rangeTup_2, \tup_1) & = 3
                               & \TM_1(\rangeTup_3, \tup_1) & = 0                                 \\
    \TM_1(\rangeTup_1, \tup_2) & = 0
                               & \TM_1(\rangeTup_2, \tup_2) & = 0
                               & \TM_1(\rangeTup_3, \tup_2) & = 1                                 \\[2mm]
    \TM_2(\rangeTup_1, \tup_3) & = 2
                               & \TM_2(\rangeTup_2, \tup_3) & = 0
                               & \TM_2(\rangeTup_3, \tup_3) & = 0                                 \\
    \TM_2(\rangeTup_1, \tup_4) & = 0
                               & \TM_2(\rangeTup_2, \tup_4) & = 2
                               & \TM_2(\rangeTup_3, \tup_4) & = 0                                 \\
    \TM_2(\rangeTup_1, \tup_5) & = 0
                               & \TM_2(\rangeTup_2, \tup_5) & = 0
                               & \TM_2(\rangeTup_3, \tup_5) & = 1
  \end{align*}
  \begin{minipage}{0.49\linewidth}
    \centering
    \underline{$\db_1$}                                                                           \\
    	\begin{tabular}{lc|cc}
                               & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
		\cline{2-3}
$\tup_1$                       & $1$                        & $1$        & 5                      \\
$\tup_2$                       & $2$                        & $3$        & 1                      \\
	\end{tabular}
  \end{minipage}
  \begin{minipage}{0.49\linewidth}
    \centering
    \underline{$\db_2$}                                                                           \\
    \begin{tabular}{lc|cc}
                               & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
		\cline{2-3}
 $\tup_3$                      & $1$                        & $1$        & 2                      \\
 $\tup_4$                      & 1                          & 3          & 2                      \\
$\tup_5$                       & $2$                        & $4$        & 1                      \\
	\end{tabular}
  \end{minipage}
    \end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BG{removed this: fig:exp1 shows an example of a \abbrUAADB-DB with a possible tuple matching that fulfills the correctness criteria.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tightness of Bounds}
\label{sec:approximation-factor}

\Cref{def:bounding-incomplet-dbs} defines what it means for an \abbrUAADB to bound an incomplete databases. However, given an incomplete database, there may be many possible \abbrUAADBs that bound it that differ in how tight the bounds are. For instance, both $\tup_1 \defas (\uv{1}{15}{100})$ and $\tup_2 \defas \uv{13}{14}{15}$ bound tuple $(15)$, but intuitively the bounds provided by the second tuple are tighter. In this section we develop a metric for the tightness of the approximation provided by an \abbrUAADB and prove that finding a \abbrUAADB that maximizes tightness when we limit the size of the \abbrUAADB is intractable. Intuitively, given two \abbrUAADBs $\rangeDB$ and $\rangeDB'$ that both bound an incomplete $\semK$-database $\db$, $\rangeDB$ is a tighter bound than $\rangeDB'$ if the set of deterministic databases bound by $\rangeDB$ is a subset of the set of deterministic databases bound by $\rangeDB'$. As a sanity check, consider $\rangeDB_1 \defas \{t_1\}$ and $\rangeDB_2 \defas \{t_2\}$ using $t_1$ and $t_2$ from above and assume that $\dataDomain = \semN$. Then $\rangeDB_2$ tigher bound than $\rangeDB_1$ since the three deterministic databases it bounds $\{(13)\}$, $\{(14)\}$ and $\{(15)\}$ are also bound by $\rangeDB_1$, but $\rangeDB_1$ bounds additional databases, e.g., $\{(2)\}$ that are not bound by $\rangeDB_2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Bound Tightness]\label{def:bound-tightness}
  Consider two $\uaaK{\semK}$-databases $\rangeDB$ and $\rangeDB'$ over the same schema
$\aschema$. We say that $\rangeDB$ is at least as tight as $\rangeDB'$, written as $\rangeDB \dbleq \rangeDB'$, if for all $\semK$-databases $\db$ with schema $\aschema$ we have:
  \begin{align*}
 \db \dbbounds \rangeDB \rightarrow \db \dbbounds \rangeDB'
  \end{align*}
  We say that $\rangeDB$ is a strictly tighter than $\rangeDB$, written as $\rangeDB \dble \rangeDB'$ if $\rangeDB \dbleq \rangeDB'$ and there exists $\db \dbbounds \rangeDB'$ with $\db \not\dbbounds \rangeDB$. Furthermore, we call $\rangeDB$  a maximally tight bound for an incomplete $\semK$-database $\pdb$ if:
  \begin{align*}
    &\pdb \dbbounds \rangeDB\\
   \not \exists \rangeDB': &\rangeDB' \dble \rangeDB
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that the notion of tightness is well-defined even if the data domain $\dataDomain$ is infinite. For instance, if we use the reals $\mathbb{R}$ instead of natural numbers as the domain in the example above, then still $\rangeDB_1 \dbge \rangeDB_2$.
In general \abbrUAADBs that are tighter bounds are preferable. However, computing a maximally tight bound is intractable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Finding Maximally Tight Bounds]\label{def:intractability-of-tight-bounds}
Let $\pdb$ be an incomplete $\uaaK{\semK}$-database. It is \nphard in the size of $\pdb$ to compute a maximally tight bound $\rangeDB$ for $\pdb$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
\BG{Need to find reduction that works.}
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the light of this result, the efficient methods for translating incomplete and probabilistic databases into \abbrUAADBs do not guarantee tight bounds. Furthermore, even if the input is maximally tight, our query semantics does not preserve this property. Note that this strictly necessary since computing tight bounds on aggregation function results is already hard in incomplete and probabilistic databases (e.g., see~\cite{DBLP:journals/tcs/ArenasBCHRS03}). Nonetheless, comparing the tightness of \abbrUAADBs is useful for evaluating how tight bounds are in practice as we will do in \Cref{sec:experiments}.

%\subsection{Tuple matching}
%Define matching $t' \tmatches t$ as true iff $\forall{i \in [1,n]}:t(a_i) \in I_{t'(a_i)}$ \\
%A tuple matching $TM_{R',R}(t',t)=k$ is the mappings from an annotated tuple $t'$ and a possible world tuple $t$ to a semiring value $k$. \\
%As a constrain, any tuple matching need to fully match all certain tuples from annotated relation:
%$$\forall_{t' \in R'}:\sum_{t \in R}TM_{R',R}(t',t)=R'(t').k_c$$
%A annotated relation $R'$ is c-sound if:
%$$\forall_{D(R) \in \dataDomain}:\exists TM_{R',R}:\forall_{t \in R}:\sum_{t' \in R'}TM_{R',R}(t',t) \leq R(t)$$
%A annotated relation $R'$ is p-complete if:
%$$\forall_{t' \in R'}:\sum_{t \in R}TM_{R',R}(t',t)=R'(t').k_p$$
%$$\forall_{D(R) \in \dataDomain}:\exists TM_{R',R}:\forall_{t \in R}:\sum_{t' \in R'}TM_{R',R}(t',t) \geq R(t)$$



%%%
%\subsection{Certain tuples based tuple matching}
%In certain tuples based tuple matching, we match annotated tuples to certain tuples in all possible worlds.\\
%An annotated relation $R'$ is c-sound if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \leq certain(\dataDomain)(t)$$
%A annotated relation $R'$ is c-complete if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \geq certain(\dataDomain)(t)$$
%%%

%\subsection{Expressions}
%An attribute $x$ is certain iff the upper bound and lower bound of the attribute are equal.
%Comparison and boolean operators can be defined as:
%\begin{enumerate}
%\item \[ \begin{cases}
%\ubMarker{(a>b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \\
%\ubMarker{(a>b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\[ \begin{cases}
%\lbMarker{(a>b)} = T & \text{if } \lbMarker{a}>\ubMarker{b} \\
%\lbMarker{(a>b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\item \[ \begin{cases}
%\ubMarker{(a=b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
%\ubMarker{(a=b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\[
%\begin{cases}
%\lbMarker{(a=b)} = \btrue & \text{if } \ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} \\
%\lbMarker{(a=b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\item \[ \ubMarker{(p \wedge q)} = \ubMarker{p} \wedge \ubMarker{q} \]
%\[ \lbMarker{(p \wedge q)} = \lbMarker{p} \wedge \lbMarker{q} \]
%\item \[ \ubMarker{(p \vee q)} = \ubMarker{p} \vee \ubMarker{q} \]
%\[ \lbMarker{(p \vee q)} = \lbMarker{p} \vee \lbMarker{q} \]
%\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\abbrUAADB Query Semantics}
\label{sec:uaadb-query-semantics}

In this section we first introduce a semantics for $\raPlus$ queries over \abbrUAADBs that preserves bounds, i.e., if the input of a query $\query$ bounds an incomplete $\semK$-database $\pdb$, then the output bounds $\query(\pdb)$. Conveniently, it turns out that the standard query semantics for  $\semK$-relations with a slight extension to deal with uncertain boolean values in conditions is sufficient for this purpose. Recall from \Cref{sec:expression} that conditions (or more generally scalar expressions) over range-annotated values evaluate to triples of boolean values, e.g., $\uv{F}{F}{T}$ would mean that the condition is false in some worlds, is false in the \abbrBGW, and may be true in some worlds. Recall the standard semantics for evaluating selection conditions over $\semK$-relations. For a selection $\selection_{\theta}(R)$ the annotation of a tuple $t$ in annotation of $\tup$ in the result of the selection is computed by multiplying $\rel(\tup)$ with $\theta(\tup)$ which is defined as a function $\semB \to \{ \zeroK, \oneK \}$ that returns $\oneK$ if $\theta$ evaluates to true on $\tup$ and $\zeroK$ otherwise. In $\uaaK{\semK}$-relations tuple $\tup$ is a tuple of range-annotated values and, thus,  $\theta$ evaluates to an range-annotated Boolean value as described above.



Turns out that \abbrUAADB relations follows the standard k-relational querying semantics by treating range annotations as a vector of semiring values $(\lbMarker{k},k,\ubMarker{k})$. As defined in \Cref{sec:expression}, the selection condition evaluates to a triple of boolean values $\semB^3$ and we need to map it to corresponding semiring elements that works for selection querying semantics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Boolean to Semiring Mapping]\label{def:lift-bool-to-K}
  Let $\semK$ be a semiring. We define a mapping function $\rliftK{\semK}:\semB^3 \rightarrow \semK^3$ as:
  \begin{align*}
    \rliftK{\semK}(b_1,b_2,b_3) &\defas (k_1,k_2,k_3) \,\,\,\text{where}\\
    \forall i \in \{1,2,3\}: k_i &\defas
    \begin{cases} 1_k & \text{if } b_i = true\\
      0_k & \text{otherwise}
    \end{cases}
    \end{align*}
% 	\[ \rliftK{\semK}(b_1,b_2,b_3) = (k_1,k_2,k_3) \text{ s.t. } \\
% 	\forall i \in \{1,2,3\}: k_i = \begin{cases} 1_k & \text{if } b_i = true      \\
% 0_k                                                & \text{otherwise}
% \end{cases} \]
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We use the mapping of range-annotated Boolean values to $\uaaK{\semK}$ elements to define evaluation of selection conditions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Selection Conditions over Range-annotated Values]\label{def:range-selection}
  Let $\semK$ be a semiring, $\rangeTup$ a range-annotated tuple, and $\theta$ be a Boolean condition over variables representing attributes from $\rangeTup$. Furthermore, let $\rval_{\rangeTup}$ denote the range-annotated valuation that maps each variable to the corresponding value from $\rangeTup$. We define $\theta(\rangeTup)$, the result of the condition $\theta$ applied to $\rangeTup$ in semiring $\semK$ as:
  \begin{align*}
   \theta(\rangeTup) \defas \rliftK{\semK}(\seval{\theta}{\rval_{\rangeTup}})
  \end{align*}
  % For selection operation $\selection_\theta(R)$ following standard semiring querying sematics:
  %   \[ [\selection_\theta(R)](t)=R(t) \otimes \theta(t) \]
  %   Define $(\theta(t))$ is a triple $k^I$ s.t.
  %   \[ \theta(t)=\rliftK{\semK}(\seval{\theta(t)}{\rval}) \]
  \end{Definition}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{Example}\label{ex:selections}
    Consider the example $\uaaK{\semN}$-relation $\rel$ shown below. The single tuple $\rangeTup$ of this relation exists at least once in every possible world, twice in the \abbrBGW, and no possible world contains  more than $3$ tuples bound by this tuple.

    \begin{center}
      {\upshape
    \begin{tabular}{c|cc}
      \thead{A}    & \thead{B} & \underline{$\uaaK{\semN}$} \\ \cline{1-2}
      \uv{2}{1}{3} & $2$         & $\ut{1}{2}{3}$
    \end{tabular}
    }
  \end{center}

    To evaluate a query $\query \defas \selection_{A = 3}(\rel)$ over this relations, we first evaluate the expression $A = 2$ using range-annotated expression evaluation semantics. We get $\uv{1}{2}{3} = \uv{2}{2}{2}$ which evaluates to $\uv{F}{T}{T}$. Using $\rliftK{\semN}$, this value is mapped to $\ut{0}{1}{1}$. To calculate the annotation of the tuple in the result of the selection we then multiply these values with the tuple's annotation in $\rel$ and get:
    $$\rel(\rangeTup) \multOf{\uaaK{\semN}} \theta(\rangeTup) = \ut{1}{2}{3} \cdot \ut{0}{1}{1} = \ut{0}{2}{3}$$
    Thus, the tuple may not exist in every possible world of the query result, appears twice in the \abbrBGW query result, and occurs at most three times in any possible world of the query result.
  \end{Example}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preservation of Bounds}

For this query semantics to be useful, we need to prove that it preserves bounds. Intuitively, this is true because expressions are evaluated using our range-annotated expression semantics which preserves bounds on values and queries are evaluated in a direct-product semiring $\uaaK{\semN}$ for which semiring operations are defined point-wise. Furthermore, we utilize a result we have proven in \cite[Lemma 2]{FH18}: the operations of l-semirings preserve the natural order, e.g., if $k_1 \ordK k_2$ and $k_3 \ordK k_4$ then $k_1 \addK k_3 \ordK k_2 \addK k_4$.
% The annotations propagate through standard querying semantics by mapping the expression outputs to a triple of semiring values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}[\raPlus Queries Preserve Bounds]\label{lem:ra-plus-preserves-bounds}
Let $\pdb$ be an incomplete $\semK$-database, $\query$ be a $\raPlus$ query, and $\rangeDB$ be an $\uaaK{\semK}$-database that bounds $\db$. Then $\query(\rangeDB)$ bounds $\query(\pdb)$.
  % Under $\raPlus$, given $R$ is lower bounded by $R^I$ w.r.t. $TM_{R,R^I}$, there exist $TM'_{Q(R),Q(R^I)}$ s.t. $Q(R)$ is lower bounded by $Q(R^I)$.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{proof}
	We prove this lemma using induction over the structure of a relational algebra expression under the assumption that $\rangeDB$ bounds the input $\pdb$.

	\proofpara{Base case}
	The query $\query$ consists of a single relation access $\rel$. The result is bounded following from $\rangeDB \dbbounds \pdb$.

	\proofpara{Induction step}
Let $\rangeRel$ and $\rangeOf{S}$ bound $n$-ary relation $\rel$ and $m$-ary relation $S$. Consider $\db \in \pdb$ and let $\TM_\rel$ and $\TM_{S}$ be two tuple matchings based on which these bounds can be established for $\db$. We will demonstrate how to construct a tuple matching $\TM_Q$ based on which $\query(\rangeDB)$ bounds $\query(\db)$. From this then immediately follows that $\query(\pdb) \dbbounds \query(\rangeDB)$. Note that by definition of $\uaaK{\semK}$ as the 3-way direct product of $\semK$ with itself, semiring operations are point-wise, e.g., $\lbMarker{k_1 \addOf{\uaaK{\semK}} k_2} = \lbMarker{k_1} \addK \lbMarker{k_2}$. Practically, this means that queries are evaluated over each dimension individually. We will make use of this fact in the following. We only prove that $\TM_Q$ is a lower bound since the proof for $\TM_Q$ being an upper bound is symmetric.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\projection_U(\rangeRel)$}
Recall that for $\TM$ to be a tuple matching, two conditions have to hold: (i) $\TM(\rangeTup, \tup) = \zeroK$ if $\tup \not\tmatch \rangeTup$ and (ii) $\sum_{\rangeTup \in \rangeDom^n} \TM(\rangeTup,\tup) = \rel(\tup)$.
Consider an $U$-tuple $\tup$. Applying the definition of projection for $\semK$-relations we have:
\[
\projection_U(\rel)(\tup) = \sum_{\tup = \tup'[U]} \rel(\tup)
\]

Since $\TM_R$ is a tuple matching based on which $\rangeRel$ bounds $\rel$, we know that by the definition of tuple matching the sum of annotations assigned to a tuple $\tup$ by the tuple matching is equal to the annotation of the tuple in $\rel$):


\begin{equation}\label{eq:project-proof-annotation-equal-tm-sum}
\sum_{\tup = \tup'[U]} \rel(\tup) = \sum_{\tup = \tup'[U]} \sum_{\rangeTup \in \rangeDom^n} \TM_R(\rangeTup, \tup')
\end{equation}

By definition for any tuple matching $\TM$ we have $\TM(\rangeTup,\tup) = \zeroK$ if $\tup \not\tmatch \rangeTup$. Thus, \Cref{eq:project-proof-annotation-equal-tm-sum} can be rewritten as:

\begin{equation}
  \label{eq:2}
= \sum_{\tup = \tup'[U]} \sum_{\tup' \tmatch \rangeTup} \TM_R(\rangeTup, \tup')
\end{equation}

Observe that for any n-ary range-annotated $\rangeTup$ and n-ary tuple $\tup$ it is the case that $\tup \tmatch \rangeTup$ implies $\tup[U] \tmatch \rangeTup[U]$ (if $\rangeTup$ matches $\tup$ on all attributes, then clearly it matches $\tup$ on a subset of attributes). For pair  $\tup$ and $\rangeTup$ such that $\tup[U] \tmatch \rangeTup[U]$, but $\tup \not\tmatch \rangeTup$ we know that $TM_R(\rangeTup, \tup) = \zeroK$. Thus,

\begin{equation}
  \label{eq:3}
= \sum_{\tup = \tup'[U]} \sum_{\rangeTup = \rangeTup'[U] \wedge \tup \tmatch \rangeTup} \TM_R(\rangeTup', \tup')
\end{equation}

So far we have established that:

\begin{equation}
  \label{eq:4}
  \projection_U(\rel)(\tup) = \sum_{\tup = \tup'[U]} \sum_{\rangeTup = \rangeTup'[U] \wedge \tup \tmatch \rangeTup} \TM_R(\rangeTup', \tup')
\end{equation}

We now define $\TM_Q$ as shown below:
\begin{equation}
  \label{eq:5}
  \TM_Q(\rangeTup,\tup) \defas \sum_{\forall \rangeTup', \tup: \rangeTup'[U]=\rangeTup \wedge t'[U]=t}\TM_{R}(\rangeTup', \tup')
\end{equation}

$\TM_Q$ is a tuple matching since \Cref{eq:4} ensures that $\forall \tup \in \dataDomain^n: \sum_{\rangeTup \in \rangeDom^n} \TM(\rangeTup,\tup)=\rel(\tup)$ (second condition in the definition) and we defined $\TM_Q$ such that $\TM_Q(\rangeTup,\tup) = \zeroK$ if $\tup \not\tmatch \rangeTup$. What remains to be shown is that $\projection_U(\rangeRel)$  bounds $\projection_U(\rel)$  based on $\TM_Q$. Let $\card{U} = m$, we have to show that

\[
  \forall {\rangeTup \in \rangeDom^m}: \lbMarker{\projection_U(\rangeRel)(\rangeTup)} \ordK \sum_{\tup \in \dataDomain^m}\TM_Q(\rangeTup, \tup)
  \]

  Since addition in $\uaaK{\semK}$ is pointwise application of $\addK$, using the definition of projection over $\semK$-relations we have

  \[
    \lbMarker{\projection_U(\rangeRel)(\rangeTup)} = \sum_{\rangeTup'[U] = \rangeTup} R(\rangeTup')
  \]

Furthermore, since $\TM_R$ is a tuple matching based on which $\rangeRel$ bounds $\rel$,
\[
= \sum_{\rangeTup'[U] = \rangeTup \wedge t \in \dataDomain^n} \TM_R(\rangeTup, \tup)
  \]

  Using again the fact that $\tup \not \tmatch \rangeTup$ implies $\TM_R(\rangeTup, \tup) = \zeroK$,

  \begin{align*}
    = &\sum_{\forall \tup', \rangeTup': \rangeTup'[U] = \rangeTup \wedge \tup' \tmatch \rangeTup'} \TM_R(\rangeTup', \tup')\\
    = &\sum_{\tup \tmatch \rangeTup} \sum_{\forall \tup', \rangeTup': \rangeTup'[U] = \rangeTup \wedge \tup'[U] = \tup} \TM_R(\rangeTup', \tup')\\
    = &\sum_{\tup \tmatch \rangeTup} \TM_Q(\rangeTup,\tup)     = \sum_{\tup \in \dataDomain^m} \TM_Q(\rangeTup,\tup)
  \end{align*}

Since we have established that $ \lbMarker{\projection_U(\rangeRel)(\rangeTup)} \ordK \sum_{\tup \in \dataDomain^m} \TM_Q(\rangeTup,\tup)$, $\projection_U(\rangeRel)$ lower bounds $\projection_U(\rel)$ via $\TM_Q$.





% Thus, if any $U$-tuple $\tup$ and range-annotated $U$-tuple $\rangeTup$ we define

% \[
% \TM_Q(\rangeTup, \tup) = \sum_{\forall \tup' \in \dataDomain^n, \rangeTup' \in \rangeDom^n: \tup = \tup'[U] \wedge \rangeTup'[U] = \rangeTup} \TM_R(\rangeTup', \tup')
%   \]

%   then $\TM_Q$ fulfills condition (i). For (ii) we have to show that $\TM_Q(\rangeTup, \tup) \neq \zeroK$ implies that $\tup \tmatch \rangeTup$.



% Observe that for any range-annotated tuple $\rangeTup$, the set $\{ \tup \mid \tup \tmatch \rangeTup \}$ is a subset of $\{ \tup \mid \tup[U] \tmatch \rangeTup[U]\}$. Recall that the definition of tuple matching enforces that $\TM(\rangeTup, \tup) = \zeroK$ if $\tup \not\tmatch \rangeTup$. This implies for that any tuple matching $\TM$ it is the case that  $\sum_{\tup \tmatch \rangeTup} \TM(\rangeTup, \tup) = \sum_{\tup[U] \tmatch \rangeTup[U]} \TM(\rangeTup, \tup)$.


% Since n-ary relation $\rangeRel$ bounds $\rel$, by \Cref{def:tuple-matching}, we have
% %
% \begin{equation}\label{eq:project-proof-tm-bounds}
%   \forall {\rangeTup \in \rangeDom^n}: \lbMarker{\rangeRel(\rangeTup)} \ordK \sum_{\tup \in \dataDomain^n}\TM_\rel(\rangeTup, \tup)
% \end{equation}
% %



% Substituting the definition of projection over $\semK$-relations and
% recalling that addition in $\uaaK{\semK}$ is defined as pointwise application of $\addK$ we have:
% \[
%   \lbMarker{\left(\projection_U(\rangeRel)(\rangeTup)\right)}
%   =\lbMarker{\left(\sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}\rangeRel(\rangeTup') \right)}
%   =\sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}\rangeRel\lbMarker{(\rangeTup')}
% \]
% Using \Cref{eq:project-proof-tm-bounds}  and the fact that semiring addition preserves the natural order:
% \[
%   \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}\rangeRel\lbMarker{(\rangeTup')}
%   \ordK \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}  \sum_{\forall t \in \dataDomain^n}\TM_R(t,\rangeTup')
% \]
% %
% Recall that the definition of tuple matching (\Cref{def:tuple-matching}) enforces that for any tuple matching $\TM$ it is the case that $\TM(\rangeTup, \tup) = \zeroK$ if $\tup \not\tmatch \rangeTup$. Thus, we can rewrite the equation above into:
% \[
% = \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}\sum_{\forall \tup: \tup \tmatch \rangeTup'}\TM_R(t,\rangeTup')
% \]
% %
% Observe that for any range-annotated tuple $\rangeTup$, the set $\{ \tup \mid \tup \tmatch \rangeTup \}$ is a subset of $\{ \tup \mid \tup[U] \tmatch \rangeTup[U]\}$. Recall that the definition of tuple matching enforces that $\TM(\rangeTup, \tup) = \zeroK$ if $\tup \not\tmatch \rangeTup$. This implies for that any tuple matching $\TM$ it is the case that  $\sum_{\tup \tmatch \rangeTup} \TM(\rangeTup, \tup) = \sum_{\tup[U] \tmatch \rangeTup[U]} \TM(\rangeTup, \tup)$. Applying this equivalence we get:
% %
% \[
% =  \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup \wedge \forall \tup: t[U] \tmatch \rangeTup'[U]} \TM_R(\rangeTup', \tup)
% \]
% Recall that in any tuple matching for a possible world $D$ the sum of annotations assigned to each tuple $t$ is equal to
% $D(t)$: $\forall \tup \in \dataDomain^n: \sum_{\rangeTup \in \rangeDom^n} \TM(\rangeTup,\tup)=\rel(\tup)$. Thus, the above equation is equivalent to:
% \[
% =\sum_{\forall \tup: \exists \rangeTup': \rangeTup'[U]=\rangeTup \wedge t[U] \tmatch \rangeTup'[U]} \rel(\tup)
% \]
% Finally, we can substitute the definition of projection and again use the fact that tuple matchings assign $\zeroK$ to non-matching tuples to get:
% \[
% = \sum_{\forall \tup: \tup \tmatch \rangeTup} \projection_U(\rel)(\tup) = \projection_U(\rel)(\bgMarker{\tup[U]})
%   \]
% To summarize, we have shown that
% \[
%   \lbMarker{\left(\projection_U(\rangeRel)(\rangeTup)\right)}
%   \ordK \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup \wedge \forall \tup: t[U] \tmatch \rangeTup'[U]} \TM_R(\rangeTup', \tup)
% \]

% Note

% that, given a tuple matching $\TM_Q$ and range-annotated tuple $\rangeTup$, the set $\{ \tup \mid \tup \tmatch \rangeTup \}$ is a subset of $\{ \tup \mid \tup[U] \tmatch \rangeTup[U]\}$. Since for any tuple matching $\TM(\rangeTup, \tup) = \zeroK$ if $\tup \not\tmatch \rangeTup$ this implies $\sum_{\tup \tmatch \rangeTup} \TM(\rangeTup, \tup) = \sum_{\tup[U] \tmatch \rangeTup[U]} \TM(\rangeTup, \tup)$.
% By definition of projection and since (i) query evaluation in $\uaaK{\semK}$ is point-wise and (ii) semiring addition preserves the natural order we have:
% %
% \begin{align*}
%   \projection_U(\rangeRel)\lbMarker{(\rangeTup)} &=\sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}\rangeRel\lbMarker{(\rangeTup')} \ordK \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}  \sum_{\forall t \in \dataDomain^n}\TM_R(t,\rangeTup') \\
%                                           &= \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup}\sum_{\forall \tup: \tup \tmatch \rangeTup'}\TM_R(\rangeTup', \tup) \tag{\Cref{def:tuple-matching}}\\
%                                           &= \sum_{\forall \rangeTup': \rangeTup'[U]=\rangeTup \wedge \forall \tup: t[U] \tmatch \rangeTup'[U]} \TM_R(\rangeTup', \tup) \\
%                                             &=\sum_{\forall \tup: \exists \rangeTup': \rangeTup'[U]=\rangeTup \wedge t[U] \tmatch \rangeTup'[U]} \rel(\tup) = \sum_{\forall \tup: \tup \tmatch \rangeTup} \projection_U(\rel)(\tup)
% \end{align*}
% Thus, if we set $\TM_Q(\rangeTup,\tup) \defas \sum_{\forall \rangeTup', \tup: \rangeTup'[U]=\rangeTup \wedge t'[U]=t}\TM_{R}(\rangeTup', \tup')$, then %
%  $Q(\rangeRel)$ lower bounds $Q(\rel)$ through tuple matching $\TM$.  % $\TM(\rangeTup,\tup)=\sum_{\rangeTup'[U]=\rangeTup}\sum_{t'[U]=t}\TM_{R}(\rangeTup', \tup')$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\selection_\theta(\rangeRel)$}
By definition of selection and based on (i) and (ii) as in the proof of projection we have
%
$$\query(\rangeRel)\lbMarker{(\rangeTup)} = \lbMarker{\rangeRel(\rangeTup)} \multK \lbMarker{ \theta(\rangeTup)} \ordK \sum_{t \in \dataDomain^n} \TM_{\rel}(\rangeTup,t) \multK \lbMarker{ \theta(\rangeTup)}$$
%
Assume that for a tuple $\tup$ we have $t \not\tmatch \rangeTup$, then by \Cref{def:tuple-matching} it follows that $\TM_{rel}(\rangeTup, \tup) = \zeroK$. In this case we get $\lbMarker{\query(\rangeRel)(\rangeTup)} = \rangeRel(\rangeTup) \multK \zeroK = \zeroK$. Since $\zeroK \addK k = k$ for any $k \in \semK$, we get
$$\sum_{t \in \dataDomain^n} \TM_{\rel}(\rangeTup,t) \multK \lbMarker{ \theta(\rangeTup)} = \sum_{t \tmatch \rangeTup} \TM_{\rel}(\rangeTup,t) \multK \lbMarker{ \theta(\rangeTup)}$$
Note that based on \Cref{theo:expr-bound}, we have  $\lbMarker{\theta(\rangeTup)} \ordK \theta(\tup)$ since $\tup \tmatch \rangeTup$ from which follows that:
$\sum_{t \tmatch \rangeTup} \TM_{\rel}(\rangeTup,t) \multK \lbMarker{ \theta(\rangeTup)} \ordK \sum_{t \tmatch \rangeTup} \TM_{\rel}(\rangeTup,t) \multK \lbMarker{ \theta(\tup)}$.
It follows that $Q(\rangeRel)$ lower bounds $Q(\rel)$ through $\TM(\rangeTup,t) \defas \TM_{\rel}(\rangeTup,t) \multK \lbMarker{ \theta(t)}$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\rangeRel \times \rangeOf{S}$}
Based on the definition of cross product for $\semK$-relations, (i) from above, and that semiring multiplication preserves natural order we get
$\lbMarker{(\rangeRel \times \rangeOf{S})(\rangeTup)} = \lbMarker{\rangeRel(\rangeTup[\rel])}  \multK \lbMarker{\rangeOf{S}(\rangeTup[S])} \ordK \sum_{t \in \dataDomain^n}\TM_R(\rangeTup[R], \tup) \multK \sum_{t' \in \dataDomain^m}\TM_{S}(\rangeTup[S], \tup')$.
% By definition of join, $\lbMarker{(R(\rangeTup) \times P(\rangeTup'))}=\lbMarker{R(\rangeTup)} \otimes \lbMarker{R(\rangeTup)} \leq \sum_{t \in R}\TM(\rangeTup,\tup) \otimes \sum_{t \in R}TM_{P,\rangeOf{S}}(t',\rangeTup')$.
Thus, $\rangeRel \times \rangeOf{S}$ lower bounds $R \times S$ via $\TM_Q(\rangeTup, \tup) \defas \sum_{t \in \dataDomain^n}\TM_R(\rangeTup[R], \tup) \multK \sum_{t \in \dataDomain^m}\TM_{S}(\rangeTup[S], \tup)$.

%%%%%%%%%%%%%%%%%%%%
\proofpara{$\rangeRel \union \rangeOf{S}$}
Assume that $R$ and $S$ are n-ary relations.
Substituting the  definition of union and by (i) and (ii) from above we get:
$\lbMarker{(\rangeRel \union
  \rangeOf{S})(\rangeTup)}=\lbMarker{\rangeRel(\rangeTup)} \addK \lbMarker{\rangeOf{S}(\rangeTup)} \ordK \sum_{t \in \dataDomain^n}\TM_R(\rangeTup, \tup) \addK \sum_{\tup \in \dataDomain^n} \TM_{S}(\rangeTup, \tup)$. Thus, $\rangeRel \union \rangeOf{S}$ lower bounds $R \union S$ via $\TM_Q(\rangeTup, \tup) \defas \sum_{\tup \in \dataDomain^n}\TM_R(\rangeTup, \tup) \addK \sum_{\tup \in \dataDomain^n}\TM_{S}(\rangeTup, \tup)$.

%%%%%%%%%%%%%%%%%%%%
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{Lemma}
%\ubMarker{k} is subadditive and submultiplicative
%\begin{proof}
%Recall that $\pwAdd$ and $\pwMult$ are defined element-wise and that $\pwPossible(\pwe{k}) = \LubK(\pwe{k})$. Furthermore, $k_1 \ordK k_2$ iff $\exists k': k_1 \addK k' = k_2$. Consider an arbitrary $\pwe{k_1}, \pwe{k_2} \in \pwkDom$.  Let $k_{lub_1} = \LubK(\pwe{k_1})$ and $k_{lub_2} = \LubK(\pwe{k_2})$. Based on the definition of $\LubK$ this implies that for any $i$, $k_{lub_1} \geqK \pwe{k_1}[i]$ which in turn implies that $\pwe{k_1}[i] \addK k' = k_{glb_1}$ for some $k'$. Analog, we can find a $k''$ such that $\pwe{k_2}[i] \addK k'' = k_{glb_2}$.
%
%  \proofpara{Subadditivity}
%Let $k_{lub} = \LubK(\pwe{k_1} \pwAdd \pwe{k_2})$. We are going to prove that $k_{lub_1} \addK k_{lub_2}$ is an upper bound for $(\pwe{k_1} \pwAdd \pwe{k_2})$, i.e., that $\forall i \in \pwDom: k_{lub_1} \addK k_{lub_2} \geqK (\pwe{k_1} \pwAdd \pwe{k_2})[i]$. Since, $k_{lub}$ is the least upper bound this implies that $k_{lub_1} \addK k_{lub_2} \geqK k_{lub}$. Consider an arbitrary $i \in \pwDom$. Based on the discussion above we have:
%
%\noindent\resizebox{1\linewidth}{!}{
%  \begin{minipage}{1.05\linewidth}
%\begin{align*}
%&k_{lub_1} \addK k_{lub_2} = (\pwe{k_1}[i] \addK k') \addK (\pwe{k_2}[i] \addK k'')  \\
%&= (\pwe{k_1} \pwAdd \pwe{k_2})[i] \addK k' \addK k'' \geqK (\pwe{k_1} \pwAdd \pwe{k_2})[i]
%\end{align*}
%\end{minipage}
%}
%
%Thus, $k_{lub_1} \addK k_{lub_2}$ is an upper bound and since $k_{lub_1} = \pwPossible(\pwe{k_1})$ and $k_{lub_2} = \pwPossible(\pwe{k_2})$  it follows that $\pwPossible$ is subadditive:
%\begin{align*}
%\pwCertain(\pwe{k_1}) \addK \pwCertain(\pwe{k_2}) \ordK \pwCertain(\pwe{k_1} \pwAdd \pwe{k_2})
%\end{align*}
%
%\proofpara{Submultiplicativity}
%We use an analogous argument to prove submultiplicativity. Let $k_{lub} = \pwPossible(\pwe{k_1} \multK \pwe{k_2})$. We will prove that $k_{lub_1} \multK k_{lub_2}$ is an upper bound for $(\pwe{k_1} \pwMult \pwe{k_2})$ which implies submultiplicativity. Consider $i \in \pwDom$:
%
%\noindent\resizebox{1\linewidth}{!}{
%  \begin{minipage}{1.15\linewidth}
%\begin{align*}
%&(k_{lub_1} \multK k_{lub_2})
%= (\pwe{k_1}[i] \addK k') \multK (\pwe{k_2}[i] \addK k'')\\
%= &(\pwe{k_1}[i] \multK \pwe{k_2}[i]) \addK (\pwe{k_1}[i] \multK k'') \addK (k' \multK \pwe{k_2}[i])  \addK (k' \multK k'')\\
%\geqK &(\pwe{k_1} \pwMult \pwe{k_2})[i] \qedhere
%\end{align*}
%\end{minipage}
%}
%\end{proof}
%\end{Lemma}

%\begin{enumerate}
%\item Addition
%\[ (\lbMarker{k_1},k_1,\ubMarker{k_1}) \oplus (\lbMarker{k_2},k_2,\ubMarker{k_2}) = (\lbMarker{k_1} \oplus \lbMarker{k_2}, k_1 \oplus k_2, \ubMarker{k_1} \oplus \ubMarker{k_2})\]
%\item Multiplication
%\[ (\lbMarker{k_1},k_1,\ubMarker{k_1}) \otimes (\lbMarker{k_2},k_2,\ubMarker{k_2}) = (\lbMarker{k_1} \otimes \lbMarker{k_2}, k_1 \otimes k_2, \ubMarker{k_1} \otimes \ubMarker{k_2})\]
%\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Non-Monotone Queries}\label{sec:non-monotone-queries}
\BG{Should this be a section by itself?}
In this section we discuss non-monotone queries for which require extensions of $\semK$-relational query semantics. Specifically, we will develop a semantics for set difference and aggregation. % does not apply.
When defining these operators we will make use of an auxiliary operator that merges tuples with same \abbrBG values. The purpose of this operator is to ensure that a tuple in the \abbrBGW is encoded as a single tuple in the \abbrUAADB.

\BG{Explain briefly what its purpose is}

The main purpose for using the merge operator is to prevent tuples from over-reducing or over counting. And make sure we can still extract \abbrBGW from the non-monotone query result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[\abbrBG-Combiner]\label{def:t-combiner}
  Given a \abbrUAADB relation $\rangeRel$, the combine operator $\combine$ yields a \abbrUAADB relation by grouping tuples with the same $\abbrBGW$ attribute values:
  \begin{align*}
\combine(\rangeRel)(\rangeTup) &\defas
\begin{cases}
\sum_{\rangeTup': \bgMarker{\rangeTup}=\bgMarker{\rangeTup'}}\rangeRel(\rangeTup') & \text{if } \rangeTup=Comb(\rangeRel,\bgMarker{\rangeTup}) \\
0_k & \text{else}
\end{cases}
\end{align*}
% \sum_{\rangeTup': \bgMarker{\rangeTup} = \bgMarker{\rangeTup'}} \rangeRel{R}
%   \end{align*}
% $C(\rangeRel)=R_c$ is defined as
% $	\[ R_c(t) = \begin{cases}
% \sum_{BG(t)=BG(\rangeTup)}\rangeRel(\rangeTup) & \text{if } t=Comb(\rangeRel,BG(t)) \\
% 0_k & \text{else}
% \end{cases}
% \]
where $Comb(\rangeRel,t)$ defined below computes the mimimum bounding box for the ranges of all tuples from $\rangeRel$ that have the same \abbrBGW values as $t$ and are not annotated with $\zeroOf{\uaaK{\semK}}$. Let $a$ be an attribute from the schema of $\rangeRel$, then
\begin{align*}
Comb(\rangeRel,t).\lbMarker{a} &=\min_{\bgMarker{\rangeTup}=t \wedge \rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semK}}} \rangeTup.\lbMarker{a}\\
\bgMarker{Comb(\rangeRel,t).a} &=\bgMarker{\rangeTup.a}\\
Comb(\rangeRel,t).\ubMarker{a} &=\max_{\bgMarker{\rangeTup}=t \wedge \rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semK}}}\rangeTup.\ubMarker{a}
\end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The \abbrBG-combiner merges all tuples with the same \abbrBG attribute values are combined by merging their attribute ranges and summing up their annotations. For instance, consider a relation $\rangeRel$ with two tuples $(\uv{1}{2}{2}, \uv{1}{3}{5})$ and $(\uv{2}{2}{4}, \uv{3}{3}{4})$ which are annotated with $\ut{1}{2}{2}$ and $\ut{3}{3}{4}$, respectively. Applying \abbrBG-combiner to this relation the two tuples are combined (they have the same \abbrBGW values) into a tuple $(\uv{1}{2}{4}, \uv{1}{3}{5})$ annotated with $\ut{1+3}{2+3}{2+4} = \ut{4}{5}{6}$. Before moving on and discussing semantics for set difference and aggrgeation we first establish that the \abbrBG-combiner preserves bounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Lemma}\label{def:combine preserves bounds}
Let $\rangeRel$ by a $\uaaK{\semK}$-relation that bounds an n-nary $\semK$-relation $\rel$. Then $\combine(\rangeRel)$ bounds $\rel$.
\end{Lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Consider a tuple $\tup \in \dataDomain^n$ and let $supp(\rangeRel, \tup)$ denote the set $\{ \rangeTup \mid \rangeRel(\rangeTup) \neq \zeroOf{\uaaK{\semK}} \wedge \bgMarker{\rangeTup} = \tup \}$. Observe that $Comb(\rangeRel, \tup)$ merges the range annotations $supp(\rangeRel, \tup)$. Let $\rangeTup$ be the result of $Comb(\rangeRel, \tup)$. Then
$$\lbMarker{\combine(\rangeRel)(\rangeTup)}=\sum_{\bgMarker{\rangeTup}=\bgMarker{\rangeTup'}}\rangeRel(\rangeTup') \ordK \sum_{\bgMarker{\rangeTup}=\bgMarker{\rangeTup'}} \sum_{\tup \in \dataDomain^n}\TM(\rangeTup,\tup)$$
Thus, $\combine(\rangeRel)$
bounds $\rel$ through $\TM'(\rangeTup, \tup)=\sum_{\bgMarker{\rangeTup}=\bgMarker{\rangeTup'}}\sum_{\tup \in \dataDomain^n}\TM(\rangeTup', \tup)$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Set Difference}
\label{sec:set-difference}

\BG{In case we have trouble fixing our space problem, then I think in worst case we can prioritize aggregation over set difference.}

Geerts~\cite{Geerts:2010bz} did extend $\semK$-relations to support set difference through m-semirings which are semirings equipped with a monus operation that is used to define difference. The monus operation $\monK$ is defined based on the natural order of semirings as $k_1 \monK k_2 = k_3$ where $k_3$ is the smallest element from $\semK$ \st $k_2 \addK k_3 \geqK k_1$. For instance, the monus of semiring $\semN$ is truncating subtraction: $k_1 \monOf{\semN} k_2 = max(0, k_1 - k_2)$. The
monus construction for a semiring $\semK$ can be lifted through point-wise application to  $\semkq$ since $\semkq$-semirings are direct products. We get $\ut{k_1}{k_2}{k_3} \monOf{\uaaK{\semK}} \ut{l_1}{l_2}{l_3} = \ut{k_1 \monK l_1}{k_2 \monK l_2}{k_3 \monK l_3}$. However, the result of $k \monOf{\semkq} k'$ for $k, k' \in \uaaK{\semK}$ is not necessarily in $\uaaK{\semK}$, i.e., this semantics for set difference does not preserve bounds even if we disallow range-annotated values.
For instance, consider an incomplete $\semN$-relations with two possible worlds: $\db_1 = \{ R(1) \mapsto 2, S(2) \mapsto 1\}$ and $\db_2 = \{ R(1) \mapsto 1, R(2) \mapsto 1,  S(1) \mapsto 3\}$. Here we use $\tup \mapsto k$ to denote that tuple $\tup$ is annotated with $k$. Without using range-annotations, i.e., we can bound these worlds using $\uaaK{\semN}$-database $\rangeDB_1$:
$\rangeDB \defas \{ \rangeRel(1) \mapsto (1,2,2), \rangeRel(2) \mapsto (0,0,1), \rangeOf{S}(1) \mapsto (0,0,3), \rangeOf{S}(2) \mapsto (0,1,1) \}$. Consider the query $\rel \difference S$. Applying the definition of set difference from Geerts~\cite{Geerts:2010bz} which is $(\rel - S)(\tup) \defas \rel(\tup) \monK S(\tup)$, for tuple $\rangeTup \defas (1)$  we get the annotation  $\rangeRel(\rangeTup) \monOf{\uaaK{\semN}} \rangeOf{S}(\rangeTup) = (1,2,2) \monOf{\uaaK{\semN}} (0,0,3) = (\max(1 - 0,0), \max(2 - 0,0), \max(2 - 3,0)  = (1,2,0)$. However,  $\lbMarker{(1,2,0)} = 1$ is not a lower bound on the certain annotation of $\rangeTup$ , since $\rangeTup$ is not in the result of the query in $db_2$ ($max(1-3,0) = 0$). This failure of the point-wise semantics to preserve bounds is not all uprising if we consider the following  observation from~\cite{GL17}: because of the negation in set difference, a lower bound on certain answers can turns into  an upper bound. To calculate an lower (upper) bound for the result one has to combine a lower bound for the LHS input of the set difference with an upper bound of the RHS. Thus, we can define $(\rangeRel \difference \rangeOf{S})(\rangeTup) \defas
\ut
{\lbMarker{\rangeRel(\rangeTup)} \monK \ubMarker{\rangeOf{S}({\rangeTup})}}
{\bgMarker{\rangeRel(\rangeTup)} \monK \bgMarker{\rangeOf{S}({\rangeTup})}}
{\ubMarker{\rangeRel(\rangeTup)} \monK \lbMarker{\rangeOf{S}({\rangeTup})}
}
$
to get a result that preserves bounds. For instance, for $\rangeTup \defas (1)$ we get $(\max(1 - 3,0), \max(2 - 0,0), \max(2 - 0,0)) = (0,2,2)$.

This semantics is however still not sufficient if we consider range-annotated values. For instance, consider the following $\uaaK{\semN}$-database $\rangeDB_2$ that also bounds our example incomplete  $\semN$-database :
$\{ \rangeRel(1) \mapsto (1,1,1), \rangeRel(\uv{1}{1}{2}) \mapsto (1,1,1), \rangeOf{S}(\uv{1}{1}{2}) \mapsto (1,1,3) \}$.
Observe that tuple $(1))$ from the \abbrBGW ($\db_1$) is encoded as two tuples in $\rangeDB_2$. To calculate the annotation of this tuple in the \abbrBGW we need to sum up the annotations of all such tuples in the LHS and RHS. To calculate lower bound annotations, we need to also use the sum of annotations of all tuples representing the tuple and then compute the monus of this sum with the sum of all annotations of tuples from the RHS that could be equal to this tuple in some world. Two range-annotated tuples may represent the same tuple in some world if all of their attribute values overlap.
Conversely, to calculate an upper bound it is sufficient to use annotations of RHS tuples if both tuples are certain (they are the same in every possible world).
We use the \abbrBG-combiner operator define above to merge tuples with the same \abbrBG values and then apply the monus using the appropriate set of tuples from the RHS.

% For instance, $(\uv{1}{1}{2})$ me encode tuple $(2)$ in some world and thus its annotation has to be taken into account
% Based on this example it is obvious that we need to


% That is, for set difference a tuple is only certain in the result if it is certain in the left input and does not belong to the right input in any possible world. Thus, to determine whether a tuple is part of the lower bound on the query result we need to "subtract" from the annotation of the tuple in the left input the sum of the upper bound annotations for all tuples that possibly overlap with this tuple. For instance, consider a query $\rel \difference S$ over database instance $\rel = \{ (\uv{}{}{} ) \}$ and $S = \{ (\uv{}{}{}), (\uv{}{}{})\}$
% We define set difference using the \abbrBG-combiner to avoid subtracting one tuple multiple times.



%For instance, consider two possible worlds for relations $\rel$ and $S$: $\db_1 = \{ R(1) \mapsto 2, S(1) \mapsto 1\}$ and % $\db_2 = \{ R(1) \mapsto 1, R(2) \mapsto 1,  S(2) \mapsto 3\}$. One possible \abbrUAADB that bounds these two possible worlds is $\rangeDB \defas \{ \rangeRel(1) \mapsto (1,1,1), \rangeRel(\uv{1}{1}{2}) \mapsto (1,1,1), \rangeOf{S}(\uv{1}{1}{2}) \mapsto (0,1,3) \}$.
% Consider the query $\rel \difference S$.
% Note that tuple $(1)$ occurs once in the query result in $\db_1$ but has multiplicity in the query result in $\db_2$ since in this tuple occurs with multiplicity $3$ in $S$ in $\db_2$. Thus, the certain annotation of the tuple in $\rangeRel \monOf{\semN} \rangeOf{S}$ should be $0$. However, applying the definition of set difference naively we immediately face the problem that the monus is applied based on equality of range-annotated tuples, e.g., for $\rangeTup \defas (\uv{1}{1}{2})$ we get $(\rangeRel - \rangeOf{S})(\rangeTup) = \rangeRel(\rangeTup) \monOf{\uaaK{\semN}} \rangeOf{S}(\rangeTup) = (1,1,1) \monOf{\uaaK{\semN}} (0,0,0) = (1,1,1)$. However, as stated above the certain annotation of this tuple should be $0$. We address this issue by first normalizing both inputs of the difference using the \abbrDB-combiner to ensure that there are no two tuples with the same \abbrBG values in the inputs and by subtracting







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{Definition}[Set Difference]\label{def:set-diff-semantics}
Let $\rangeTup$ and $\rangeTup'$ be n-ary range-annotated tuples with schema $(a_1, \ldots, a_n)$.
   We define a predicate $\rangeTup \equiv \rangeTup'$ that evaluates to true iff $\rangeTup=\rangeTup'$ and both $\rangeTup$ and $\rangeTup'$ are certain and a predicate $\rangeTup \matches \rangeTup'$ that evaluates to true iff $\forall i \in \{1, \ldots, n\}: \lbMarker{\rangeTup.a_i} \ordK \lbMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i} \vee \lbMarker{\rangeTup.a_1} \ordK \ubMarker{\rangeTup'.a_i} \ordK \ubMarker{\rangeTup.a_i}$. Using these predicates we define set difference as shown below.
   \begin{align*}
     \lbMarker{(\rangeRel_1 - \rangeRel_2)(\rangeTup)}  & \defas \lbMarker{\combine(\rangeRel_1)(\rangeTup)} \monK \sum_{\rangeTup \matches \rangeTup'} \ubMarker{\rangeRel_2(\rangeTup')} \\
     \bgMarker{(\rangeRel_1 - \rangeRel_2)(\rangeTup)} & \defas \bgMarker{\combine(\rangeRel_1)(\rangeTup)} \monK \sum_{\bgOf{\rangeTup} = \bgOf{\rangeTup'}} \bgMarker{\rangeRel_2(\rangeTup')} \\
     \ubMarker{(\rangeRel_1 - \rangeRel_2)(\rangeTup)}      & \defas \ubMarker{\combine(\rangeRel_1)(\rangeTup)} \monK \sum_{\rangeTup \equiv \rangeTup'} \lbMarker{\rangeRel_2(\rangeTup')}
   \end{align*}
 \end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Bound Preservation}
\label{sec:bound-preservation-diff}

We now demonstrate that the semantics we have defined for set difference preserves bounds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Set Difference Preserves Bounds]\label{theo:set-difference-prese}
Let $\query \defas R - S$, $\rel$ and $S$ be incomplete $\semK$-relations, and $\rangeRel$ and $\rangeOf{S}$ be $\uaaK{\semK}$-relations that bound $\rel$ and $S$. Then $\query(\rangeRel,\rangeOf{S})$ bounds $\query(\rel,S)$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}

\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{uaa-aggregation.tex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation}
\label{sec:implementation}
In this section we discuss about the implementation of our $\abbrAUDB$ model as a middleware on conventional database systems as part of GProM. We interpolate the model as conventional database relations and use query rewriting to propagate annotations while processing the query.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relational encoding of \abbrAUDB}

\BG{Do we put labeling schemes here, or what is the purpose of this? Or is the the relational encoding of $\uaaK{\semK}$-semirings.}
For a $\uaaK{\semK}$ tuple $\rangeTup$ with row annotation $\rangeRel(\rangeTup)=(\lbMarker{k},\bgMarker{k},\lbMarker{k})$. We encode each range annotated attribute as three attributes in the database and tuple level annotation as three attributes too. For range annotated attribute $a$, our interpolation encodes the upper-bound, selected-guess and lower-bound parts into three relational attributes $\lbatt{a}$, $a$ and $\ubatt{a}$ respectively. Tuple level annotations are defined as $\rlb$, $\ratt$ and $\rub$ respectively to the certain, selected-guess and possible semiring values. The tuple is not exist in the database if $\ubMarker{\rangeRel(\rangeTup)}=0$.
\begin{Example}
	For $\abbrAUDB$ relation $\rangeRel(a,b)$, corresponding backend database will interpolate as conventional relation with schema$R(a,b,\ubatt{a},\lbatt{a},\ubatt{b},\lbatt{b},\rlb,\ratt,\rub)$.
\end{Example}

\BG{\textbullet I think you can just us $\lbMarker{a}$ for attribute $a$ and so on. For tuple-level we could do $\lbMarker{row}$. I think there is no problem with reusing the bounds since it will be clear when we mean the attribute and when we mean the bound. This way the reader does not have to learn yet another set of symbols. In any case you should introduce macros for that \texttt{\textbackslash{}lbatt\{a\}, \textbackslash{}ubatt\{a\}, \textbackslash{} arlb} and then do search and replace once %
 \textbullet Instead of using the SQL-like \texttt{case}, it is better to use the expression syntax from \Cref{sec:expression}. We have \texttt{\textbackslash{}ifte\{\}\{\}\{\}} for conditional expressions
 \textbullet Let's use $a \leftarrow e$ or $e \to a$ to denote renaming in projection
 \textbullet We can replace join with cross product which is simpler
 \textbullet Let us use \abbrBG instead of ``bst'' to be consistent with the remainder of the paper
 \textbullet For each operator also state what the input is, e.g., Join $R \times S$
 \textbullet For aggregation we need to also explain how the other aggregation functions work
 \textbullet Instead of $R$ and $P$ let us us the more idiomatic $R$ and $S$
 \textbullet The name ``relational database interpolation'' is misleading (implied approximation). Let's use something else, e.g., encoding
 \textbullet The macro for rewriting should probably not be the same as the one for expression evaluation
 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rewriting}\label{sec:rewrite-rules}
We use $\schemaOf(R)$ to denote the schema of input relation R and use $A$,$B$ to denote the set of non-annotation attributes for relation $R$ and $S$ to simplify the notation instead of enumerating all attributes with same rewrite. We use $\renameto$ to rename the LFS to the RHS. Assume the input rewritten schema is a valid \abbrAUDB that correctly interpolated in the relation database.
$$\rewrUAA{R}(A, \ubatt{A} , \lbatt{A}, \rlb,\ratt,\rub)$$
$$\rewrUAA{P}(B, \ubatt{B}, \ubatt{B}, \rlb,\ratt,\rub)$$

\BG{Add some introduction here (purpose, general approach, what to expect to take away from this section}
\BG{Explain how the rewriting generates three expressions for every subquery in some cases and how they are merged into a single query}
\BG{Some of the rules are missing operators, e.g., for the selection there should be a projection to calculate the annotation columns?}
\BG{Need to have notation for an expression rewrite that implements the semantics from \Cref{sec:expression}}
\BG{I think instead of the ternary operator notation for conditionals we should rather use the notation we already defined in \Cref{sec:expression}.}
\BG{Explain the schema of the rewritten version, e.g., what are the names of attributes storing attribute ranges and tuple-level annotations?}
\BG{For aggregation should we list the different variants for different aggregation functions or can we maybe reuse something from }
\BG{Add a notation for the application of the rewriting instead of using $=$ with the original query on the LHS and the rewritten version on the RHS}
\begin{enumerate}
\item Selection
\[ CET \defas (\ifte{\lbMarker{\theta}}{1}{0})*\rlb \leftarrow \rlb \]
\[ SG \defas (\ifte{\theta}{1}{0})*\ratt \renameto \ratt\]
\[ \rewrUAA{\selection_{\theta}(R)}=\projection_{A,\ubatt{A}, \lbatt{A}, CET,SG,\rub}(\selection_{\ubMarker{\theta}}(\rewrUAA{R})) \]

\item Projection
\[ \rewrUAA{\projection_{U}(R)}=\projection_{U,\ubatt{U},\lbatt{U},\rlb,\ratt,\rub}(\rewrUAA{R}) \]

\item Cross Product
\[ CET \defas R.\rlb*S.\rlb \renameto \rlb \]
\[ SG \defas R.\ratt*S.\ratt \renameto \ratt \]
\[ POS \defas R.\rub*S.\rub \renameto \rub \]
\[ \rewrUAA{R \times S} \defas \projection_{A,B,\ubatt{A},\lbatt{A},\ubatt{B},\lbatt{B},CET,SG,POS}(\rewrUAA{R} \times \rewrUAA{P})\]

\item Join
\[ CET \defas (\ifte{\lbMarker{\theta}}{1}{0})*R.\rlb*S.\rlb \renameto \rlb \]
\[ SG \defas (\ifte{\theta}{1}{0})*R.\ratt*S.\ratt \renameto \ratt \]
\[ POS \defas R.\rub*S.\rub \renameto \rub \]
\[ \rewrUAA{R \join_{\theta} S} \defas \projection_{A,B,\ubatt{A},\lbatt{A},\ubatt{B},\lbatt{B},CET,SG,POS}(\rewrUAA{R} \join_{\ubMarker{\theta}} \rewrUAA{P})\]

\item Set Difference
\[ Join \defas \combine(\rewrUAA{R}) \join_{\ubatt{A} \geq \lbatt{B} \wedge \ubatt{B} \geq \lbatt{A}} \rewrUAA{S} \]
\[ \theta \defas (\ubatt{A} = \lbatt{A}=\lbatt{B}=\lbatt{B}) \]
\[ CETV \defas (\ifte{\theta}{R.\rlb-S.\rub}{0})\]
\[ CET \defas \ifte{CETV > 0}{CETV}{0} \renameto \rlb \]
\[ SG = R.\ratt-S.\ratt \]
\[ POSV \defas \ifte{\theta}{R.\rub-S.\rlb}{R.\rub}) \]
\[ POS \defas \ifte{POSV > 0}{POSV}{0} \renameto \rub \]
\[ \rewrUAA{R \difference S} = \selection_{\rub>0}(\projection_{A,\ubatt{A},CET,SG,POS}(Join)) \]

\item Aggregation
\[ AggrF1 \defas max(\ubatt{g}) \renameto \ubatt{g},min(\lbatt{g}) \renameto \lbatt{g}\]
\[ Aggr1 \defas \aggregation{g}{AggrF1}(\rewrUAA{R}) \]
\[ \theta \defas R.\ubatt{g} \geq R'.\lbatt{g} \wedge R'.\ubatt{g} \geq R.\lbatt{g} \]
\[ Join \defas Aggr1 \join_{\theta} (\rewrUAA{R} \renameto R')\]
\[ lba \defas \ifte{\lbatt{a} < 0}{a*\rub}{0} \renameto \lbatt{a} \]
\[ bga \defas \ifte{R.g=R'.g}{a*\ratt}{0} \renameto a \]
\[ uba \defas \ifte{\ubatt{a}>0}{a*\rub}{0} \renameto \ubatt{a} \]
\begin{align*}
CET \defas & \ifte{R.\ubatt{g}=R'.\ubatt{g}=R.\lbatt{g}=R'.\lbatt{g}}{1}{0} \\
	& \renameto \rlb
\end{align*}
\[ SG \defas \ifte{R.g=R'.g}{1}{0} \renameto \ratt \]
\[ Proj \defas \projection_{R.g, R.\ubatt{g} , R.\lbatt{g},lba,bga,uba,CET,SG,R'.\rub}(Join) \]
\begin{align*}
	aAggF2 \defas
		& sum(a),sum(\ubatt{a}) \renameto \ubatt{sum(a)}, \\
		& sum(\lbatt{a}) \renameto \lbatt{sum(a)}, \\
		& max(\rlb) \renameto \rlb, \\
		& max(\ratt) \renameto \ratt, \\
		& sum(\rub) \renameto \rub
\end{align*}
\[ \rewrUAA{\aggregation{g}{sum(a)}(R)}  \defas \aggregation{g,\ubatt{g},\lbatt{g}}{aAggF2}(Proj) \]

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Optimizations for Joins}

\BG{Think about whether this part should live here or better elsewhere, or even in its own section.}
\BG{The notation should be adapted to fit the one from \Cref{sec:rewrite-rules}}.
In practice, the number of join results in rewritten query can be significantly larger than the number of best guess results due to the fact that joining ranged tuple may create a cross product of possible joining results within the overlapping range. In the worst case, a rewritten conditioned join can behave as cross product. Example shows how an overlapping range creates a cross product join on a simple equality join condition.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
	Figure~\ref{table:join_no_op} shows an example of joining two tables $R \join_{A=C} S$. In best guess world the result set only contains one tuple. However, if we want to enumerate all possible results, we need to consider all possible combinations. Four tuples are in the result which makes the join become a cross product.
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
	\centering

	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
		\textbf{A}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{1}{1}{2}$ & \ut{2}{2}{3}\\
%				\cline{1-3}
		$\uv{1}{2}{2}$ & \ut{1}{1}{2}\\
%				\cline{1-1}
	\end{tabular}
	\caption{Table R}
	\label{table:}
	\end{subtable}
	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
				% \cline{1-1}
		\textbf{C}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{1}{3}{3}$ & \ut{1}{1}{1}\\
%				\cline{1-3}
		$\uv{1}{2}{2}$ & \ut{1}{2}{2}\\
				% \cline{1-1}
	\end{tabular}
	\caption{Table S}
	\label{table:}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|cc}
				% \cline{1-2}
		\textbf{A}  & \textbf{C}  & \underline{\semqN} \\
		\cline{1-2}
		$\uv{1}{2}{2}$ & $\uv{1}{2}{2}$ & \ut{1}{2}{4}\\
				% \cline{1-2}
	\end{tabular}
	\caption{$BG(R \join_{A=C} S)$}
	\label{table:}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|cc}
				% \cline{1-2}
		\textbf{A}  & \textbf{C}  & \underline{\semqN} \\
		\cline{1-2}
		$\uv{1}{1}{2}$ & $\uv{1}{3}{3}$ & \ut{0}{0}{3}\\
		$\uv{1}{1}{2}$ & $\uv{1}{2}{2}$ & \ut{0}{0}{6}\\
		$\uv{1}{2}{2}$ & $\uv{1}{3}{3}$ & \ut{0}{0}{2}\\
		$\uv{1}{2}{2}$ & $\uv{1}{2}{2}$ & \ut{1}{2}{4}\\
				% \cline{1-2}
	\end{tabular}
	\caption{$POS(R \join_{A=C} S)$}
	\label{table:}
	\end{subtable}

	\caption{Join rewriting without optimization}
	\label{table:join_no_op}
\end{figure}

In order to reduce the running time, we introduce an optimized version of the rewrite rule for conditioned join operator. A "splice" ($SP$) process will create two different modified version of the input relation. One ($BG^{SP}(R)$) only contains best guess tuples where all attribute uncertainty are moved to tuple level. The other version ($POS^{SP}(R)$) contains all possible tuples by setting all certain and best guess annotations to zero. Two operator is defined as below:
$$ BG^{SP}(R)=\projection_{(a[\lbMarker{a}],a,a[\ubMarker{a}],(\ubMarker{a}>\lbMarker{a})?0:CET[CET], BST, BST[POS])}(\selection_{bg>0}(R)) $$
$$ POS^{SP}(R)=\projection_{(\lbMarker{a},a,\ubMarker{a},0[CET], 0[BST], POS)}(R) $$
We join the $POS^{SP}$ and $BG^{SP}$ separately and the union the result. Since $POS^{SP}(R) \join POS^{SP}(S)$ can potentially create number of tuples close to cross product. We add merge operator to limit the number of possible tuples before join.
\begin{align*}
	[[R \join_{\theta} S]]^{Op}=(BG^{SP}(R) \join_{\theta} BG^{SP}(S)) \union
	\\ [[M(POS^{SP}(R)) \join_{\theta} M(POS^{SP}(S))]]
\end{align*}

\begin{Example}
	Figure~\ref{table:join_with_op} shows the result of joining two tables from figure ~\ref{table:join_no_op} $R \join_{A=C} S$ with optimization. By sacrificing accuracy, the number of result tuples can be reduced by limiting the number of output tuples in the merge operator.
\end{Example}
\begin{figure}[ht]
	\centering

	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
%				\cline{1-1}
		\textbf{A}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{1}{1}{1}$ & \ut{0}{2}{2}\\
%				\cline{1-3}
		$\uv{2}{2}{2}$ & \ut{0}{1}{1}\\
%				\cline{1-1}
	\end{tabular}
	\caption{$BG^{SP}(R)$}
	\label{table:}
	\end{subtable}
	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
%				\cline{1-1}
		\textbf{C}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{3}{3}{3}$ & \ut{0}{1}{1}\\
%				\cline{1-3}
		$\uv{2}{2}{2}$ & \ut{0}{2}{2}\\
%				\cline{1-1}
	\end{tabular}
	\caption{$BG^{SP}(S)$}
	\label{table:}
	\end{subtable}

	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
%				\cline{1-1}
		\textbf{A}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{1}{1}{2}$ & \ut{0}{0}{3}\\
%				\cline{1-3}
		$\uv{1}{2}{2}$ & \ut{0}{0}{2}\\
%				\cline{1-1}
	\end{tabular}
	\caption{$POS^{SP}(R)$}
	\label{table:}
	\end{subtable}
	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
%				\cline{1-1}
		\textbf{C}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{1}{3}{3}$ & \ut{0}{0}{1}\\
%				\cline{1-3}
		$\uv{1}{2}{2}$ & \ut{0}{0}{2}\\
%				\cline{1-1}
	\end{tabular}
	\caption{$POS^{SP}(S)$}
	\label{table:}
	\end{subtable}

	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
				% \cline{1-1}
		\textbf{A}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{1}{1}{2}$ & \ut{0}{0}{5}\\
%				\cline{1-3}
				% \cline{1-1}
	\end{tabular}
	\caption{$M(POS^{SP}(R))$}
	\label{table:}
	\end{subtable}
	\begin{subtable}{0.4\linewidth}
	\centering
	\begin{tabular}{ cc}
				% \cline{1-1}
		\textbf{C}  & \underline{\semqN} \\
		\cline{1-1}
		$\uv{1}{2}{3}$ & \ut{0}{0}{3}\\
%				\cline{1-3}
				% \cline{1-1}
	\end{tabular}
	\caption{$M(POS^{SP}(S))$}
	\label{table:}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|cc}
				% \cline{1-2}
		\textbf{A}  & \textbf{C}  & \underline{\semqN} \\
		\cline{1-2}
		$\uv{2}{2}{2}$ & $\uv{2}{2}{2}$ & \ut{0}{2}{2}\\
		$\uv{1}{1}{2}$ & $\uv{1}{2}{3}$ & \ut{0}{0}{15}\\
				% \cline{1-2}
	\end{tabular}
	\caption{$[[R \join_{A=C} S]]^{Op}$}
	\label{table:}
	\end{subtable}

	\caption{Join rewriting without optimization}
	\label{table:join_with_op}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-rels-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{UAA-Databases}\label{sec:uaa-model}
We extend UA-relations model into UAA-relations (Uncertainty Attribute Annotated relations) by annotating each attribute in a tuple with a boolean value, define attribute determinism as a mapping between an attribute A from a tuple t and a binary(boolean) value: $\{F,T\}$ where label $F$ as uncertain and $T$ as certain.

\begin{Definition}[UAA annotations]
	Let $\uaK{\semK}$ be a UA-semiring, $B$ be a boolean semiring. A UAA-tuple $t$ in an UAA-relation $R$ have annotation: $R(t)=\{B^{arity(t)}, \uaK{\semK}\}$
\end{Definition}
Where $\uaK{\semK}$ annotates the row determinism $detR(t)=\uaK{\semK}$. The boolean vector annotates the attribute determinism $\forall_{0 \leq i<arth(t)} detA(A[i])=B[i]$.
Each boolean semiring annotates the uncertainty of the attribute in correspond location. \\
% $val(v^b)=v \mid v^b \in \mathcal{U}^+$.\\
%  $det(v^b)=b \mid v^b \in \mathcal{U}^+$.\\
%  $strip(t)=<val(v_1^{b_1}), \ldots, val(v_n^{b_n})> \mid t=<v_1^{b_1}, \ldots, v_n^{b_n}>$.\\
The annotation indicates the determinism of corresponding value in $\mathcal{U}$: \\$attrD(Q,t,A,I)=det(v^b) \mid t.A=v^b$.\\
Let $[[e]]$ denote the evaluation of a expression $e$ over values: $<v_1,v_2, \ldots, v_n> \in  \mathcal{U}^+$ or $<v_1,v_2, \ldots, v_n> \in  \mathcal{U}$. Assuming attribute values are annotated using semiring $(\{T,F\}, F, T, \vee, \wedge)$ and evaluation output of boolean expression over $\mathcal{U}^+$ to be in $\{T^T,T^F,F^T,F^F\}$, define each expression operator over $\mathcal{U}^+$ as following:
\begin{enumerate}
	\item arithmetic operators\\
	\[[[v_1^{b_1} \pm v_2^{b_2}]]=[[v_1 \pm v_2]]^{[[b_1 \wedge b_2]]}\]
	\[
	[[v_1^{b_1} \times v_2^{b_2}]]=\begin{cases}
	0^T, & \text{if} \; v_1=0^T \vee v_2=0^T\\
    [[v_1 \times v_2]]^{[[b_1 \wedge b_2]]}, & \text{else}
	\end{cases}
  \] \\
    \item comparison operators\\
	\[[[v_1^{b_1} = v_2^{b_2}]]=[[v_1 = v_2]]^{[[b_1 \wedge b_2]]}\]
	\[[[v_1^{b_1} > v_2^{b_2}]]=[[v_1 > v_2]]^{[[b_1 \wedge b_2]]}\]
	\[[[v_1^{b_1} < v_2^{b_2}]]=[[v_1 < v_2]]^{[[b_1 \wedge b_2]]}\]
	\item boolean operators\\
	\[[[\neg v_1^{b_1}]]=[[\neg v_1]]^{b_1}\]
	\[[[v_1^{b_1} \wedge v_2^{b_2}]]=[[v_1 \wedge v_2]]^{[[(\neg v_1 \wedge b_1) \vee (\neg v_2 \wedge b_2) \vee (b_1 \wedge b_2)]]}\]
	\[[[v_1^{b_1} \vee v_2^{b_2}]]=[[v_1 \vee v_2]]^{[[(v_1 \wedge b_1) \vee (v_2 \wedge b_2) \vee (b_1 \wedge b_2)]]}\]
	\item conditional operators\\
	\begin{align*}
		[[\text{if } v_1^{b_1} \text{ then } & v_2^{b_2} \text{ else } v_3^{b_3}]] \\
		& =[[\text{if } v_1 \text{ then } v_2 \text{ else } v_3]]^{[[(v_1 \wedge b_1 \wedge b_2) \vee (\neg v_1 \wedge b_1 \wedge b_3)]]}
	\end{align*}
	\item string operators\\
	\[[[v_1^{b_1} || v_2^{b_2}]]=[[v_1 || v_2]]^{[[b_1 \wedge b_2]]}\]
\end{enumerate}
%Define expression determinism to be: \\
%$exprD(t,E)=det([[E(t)]])$.\\

For the expression definitions above, string operator and most of the mathematical operators are straight forward in the sense that one uncertain value will make the result uncertain, with minor exceptions such as multiplication with $0^T$ resulting in $0^T$ independent of the other input value. In some boolean expressions, the output annotations will be depend on the value and the annotation of the input. Example \ref{example:expr-rule} shows briefly how the rules work in a database instance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{Theorem}[Expression processing in $\mathcal{U}$ is embedded in $\mathcal{U^+}$]
%Define transfer function $tr(v)=v^T \mid v \in \mathcal{U} \wedge v^T \in \mathcal{U^+}$. Define function $tr_{all}$ that apply $tr()$ to all values in expression $E$. then for any expression $E$, $tr_{all}([[E]])=[[tr_{all}(E)]]$.
%\label{theo:expr-emb}
%\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{proof}
%We prove this theorem using induction over the structure of a expression.
%
%	\proofpara{Base case} When $E$ is a single value, by assumption we know $[[v]]^T=[[v^T]]=v^T$.\\
%
%	\proofpara{Induction cases} for each operator, we have
%	\begin{align*}
%		& [[v_1^T \pm v_2^T]] = v_1^T \pm v_2^T=(v_1 \pm v_2)^{T\wedge T}=[[(v_1 \pm v_2)]]^T\\
%		& [[v_1^T \times v_2^T]]=(v_1 \times v_2)^{T \times T} = [[v_1 \times v_2]]^T \\
%		& [[v_1^T (=,>,<) v_2^T]]=(v_1 (=,>,<) v_2)^{T} = [[v_1 (=,>,<) v_2]]^T \\
%		&
%		\begin{aligned}
%    	[[v_1^T \wedge v_2^T]]= & (v_1 \wedge v_2)^{((v_1 \wedge v_2) \wedge T)\vee((v_1 \wedge v_2) \wedge T)\vee(T \wedge T)} \\
%    	 = & (v_1 \wedge v_2)^T = [[v_1 \wedge v_2]]^T
%    	\end{aligned} \\
%    	&
%    	\begin{aligned}
%    	[[v_1^T \vee v_2^T]]= & (v_1 \vee v_2)^{((v_1 \vee v_2) \wedge T)\vee((v_1 \vee v_2) \wedge T)\vee(T \wedge T)} \\
%    	= & (v_1 \vee v_2)^T = [[v_1 \vee v_2]]^T
%    	\end{aligned} \\
%    	&
%    	\begin{aligned}
%    		[[\text{if } v_1^T & \text{ then } v_2^T \text{ else } v_3^T]] \\
%    		&=(\text{if } v_1 \text{ then } v_2 \text{ else } v_3)^{(v_1 \wedge T \wedge T) \vee (\neg v_1 \wedge T \wedge T)} \\
%    		&=(\text{if } v_1 \text{ then } v_2 \text{ else } v_3)^T = [[\text{if } v_1 \text{ then } v_2 \text{ else } v_3]]^T\\
%    	\end{aligned}
%	\end{align*}
%   	Thus by induction, for any operator, $T$ annotated input will result $T$ annotated output with value same as non-annotated operator result. So for any expression $E$, normal expression computation is embedded in our annotated model.
%\end{proof}

\begin{Example}
	Table \ref{table:4.attr} shows an example instance of executing query
	$$Q=\projection_{name,color||\textvisiblespace^T||category}(food)$$.
	For the tuple $apple^T$, The value $red^T||\textvisiblespace^T$ is computed according to the rule return $red\textvisiblespace^{T \wedge T=T}$ and further combined with $fruit^T$ return the final tuple. For the tuple $carrot^T$, the first concatenation result is formed by $red^F||\textvisiblespace^T=red\textvisiblespace^{T \wedge F=F}$ and second concatenation produces $red\textvisiblespace vegetable^{F \wedge T=F}$ as the tuple result. The last tuple follows identical procedure with $F \wedge F=F$ for the last concatenation.
\label{example:expr-rule}
\end{Example}

\begin{figure}[t]
	\centering
	\begin{subtable}{\linewidth}
	\centering
	\caption{Tainted input table: \textsf{food}}
	\begin{tabular}{ |c|c|c|}
				\cline{1-3}
		\textbf{name}  & \textbf{color}  & \textbf{category}   \\
		\cline{1-3}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} \\
%				\cline{1-3}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} \\
%				\cline{1-3}
		\cMarker{tomato} & \uMarker{red} & \uMarker{fruit} \\
				\cline{1-3}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Query result}
	\begin{tabular}{ |c|c| }
				\cline{1-2}
		\textbf{name} & \textbf{description} \\
				\cline{1-2}
		\cMarker{apple} & \cMarker{red ~fruit}\\
%				\cline{1-2}
		\cMarker{carrot} & \uMarker{red ~vegetable}\\
%				\cline{1-2}
		\cMarker{tomato} & \uMarker{red ~fruit}\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}
\caption{expression combination rules example: result string is uncertain if any of the input strings are uncertain. The result is certain if all of the input strings are certain.}
\label{table:4.attr}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:


==> uaa-rels.tex <==
%!TEX root=./uaadb.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\abbrUAADBs}
\label{sec:uaa-range}

We define \termUAADBs (\abbrUAADBs) as a special type of $\semK$-relation over range-annotated domains and demonstrate how to bound an incomplete $\semK$-relation using this model.
Afterwards, we define a metric for how precise the bounds of an incomplete $\semK$-database encoded by an \abbrUAADB are, and  define a query semantics for \abbrUAADBs  that preserves bounds.
We limit the discussion to semiring $\semN$ (bag semantics). See~\cite{techreport} for the generalization to other semirings including $\semB$ (set semantics). % (semirings whose elements form a lattice structure).
% For the general construction  that works for any l-semiring (a semiring whose elements form a lattice structure) including $\semB$ (set semantics) see~\cite{techreport}.
% }
% \iftechreport{
% \abbrUAADBs are definedfor any l-semiring (a semiring whose elements form a lattice structure) including $\semB$ (set semantics), $\semN$ (bag semantics), security clearance annotations, and various types of provenance.
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\uaaN$-relations}\label{sec:uaadbs}

In addition to allowing for range-annotated values, \abbrUAADBs also differ from \abbrUADBs in that they encode an upper bound of the possible annotation of each tuple. We use $\semqN$ annotations to encode for each tuple: a lower bound on the certain multiplicity of the tuple, the  multiplicity of the tuple in the \abbrBGW, and an over-approximation of the tuple's possible multiplicity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Tuple-level Annotations]
  \label{def:uaa-tuple-annot}
The % level
range-annotated multiplicity domain $\uaaDomN$ is defined as:\\[-6mm]
%
  $$\{ \ut{\lbMarker{k}}{k}{\ubMarker{k}} \mid \lbMarker{k}, k, \ubMarker{k} \in \semN \wedge \lbMarker{k} \leq k \leq \ubMarker{k} \}$$
We use $\uaaN$ to denote semiring $\semqN$ restricted to elements from $\uaaDomN$.
  \end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  % Similar to the range-annotated domain,
  % A value $\ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}}$ from $\uaaN$ encodes an element from $\semN$ and two elements ($\lbMarker{k}$ and $\ubMarker{k}$) that bound the element from below and above.
  % Given an
  % $\uaaN$-element $k = \ut{k_1}{k_2}{k_3}$ we define
  % $\lbMarker{k} = k_1$, $\bgMarker{k} = k_2$, and $\ubMarker{k} = k_3$.
  Note that $\uaaN$ is a semiring since when combining two elements of
  $\uaaN$ with $\addOf{\semqN}$ and $\multOf{\semqN}$, the result
  $\ut{\lbMarker{k}}{\bgMarker{k}}{\ubMarker{k}}$ fulfills the requirement $\lbMarker{k} \leq \bgMarker{k} \leq \ubMarker{k}$. This is
  the case because  addition and multiplication in $\semN$ preserve
   order~\cite{FH19}, and these operations in $\semqN$ are pointwise
  application of $\addN$ and $\multN$. % , e.g.,
  % $\ut{\lbMarker{k}}{k}{\ubMarker{k}} \addOf{\semqN} \ut{\lbMarker{l}}{l}{\ubMarker{l}} = \ut{\lbMarker{l} \addN \lbMarker{l}}{k \addN l}{\ubMarker{k}
  % \addN \ubMarker{l}}$ and
  % $k_1 \ordN k_2 \wedge k_3 \ordN k_4 \Rightarrow k_1 \addN k_3 \ordN k_2 \addN
  % k_4$ for any $k_1, k_2, k_3, k_4 \in \semN$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{Definition}% [$\uaaN$-relations]
    \label{def:uaa-rels}
% Given a range-annotated data domain $\rangeDom$,
A $\uaaN$-relation of arity $n$ is a function $\rangeRel: \rangeDom^n \rightarrow \uaaN$ with finite support $\{ \rangeTup \mid \rangeRel(\rangeTup) \neq \ut{0}{0}{0} \}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \BGdel{DONT THINK WE USE THIS UNTIL MUCH LATER WHERE WE EXPLAIN IT AGAIN ANYWAYS: As a notational convenience we show certain values, i.e., values $c \in \rangeDom$ where $\lbMarker{c} = \bgMarker{c} = \ubMarker{c} = c'$, as the deterministic value $c'$ they encode.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Extracting \capitalBGW}\label{sec:uaab-get-bgw}

$\uaaN$-relations permit multiple tuples with identical values in the \termBGW (\abbrBGW). % \abbrBG values.
We extract the \termBGW encoded by a $\uaaN$-relation by grouping tuples based on their \abbrBG values and summing up their \abbrBG multiplicities.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:bool-to-K}
We lift operator $\bgName$ from values to tuples: $\bgName: \rangeDom^n \to \dataDomain^n$, i.e., given an \abbrUAADB tuple $\rangeTup = \tuple{c_1, \ldots, c_n}$, % we define
$\bgOf{\rangeTup} \defas \tuple{\bgMarker{c_1}, \ldots, \bgMarker{c_n}}$. For a  $\uaaN$-relation $\rangeRel$, $\bgOf{\rangeRel}$, the \abbrBGW encoded by $\rangeRel$, is then defined as:\\[-5mm]
%
$$\bgOf{\rangeRel}(\tup) \defas \sum_{\bgOf{\rangeTup} = \tup} \bgOf{\left(\rangeRel(\rangeTup)\right)}$$
%  The corresponding $\uaak{\semN}$-relation  $D_{bg}=\{t \rightarrow \sum_{BG(\rangeTup)=t} \rangeTup.k\}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{ex:audb-instance}
\Cref{table:UAAR_inst} shows an instance of a $\uaaN$-relation $\rel$ where each attribute is a triple showing the lower bound, \termBG, and upper bound of the value. Each tuple is annotated by a triple showing the lower multiplicity bound, \termBG multiplicity, and the upper multiplicity bound of the tuple. % Since this is a $\uaaN$ relation, the annotations encode multiplicities of tuples.
For example, the first tuple represents a tuple $\tuple{1,1}$ that appears at least twice in every possible world (its lower multiplicity bound  is $2$), appears twice in the \abbrBGW, and appears no more than thrice in any world.
	\Cref{table:UAAR_bg} shows the \abbrBGW encoded by this \abbrUAADB which is computed by summing up the multiplicities of tuples with identical \abbrBG values. For instance, the first two tuples both represent tuple $\tuple{1,1}$ in the \abbrBGW and their annotations sum up to $5$ (i.e., the tuple $\tuple{1,1}$ appears five times).
  \revm{Conversely, the first two tuples of $\db_2$ match different \abbrUAADB tuples.}
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\centering

    \begin{minipage}{0.465\linewidth}
	\begin{subtable}{\linewidth}
	\centering
	\begin{tabular}{ c|cc}
      \textbf{A}  & \textbf{B}  & \underline{\semqN} \\
      				\cline{1-2}
		$\uv{1}{1}{1}$ & $\uv{1}{1}{1}$ & \ut{2}{2}{3}\\
		$\uv{1}{1}{1}$ & $\uv{1}{1}{3}$ & \ut{2}{3}{3}\\
		$\uv{1}{2}{2}$ & $\uv{3}{3}{3}$ & \ut{1}{1}{1}\\
	\end{tabular}
	\caption{Example \abbrUAADB instance}
	\label{table:UAAR_inst}
	\end{subtable}
  \end{minipage}
  \begin{minipage}{0.505\linewidth}
	\begin{subtable}{\linewidth}
	\centering
	% \begin{tabular}{ c|cc}
	% 	\textbf{A}  & \textbf{B}  & \underline{$\semN$}  \\
	% 	\cline{1-2}
	% 	$1$ & $1$ & 5\\
	% 	$2$ & $3$ & 1\\
        %    \end{tabular}
    \begin{minipage}{0.490\linewidth}
      \centering
    \underline{$\db_1$}                                                                           \\
    	\begin{tabular}{lc|cc}
                               & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
		\cline{2-3}
$\tup_1$                       & $1$                        & $1$        & 5                      \\
$\tup_2$                       & $2$                        & $3$        & 1                      \\
	\end{tabular}
  \end{minipage}
  \begin{minipage}{0.49\linewidth}
    \centering
    \underline{$\db_2$}                                                                           \\
    \begin{tabular}{lc|cc}
                               & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
		\cline{2-3}
 $\tup_3$                      & $1$                        & $1$        & 2                      \\
 $\tup_4$                      & 1                          & 3          & 2                      \\
$\tup_5$                       & $2$                        & $3$        & 1                      \\
	\end{tabular}
  \end{minipage}
  	\caption{Worlds $\db_1$ (\abbrBGW) and $\db_2$}
	\label{table:UAAR_bg}
	\end{subtable}
  \end{minipage}\\[-3mm]
	\caption{Example \abbrUAADB relation and two worlds it bounds}
  \label{table:UAAR_overall}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[ht]
%   \BG{F and T should be introduced beforehand}
% 	\centering
% 	\begin{subtable}{0.4\linewidth}
% 	\centering
% 	\caption{R-D1}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  &  \\
% 		\cline{1-2}
% 		1 & 1 & 2\\
% %				\cline{1-3}
% 		1 & 2 & 3\\
% %				\cline{1-3}
% 		2 & 3 & 1\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}
% 	\begin{subtable}{0.4\linewidth}
% 	\centering
% 	\caption{R-D2}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  &  \\
% 		\cline{1-2}
% 		1 & 1 & 3\\
% %				\cline{1-3}
% 		1 & 2 & 2\\
% %				\cline{1-3}
% 		1 & 3 & 2\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB BG=D1 \\ Similar to tuple level}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
% %				\cline{1-3}
% 		$1^{[1,1]}$ & $2^{[2,2]}$ & (2,3,3)\\
% %				\cline{1-3}
% 		$2^{[2,2]}$ & $3^{[3,3]}$ & (0,1,1)\\
% 		$1^{[1,1]}$ & $3^{[3,3]}$ & (0,0,2)\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB one-liner}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,2]}$ & $1^{[1,3]}$ & (6,6,7)\\
% %				\cline{1-3}
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB BG=D1}
% 	\begin{tabular}{ |c|c|l}
% 				\cline{1-2}
% 		\textbf{A}  & \textbf{B}  & (c, d, p)  \\
% 		\cline{1-2}
% 		$1^{[1,1]}$ & $1^{[1,1]}$ & (2,2,3)\\
% %				\cline{1-3}
% 		$1^{[1,1]}$ & $2^{[2,3]}$ & (3,3,3)\\
% %				\cline{1-3}
% 		$2^{[1,2]}$ & $3^{[3,3]}$ & (1,1,1)\\
% 				\cline{1-2}
% 	\end{tabular}
% 	\end{subtable}

% 	\vspace*{0.5 cm}

% 	\begin{subtable}{\linewidth}
% 	\centering
% 	\caption{UADB GB=D1 tuple matchings}
% 	\begin{tabular}{ |c|}
% 				\cline{1-1}
% 		\textbf{Certain matching}\\
% 		\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D1(1,2) = 3$\\
% %				\cline{1-3}
% 		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D1(2,3) = 1$\\
% 				\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,2) = 2$\\
% %				\cline{1-3}
% 		$(1^{[1,1]}, 2^{[2,3]}) \rightarrow D2(1,3) = 1$\\
% 		$(2^{[1,2]}, 3^{[3,3]}) \rightarrow D2(1,3) = 1$\\
% 			\cline{1-1}
% 		\textbf{Possible matching} \\
% 		\cline{1-1}
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D2(1,1) = 1$\\
% 		$(1^{[1,1]}, 1^{[1,1]}) \rightarrow D1(1,1) = 1$\\
% 		\cline{1-1}
% 	\end{tabular}
% 	\end{subtable}
% \BG{Do we need this long example here?}
% \caption{A \abbrUAADB-DB instance correspond to possible worlds semantics}
% \label{fig:exp1}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Encoding Bounds}\label{sec:uaadb-bounds}

We now define what it means for an \abbrUAADB to bound an incomplete $\semN$-relation. For that, we first define bounding of deterministic tuples by range-annotated tuples. % bound (match).
%We use \abbrUAADB relation to bound all possible worlds from an incomplete database. Starting from bounding a tuple from each possible world to a \abbrUAADB tuple.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Tuple Bounding]
  \label{def:bounding-tuples}
  Let  $\rangeTup$ be a  range-annotated tuple with schema $\tuple{a_1, \ldots, a_n}$ and   $\tup$ be a tuple  with the same schema as $\rangeTup$. We say that $\rangeTup$ bounds $\tup$ written as $\tup \tmatch \rangeTup$ iff\\[-3mm]
  %
  \[
    \forall{i \in \{1, \ldots ,n\}}:
    \lbMarker{\rangeTup.a_i} \leq \tup.a_i \leq \ubMarker{\rangeTup.a_i}
  \]
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Bounding $\uaaN$ Annotations]\label{def:bounding-annotations}
% 	A value $k \in \uaaN$ is said to bound a set of values $S_k = \{k_1, \ldots, k_n\}$ from $\semN$ if:
%   \begin{align*}
%     \forall k_i \in S_k: \lbMarker{k} \leq k_i \leq \ubMarker{k}\\
%     \exists k_i \in S_k: k_i = \bgMarker{k}
%   \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

One \abbrUAADB tuple may bound multiple conventional tuples and vice versa. We define \textit{tuple matchings} as a way to match the multiplicities of  tuples of a $\uaaN$-database (or relation) with that of one possible world of an incomplete $\semN$-database (or relation).
Based on tuple matchings we then define how to  bound possible worlds.
% a mapping between a set of \abbrUAADB tuples and a set of deterministic tuples.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Tuple matching]
  \label{def:tuple-matching}
  Let $\rangeRel$ be an $n$-ary \abbrUAARel and $\rel$ an $n$-ary relation. A \emph{tuple matching} $\TM$ for $\rangeRel$ and $\rel$ is a function $(\rangeDom)^{n} \times \dataDomain^n \to \semN$.
  % $$TM_{R^I,R}(\rangeTup,t)=k$$ is the mappings from an annotated tuple $\rangeTup$ and a possible world tuple $t$ to a semiring element $k$
  \st the following conditions hold:\\[-3mm]
  %%%%%%%%%%%%%%%%%%%%
  \begin{align*}
    &\forall \rangeTup \in \rangeDom^n: \forall \tup \ntmatch \rangeTup: \TM(\rangeTup, \tup) = \zeroN
    &\forall \tup \in \dataDomain^n: \sum_{\rangeTup \in \rangeDom^n} \TM(\rangeTup, \tup)=\rel(\tup)
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A tuple matching distributes the multiplicity of a tuple from $\rel$ over one or more matching tuples from $\rangeRel$.  Multiple tuples from an \abbrUAADB may encode the same tuple when the multidimensional rectangles of their attribute-level range annotations overlap, as with the first two tuples of the \abbrUAADB in \Cref{table:UAAR_overall} and the \abbrBGW.
%. For instance,  $\tuple{\uv{1}{2}{3}}$ and $\tuple{\uv{2}{3}{5}}$ both match the tuple $\tuple{2}$.
% The conditions stating that a \abbrUAADB tuple can only match to conventional tuple if the tuple is bounded by the \abbrUAADB tuple. Also all the conventional tuples in relation $\rel$ need to be matched in the tuple matching.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:bounding-worlds}
  Given an n-ary \abbrUAADB relation $\rangeRel$ and an n-ary deterministic $\semN$-relation $\rel$ (a possible world),  relation $\rangeRel$ bounds $\rel$ (denoted $\rel \dbbounds \rangeRel$) iff there exists a tuple matching $\TM$ for $\rangeRel$ and $\rel$ \st \\[-5mm]
%
  \begin{align*} %\label{eq:lower-bound-db}
    &\forall \rangeTup \in \rangeDom^n:\sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \geq \lbMarker{\rangeRel(\rangeTup)}
    \;\text{\textbf{and}}\; % \forall \rangeTup \in \rangeDom^n:
       \sum_{\tup \in \dataDomain^n} \TM(\rangeTup,\tup) \leq \ubMarker{\rangeRel(\rangeTup)} %\label{eq:upper-bound-db}
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Having defined when a possible world is bound by a $\uaaN$-relation, we are ready to define bounding of incomplete $\semN$-relations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}\label{def:bounding-incomplete-dbs}
	Given an incomplete $\semN$-relation $\prel$ and a $\uaaN$-relation $\rangeRel$, we say that $\rangeRel$ bounds $\prel$, written as $\prel \dbbounds \rangeRel$
  iff
    \begin{align*}
    &\forall \rel \in \prel: \rel \dbbounds \rangeRel
    &&\exists \rel \in \prel: \rel = \bgOf{\rangeRel}
    \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent These definitions are extended to databases in the obvious way.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}\label{ex:bounding-incomplete-dbs}
  Consider the \abbrUAADB from \Cref{ex:audb-instance} and the worlds from~\Cref{table:UAAR_bg}. % shown below.
%
%   \begin{minipage}{0.49\linewidth}
%     \centering
%     \underline{$\db_1$}                                                                           \\
%     	\begin{tabular}{lc|cc}
%                                & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
% 		\cline{2-3}
% $\tup_1$                       & $1$                        & $1$        & 5                      \\
% $\tup_2$                       & $2$                        & $3$        & 1                      \\
% 	\end{tabular}
%   \end{minipage}
%   \begin{minipage}{0.49\linewidth}
%     \centering
%     \underline{$\db_2$}                                                                           \\
%     \begin{tabular}{lc|cc}
%                                & \textbf{A}                 & \textbf{B} & \underline{$\semN$}    \\
% 		\cline{2-3}
%  $\tup_3$                      & $1$                        & $1$        & 2                      \\
%  $\tup_4$                      & 1                          & 3          & 2                      \\
% $\tup_5$                       & $2$                        & $4$        & 1                      \\
% 	\end{tabular}
%   \end{minipage}
  The \abbrUAADB bounds these worlds, since there exist tuple matchings that provide a lower and an upper bound for the annotations of the tuples of each world. For instance, denoting the tuples from this example as
  %
  \begin{align*}
    \rangeTup_1                & \defas \tuple{\uv{1}{1}{1}, \uv{1}{1}{1}}
                               & \rangeTup_2                & \defas \tuple{\uv{1}{1}{1}, \uv{1}{1}{3}}\\
                                \rangeTup_3                & \defas \tuple{\uv{1}{2}{2}, \uv{3}{3}{3}}
  \end{align*} %
  \iftechreport{Tuple matchings $\TM_1$ and $\TM_2$ shown below to bound $\db_1$ and $\db_2$.}
  \ifnottechreport{Tuple matching $\TM_1$ shown below bounds $\db_1$.}
  \begin{align*}
    \TM_1(\rangeTup_1, \tup_1) & = 2
                               & \TM_1(\rangeTup_2, \tup_1) & = 3
                               & \TM_1(\rangeTup_3, \tup_1) & = 0                                 \\
    \TM_1(\rangeTup_1, \tup_2) & = 0
                               & \TM_1(\rangeTup_2, \tup_2) & = 0
                               & \TM_1(\rangeTup_3, \tup_2) & = 1
    \iftechreport{\\[2mm]
    \TM_2(\rangeTup_1, \tup_3) & = 2
                               & \TM_2(\rangeTup_2, \tup_3) & = 0
                               & \TM_2(\rangeTup_3, \tup_3) & = 0                                 \\
    \TM_2(\rangeTup_1, \tup_4) & = 0
                               & \TM_2(\rangeTup_2, \tup_4) & = 2
                               & \TM_2(\rangeTup_3, \tup_4) & = 0                                 \\
    \TM_2(\rangeTup_1, \tup_5) & = 0
                               & \TM_2(\rangeTup_2, \tup_5) & = 0
                               & \TM_2(\rangeTup_3, \tup_5) & = 1
%
}
  \end{align*}
    \end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \BG{removed this: fig:exp1 shows an example of a \abbrUAADB-DB with a possible tuple matching that fulfills the correctness criteria.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tightness of Bounds}
\label{sec:approximation-factor}

% \Cref{def:bounding-incomplete-dbs} defines what it means for an \abbrUAADB to bound an incomplete databases. However,
Given an incomplete database, there are many possible \abbrUAADBs that bound it, differing in tightness. For instance, both $\rangeTup_1 \defas \tuple{\uv{1}{15}{100}}$ and $\rangeTup_2 \defas \tuple{\uv{13}{14}{15}}$ bound tuple $\tuple{15}$, but intuitively the bounds provided by $\rangeTup_2$ are tighter. We develop a metric for the tightness of the approximation provided by an \abbrUAADB and prove that finding an \abbrUAADB that maximizes tightness % when we limit the size of the \abbrUAADB
is intractable. Given two \abbrUAADBs $\rangeDB$ and $\rangeDB'$ that both bound an incomplete $\semN$-database $\pdb$, $\rangeDB$ is a tighter bound than $\rangeDB'$ if the set of worlds bound by $\rangeDB$ is a subset of the set of worlds bound by $\rangeDB'$. % As a sanity check, consider $\rangeDB_1 \defas \{t_1\}$ and $\rangeDB_2 \defas \{t_2\}$ using $t_1$ and $t_2$ from above and assume that $\dataDomain = \semN$. Then $\rangeDB_2$ is a tighter bound than $\rangeDB_1$ since the three deterministic databases it bounds $\{(13)\}$, $\{(14)\}$ and $\{(15)\}$ are also bound by $\rangeDB_1$, but $\rangeDB_1$ bounds additional databases, e.g., $\{(2)\}$. % that are not bound by $\rangeDB_2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}% [Bound Tightness]
  \label{def:bound-tightness}
  Consider two $\uaaN$-databases $\rangeDB$ and $\rangeDB'$ over the same schema
$\aschema$. We say that $\rangeDB$ is at least as tight as $\rangeDB'$, written as $\rangeDB \dbleq \rangeDB'$, if for all $\semN$-databases $\db$ with schema $\aschema$ we have:
  \begin{align*}
 \db \dbbounds \rangeDB \rightarrow \db \dbbounds \rangeDB'
  \end{align*}
  We say that $\rangeDB$ is strictly tighter than $\rangeDB'$, written as $\rangeDB \dble \rangeDB'$ if $\rangeDB \dbleq \rangeDB'$ and there exists $\db \dbbounds \rangeDB'$ with $\db \not\dbbounds \rangeDB$. Furthermore, we call $\rangeDB$  a maximally tight bound for an incomplete $\semN$-database $\pdb$ if:
  \begin{align*}
    \pdb &\dbbounds \rangeDB
   &\not \exists \rangeDB':\; \pdb \dbbounds \rangeDB' \wedge \rangeDB' \dble \rangeDB
  \end{align*}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This notion of tightness is well-defined even if the data domain $\dataDomain$ is infinite. % For instance, if we use the reals $\mathbb{R}$ instead of natural numbers as the domain in the example above, then still $\rangeDB_1 \dbge \rangeDB_2$.
In general \abbrUAADBs that are tighter bounds are preferable. However, computing a maximally tight bound is intractable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}\label{def:intractability-of-tight-bounds}
Let $\pdb$ be an incomplete $\semN$-database encoded as a \abbrCtable~\cite{DBLP:journals/jacm/ImielinskiL84}.  % in the size of $\pdb$
Computing a maximally tight bound $\rangeDB$ for $\pdb$ is \nphard.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof Sketch]
  \ifnottechreport{
    Proven through reduction from 3-colorability~\cite{techreport}.
    We construct a C-table with one tuple and encode the 3-colorability of the input graph $G$ in the local condition of the tuple, i.e., the tuple is possible iff $G$ is 3-colorable.
    The maximally tight  upper multiplicity bound for this tuple is $1$ iff graph $G$ is 3-colorable.
  }
  \iftechreport{
We prove the claim through a reduction from 3-colorability.
\BG{Write proof. can we generalize to any model not just C-tables. If yes, does this require a size-bound?}
    }
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In the light of this result, we devise methods for translating incomplete and probabilistic databases into \abbrUAADBs that do not guarantee tight bounds.
% Even if we were able to compute tight bounds, preserving these bounds under  queries is computationally hard. This follows from well-known hardness results for computing certain answers.
% Thus, % even if the input is maximally tight,
% our query semantics does not preserve tightness of bounds.
% Note that this strictly necessary since computing tight bounds on aggregation function results is already hard in incomplete and probabilistic databases (e.g., see~\cite{DBLP:journals/tcs/ArenasBCHRS03}).
% Nonetheless, % comparing the tightness of \abbrUAADBs is useful for
% we will use this metric in \Cref{sec:experiments} to evaluate relative tightness of bounds.
  % (this follows from hardness results for computing tight bounds for the results of an aggregation query over incomplete databases).
%\subsection{Tuple matching}
%Define matching $t' \tmatches t$ as true iff $\forall{i \in [1,n]}:t(a_i) \in I_{t'(a_i)}$ \\
%A tuple matching $TM_{R',R}(t',t)=k$ is the mappings from an annotated tuple $t'$ and a possible world tuple $t$ to a semiring value $k$. \\
%As a constrain, any tuple matching need to fully match all certain tuples from annotated relation:
%$$\forall_{t' \in R'}:\sum_{t \in R}TM_{R',R}(t',t)=R'(t').k_c$$
%A annotated relation $R'$ is c-sound if:
%$$\forall_{D(R) \in \dataDomain}:\exists TM_{R',R}:\forall_{t \in R}:\sum_{t' \in R'}TM_{R',R}(t',t) \leq R(t)$$
%A annotated relation $R'$ is p-complete if:
%$$\forall_{t' \in R'}:\sum_{t \in R}TM_{R',R}(t',t)=R'(t').k_p$$
%$$\forall_{D(R) \in \dataDomain}:\exists TM_{R',R}:\forall_{t \in R}:\sum_{t' \in R'}TM_{R',R}(t',t) \geq R(t)$$



%%%
%\subsection{Certain tuples based tuple matching}
%In certain tuples based tuple matching, we match annotated tuples to certain tuples in all possible worlds.\\
%An annotated relation $R'$ is c-sound if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \leq certain(\dataDomain)(t)$$
%A annotated relation $R'$ is c-complete if:
%$$\exists TM:\forall_{t' \in R'}:\sum_{t \in R}TM(R',R,t',t) \geq certain(\dataDomain)(t)$$
%%%

%\subsection{Expressions}
%An attribute $x$ is certain iff the upper bound and lower bound of the attribute are equal.
%Comparison and boolean operators can be defined as:
%\begin{enumerate}
%\item \[ \begin{cases}
%\ubMarker{(a>b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \\
%\ubMarker{(a>b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\[ \begin{cases}
%\lbMarker{(a>b)} = T & \text{if } \lbMarker{a}>\ubMarker{b} \\
%\lbMarker{(a>b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\item \[ \begin{cases}
%\ubMarker{(a=b)} = T & \text{if } \ubMarker{a}>\lbMarker{b} \wedge \lbMarker{a}<\lbMarker{b} \vee \ubMarker{a}>\ubMarker{b} \wedge \lbMarker{a}<\ubMarker{b} \\
%\ubMarker{(a=b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\[
%\begin{cases}
%\lbMarker{(a=b)} = \btrue & \text{if } \ubMarker{a}=\lbMarker{b} \wedge \ubMarker{b}=\lbMarker{a} \\
%\lbMarker{(a=b)} = \bfalse & \text{else}
%\end{cases}
%\]
%\item \[ \ubMarker{(p \wedge q)} = \ubMarker{p} \wedge \ubMarker{q} \]
%\[ \lbMarker{(p \wedge q)} = \lbMarker{p} \wedge \lbMarker{q} \]
%\item \[ \ubMarker{(p \vee q)} = \ubMarker{p} \vee \ubMarker{q} \]
%\[ \lbMarker{(p \vee q)} = \lbMarker{p} \vee \lbMarker{q} \]
%\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uaadb"
%%% End:

